Syntactic Effectful Realizability in Higher-Order Logic

Realizability interprets propositions as specifications for computational entities in programming languages. Specifically, syntactic realizability is a powerful machinery that handles realizability as a syntactic translation of propositions into new propositions that describe what it means to realize the input proposition. This paper introduces EffHOL (Effectful Higher-Order Logic), a novel framework that expands syntactic realizability to uniformly support modern programming paradigms with side effects. EffHOL combines higher-kinded polymorphism, enabling typing of realizers for higher-order propositions, with a computational term language that uses monads to represent and reason about effectful computations. We craft a syntactic realizability translation from (intuitionistic) higher-order logic (HOL) to EffHOL, ensuring the extraction of computable realizers through a constructive soundness proof. EffHOL's parameterization by monads allows for the synthesis of effectful realizers for propositions unprovable in pure HOL, bridging the gap between traditional and effectful computational paradigms. Examples, including continuations and memoization, showcase EffHOL's capability to unify diverse computational models, with traditional ones as special cases. For a semantic connection, we show that any instance of EffHOL induces an evidenced frame, which, in turn, yields a tripos and a realizability topos.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 2.03.  Cleaned generation of samples.
	       New options for printing conference proceedings
	       in ACM journals

Version 2.02   Documentation update.
	       Changes in TOG templates
	       Corrected typo in ACM/IMS journals

Version 2.01   \acmPrice now produces a warning.

Version 2.00   ACM switches to electronic only version.
	       We do not print article tabs anymore.
	       New copyright wording.
	       Deleted \acmPrice.

Version 1.93   Added PACMSE

Version 1.92   Documentation update
	       Emergency change: changed order of hyperref and hyperxmp
	       due to changes in the undelying packages

Version 1.91   Minor changes in ACMCP format

Version 1.90a  Changes in the sample keywords and concepts

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> section/CC.tex <==


\begin{figure*}[t]
  %  \centering
  \hspace*{-0.5cm}
\begin{small}
   \scalebox{0.9}{
   \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}@{}l|@{\hspace{-0.15in}}l|@{\hspace{-0.15in}}l@{\hspace{0.5in}}}%{@{}l|@{\hspace{-0.15in}}l|@{\hspace{-0.15in}}l@{\hspace{0.5in}}}
   $ \begin{array}[t]{@{}l@{\hspace{0.2in}}l@{\hspace{0.07in}}l@{\hspace{0.07in}}l}
   %%%%%%%%%%%%%%%%%% SORT -> KIND %%%%%%%%%%%%%%%%%%%%%%
       \multicolumn{4}{c}{ \boldsymbol{\ttrkind{-} : \mathtt{sort} \to \mathtt{kind}}}
        \\[\sskip]
        & \ttrkind{\STAR} &\eqdef& \star
        \\[0.1cm]
        &\ttrkind{\predcon{\sort}} &\eqdef& \typecon{\ttrkind{\sort}}  
    \end{array}$
    &
    $\begin{array}[t]{@{}l@{\hspace{0.2in}}l@{\hspace{0.07in}}l@{\hspace{0.07in}}l}
    %%%%%%%%%%%%%%%%%% TERM -> TYPE %%%%%%%%%%%%%%%%%%%%%%
      \multicolumn{4}{c}{\boldsymbol{\ttretype{\scontext}{-}{\sort} : \mathtt{term} \to \mathtt{type}}}\\[\sskip]
    %%% var
        &\ttretype{\scontext}{\spred}{\sort} &\eqdef& \typevar_{\spred}\\[0.1cm]
    %%% comprehension
        &\ttretype{\scontext}{\comprehend{\spred}{\sort}{\sprop}}{\predcon{\sort}} &\eqdef& \typeabs{\typevar_\spred}{\ttrkind{\sort}}{\ttrtype{\scontext , \spred : \sort}{\sprop}}
        \\[0.1cm]
        &\ttretype{\scontext}{\compbase{\sprop}}{\predcon{\sort}} &\eqdef& {\ttrtype{\scontext , \spred : \sort}{\sprop}}
    \end{array}$
&
   $\begin{array}[t]{@{}l@{\hspace{0.2in}}l@{\hspace{0.07in}}l@{\hspace{0.07in}}l}
      %%%%%%%%%%%%%%%%%% TERM -> EXPRESSION %%%%%%%%%%%%%%%%%%%%%%
        % \ttrtrm{\scontext}{-}{\sort}  : \left(\sterm : \mathtt{term}_{\scontext}\left(\sort\right)\right) \to \mathtt{expression}\left(\ttrind{\trtype{}{\sterm} }{\sort} \right)&&&\\
        \multicolumn{4}{c}{\boldsymbol{\ttrtrm{\scontext}{-}{\sort}  : \mathtt{term} \to \mathtt{expr}}}\\[\sskip]
    %%% var
        &\ttrtrm{\scontext}{\spred}{\sort} &\eqdef& \tpred_{\spred}\\[0.1cm]
    %%% comprehension
        &\ttrtrm{\scontext}{\comprehend{\spred}{\sort}{\sprop}}{\predcon{\sort}} &\eqdef& \eforall{\typevar_{\spred} : \ttrkind{\sort}}{
            \tcomp{\termvar}{\ttrtype{\scontext , \spred : \sort}{\sprop}}
               {\tpred_\spred}{\ttrind{\typevar_\spred}{\sort}}
               {\ttrspec{\scontext , \spred : \sort}{\sprop}{x} }
            }     \\[0.1cm]
          &\ttrtrm{\scontext}{\compbase{\sprop}}{\predcon{\sort}} &\eqdef& {
            \tcompbase{\termvar}{\ttrtype{\scontext , \spred : \sort}{\sprop}}
               {\ttrspec{\scontext , \spred : \sort}{\sprop}{x} }
            }
\end{array}$
    \\[\sskip]
    \\
    \hline
    \\
    $\begin{array}[t]{@{}l@{\hspace{0.2in}}l@{\hspace{0.07in}}l@{\hspace{0.07in}}l}
   %%%%%%%%%%%%%%%%%% SORT -> INDEX %%%%%%%%%%%%%%%%%%%%%%
        \multicolumn{4}{c}{ \boldsymbol{\ttrind{-}{-} : \mathtt{sort} \to \mathtt{type}\to \mathtt{index}}}
        \\[\sskip]
        & \ttrind{\type} {\STAR} &\eqdef& \refpredN{\type} 
        \\[0.1cm]
        &\ttrind{\type} {\predcon{\sort}} &\eqdef& \tindprod{\typevar_{0} : \ttrkind{\sort}}{
        \refpred{\typeapp{\type}{\typevar_{0}}}{\ttrind{\typevar_{0} }{\sort}}}
    \end{array}$
    &
    $\begin{array}[t]{@{}l@{\hspace{0.2in}}l@{\hspace{0.07in}}l@{\hspace{0.07in}}l}
 %%%%%%%%%%%%%%%%%% PROPOSITION -> TYPE %%%%%%%%%%%%%%%%%%%%%%
    \multicolumn{4}{c}{   \boldsymbol{\ttrtype{\scontext}{-} : \mathtt{prop} \to \mathtt{type}}}
        \\[\sskip]
    %%% implication
        &\ttrtype{\scontext}{\simplies{\sprop_{1}}{\sprop_{2}}} &\eqdef& \typefun{\ttrtype{\scontext}{\sprop_{1}} } {M \ttrtype{\scontext}{\sprop_{2}}}\\[0.1cm]
    %%% forall
        &\ttrtype{\scontext}{\forall_{\spred : \sort}  \sprop} &\eqdef&  \ttypprod{\typevar_\spred :\ttrkind{\sort}} {\typecomp{\ttrtype{\scontext , \spred : \sort}{\sprop}}}\\[0.1cm]% \lcnote{should be X_u'?}\\
    %%% membership
        &\ttrtype{\scontext}{\smem{ \sterm_{1} }{\sterm_{2}} } &\eqdef& \typeapp{\ttretype{\scontext}{\sterm_{2}}{\predcon{\sort}}}{\ttretype{\scontext}{\sterm_{1}}{\sort}}
        \\[0.1cm]
       &\ttrtype{\scontext}{\smembase{\sterm} }{} &\eqdef& {\ttretype{\scontext}{\sterm}{}}
        \\
    \end{array}$
    &
    $\begin{array}[t]{@{}l@{\hspace{0.2in}}l@{\hspace{0.07in}}l@{\hspace{0.07in}}l}
   %%%%%%%%%%%%%%%%%% PROPOSITION -> SPECIFICATION %%%%%%%%%%%%%%%%%%%%%%
      \multicolumn{4}{c}{   \boldsymbol{\ttrspec{\scontext}{-}{-} : \mathtt{prop} \to \mathtt{prog}\to \mathtt{spec}}}
        \\[\sskip]
    %%% implication
        &\ttrspec{\scontext}{\simplies{\sprop_{1}}{\sprop_{2}}}{\term} &\eqdef& \tspectypprod{\termvar_{1} : \ttrtype{\scontext}{\sprop_{1}} }{ \ttrspec{\scontext}{\sprop_{1}}{\termvar_{1}} \supset \after{\termapp{\term}{\termvar_{1}}}{\termvar_{2}}{\ttrspec{\scontext}{\sprop_{2}}{\termvar_{2}}}}\\[0.1cm]
    %%% forall
        &\ttrspec{\scontext}{\forall_{\spred : \sort} \sprop}{\term} &\eqdef& \tspeckinprod{\typevar_\spred : \ttrkind{\sort}} \forall_{\tpred_\spred : \ttrind{\typevar_\spred}{\sort} } .
        \after{\termtypeapp{\term}{\typevar_\spred}}{\termvar_{0}}{\ttrspec{\scontext , \spred : \sort}{\sprop}{\termvar_{0}}}\\[0.1cm]
     %   {\color{red}\subst{ \tpred_{\spred} \eqdef\tpred }}}\lcnote{I think we don't need it}\\
    %%% membership
        &\ttrspec{\scontext}{\smem{ \sterm_{1}}{\sterm_{2}} }{\term} & \eqdef& \tmem{ \term }{ \eapp{\ttrtrm{\scontext}{\sterm_{2}}{\predcon{\sort}}}{\ttretype{\scontext}{\sterm_{1}}{\sort}} }{ \ttrtrm{\scontext}{\sterm_{1}}{\sort} }
        \\[0.1cm]
        &\ttrspec{\scontext}{\smembase{ \sterm}}{\term} & \eqdef& \tmembase{ \term }{ \ttrtrm{\scontext}{\sterm}{\predcon{\sort}}}
        \\
    \end{array}$
\end{tabular*}
}
\end{small}  
% \emnote{Due to the way we translate $u$, I think we \textbf{have} to be careful with  name variables $X_u$/$y_u$ (and not only $X$/$y$)}
    \caption{The Realizability Translation}
    \label{fig:trans2exists}
\end{figure*}


\begin{definition}[Internal CC for Tripos]\label{cc-tripos}
CC holds internally in a tripos when the following holds in its internal model of higher-order logic for all sets~$I$:
\begin{center}$\begin{array}{@{}c@{}}
\forall R : \N \times I \to \Omega.\; \Total(R) \;\supset\; \exists S : \N \times I \to \Omega.\; \Total(S) \mathrel{\wedge} S \mathop{\subseteq} R \mathrel{\wedge} \Det(S) \\[2pt]
\text{where} \\[2pt]
\begin{array}{@{}r@{{}={}}l@{\qquad}r@{{}={}}l@{}}
\Total(R) & \forall n : \N.\; \isnat \supset \exists i : I.\; n \mathrel{R} i &
\isnat & \forall \phi : \N \to \Omega.\; \phi(0) \mathrel{\wedge} (\forall n' : \N.\; \phi(n') \supset \phi(n'\mathord{+}1)) \mathrel{\supset} \phi(n)
\\
S \mathop{\subseteq} R & \forall n : \N, i : I.\; n \mathrel{S} i \mathrel{\supset} n \mathrel{R} i &
\Det(S) & \forall n : \N, i, i' : I.\; n \mathrel{S} i \mathrel{\wedge} n \mathrel{S} i' \mathrel{\supset} i =_I i'\\
\end{array}
\end{array}$%
\end{center}
\end{definition}

$\isnat$ is designed so that defining $n \approx_\N n'$ as $n =_\N n' \mathrel{\wedge} \isnat$ makes $\langle \N, \approx_\N \rangle$ a natural-number object in the constructed topos.


\begin{align*}
\interp{\Total\left(R\right)}^{T}
 &= \ttypprod{\typevar_n :\ttrkind{\N}} {\typecomp{\N \rightarrow \typecomp{\ttrtype{\scontext , \spred : \sort}{\exists i : I.\; n \mathrel{R} i}}}}\\
    \interp{\Total\left(R\right)}^{S}_{p} &= \tspeckinprod{\typevar_{n} : \ttrkind{\N}} \forall_{\tpred_{n} : \ttrind{\typevar_{n}}{\N} } .
        \after{\termtypeapp{\term}{\typevar_{n}}}{\termvar_{0}}{\tspectypprod{n : \N }{ \isnat \supset \after{\termapp{\term}{\termvar_{0}}}{\termvar_{2}}{\ttrspec{\scontext}{\exists i : I.\; n \mathrel{R}}{\termvar_{1}}}}}
\\
\interp{\Det\left(S\right)}^{T}
 &=  \interp{\forall n : \N, i, i' : I.\; n \mathrel{S} i \mathrel{\wedge} n \mathrel{S} i' \mathrel{\supset} i =_I i'}^{T}
 \\
    \interp{\Det\left(S\right)}^{S}_{p} &= 
    \\
    \interp{S \mathop{\subseteq} R}^{T}
 &=  \interp{\forall n : \N, i : I.\; n \mathrel{S} i \mathrel{\supset} n \mathrel{R} i}^{T} 
 \\
    \interp{S \mathop{\subseteq} R}^{S}_{p} &= 
\end{align*}

where:

\begin{align*}
    &\left\llbracket \exists_{i:I}.\left(n,i\right)\in R\right\rrbracket ^{T}&=\left\llbracket \forall_{P:\star}.\left(\forall_{i:I}.\left(\left(n,i\right)\in R\right)\rightarrow\overline{P}\right)\rightarrow\overline{P}\right\rrbracket ^{T}&=\prod_{X:*}M\left(\left(\prod_{X_{i}:\left\llbracket I\right\rrbracket ^{K}}M\left(X_{R}\left\llbracket \left(n,i\right)\right\rrbracket ^{t}\rightarrow MX\right)\right)\rightarrow MX\right)
\end{align*}

\begin{align*}
&\left\llbracket \exists_{i:I}.\left(n,i\right)\in R\right\rrbracket _{p}^{S}\\&=\left\llbracket \forall_{P:\star}.\left(\forall_{i:I}.\left(\left(n,i\right)\in R\right)\supset\overline{P}\right)\supset\overline{P}\right\rrbracket _{p}^{S}\\&=\cap_{X:*}\forall_{y:R_{X}}\left\langle x_{0}\leftarrow p\;X\right\rangle \left(\sqcap_{x_{1}:\left\llbracket \left(\forall_{i:I}.\left(\left(n,i\right)\in R\right)\supset\overline{P}\right)\right\rrbracket ^{T}}\left(\left\llbracket \left(\forall_{i:I}.\left(\left(n,i\right)\in R\right)\supset\overline{P}\right)\right\rrbracket _{x_{1}}^{S}\right)\supset\left\langle x_{2}\leftarrow x_{0}\;x_{1}\right\rangle \left(x_{2}\in y_{P}\right)\right)
\end{align*}

\begin{align*}
&\left\llbracket \left(\forall_{i:I}.\left(\left(n,i\right)\in R\right)\supset\overline{P}\right)\right\rrbracket _{x_{1}}^{S}\\&=\cap_{X_{i}:\left\llbracket I\right\rrbracket ^{K}}\forall_{y_{i}:\left\llbracket I\right\rrbracket _{X_{i}}^{I}}\left\langle x_{3}\leftarrow x_{1}\;X_{i}\right\rangle \left\llbracket \left(\left(n,i\right)\in R\right)\supset\overline{P}\right\rrbracket _{x_{2}}^{S}\\&=\cap_{X_{i}:\left\llbracket I\right\rrbracket ^{K}}\forall_{y_{i}:\left\llbracket I\right\rrbracket _{X_{i}}^{I}}\left\langle x_{3}\leftarrow x_{1}\;X_{i}\right\rangle \left(\sqcap_{x_{4}:X_{R}\ \left\llbracket \left(n,i\right)\right\rrbracket ^{t}}\left(\left(x_{4};\left\llbracket \left(n,i\right)\right\rrbracket ^{e}\in y_{R}\;\left\llbracket \left(n,i\right)\right\rrbracket ^{t}\right)\supset\left\langle x_{5}\leftarrow x_{2}\;x_{4}\right\rangle \left(x_{5}\in y_{P}\right)\right)\right)
\end{align*}



\begin{small}
\[\left\llbracket \text{CC}\right\rrbracket ^{T} = \prod_{X_{R}:\left\llbracket \mathbb{N}\times I\right\rrbracket ^{K}\rightarrow*}M\left(\left\llbracket \text{Tot}\left(R\right)\right\rrbracket ^{T}\rightarrow M\left(\prod_{X:*}\left(\prod_{X_{S}:\left\llbracket \mathbb{N}\times I\right\rrbracket ^{K}\rightarrow*}\left(M\left\llbracket \text{Tot}\left(S\right)\right\rrbracket ^{T}\times M\left\llbracket S\subseteq R\right\rrbracket ^{T}\times M\left\llbracket \text{Det}\left(S\right)\right\rrbracket ^{T}\right)\rightarrow MX\right)\rightarrow MX\right)\right) \]
\end{small}

\begin{align*}
&\left\llbracket \text{CC}\right\rrbracket _{p}^{S}\\&=\left\llbracket \forall R:N\times I\rightarrow\star.\text{Tot}\left(R\right)\supset\exists S:N\times I\rightarrow\star.\text{Tot}\left(S\right)\wedge S\subseteq R\wedge\text{Det}\left(S\right)\right\rrbracket _{p}^{S}\\&=\cap_{X_{R}:\left\llbracket N\times I\right\rrbracket ^{K}\rightarrow*}\forall_{y_{R}:\left\llbracket N\times I\rightarrow\star\right\rrbracket _{X_{R}}^{I}}\left\langle x_{0}\leftarrow p\;X_{R}\right\rangle \left(\sqcap_{x_{1}:\left\llbracket \text{Tot}\left(R\right)\right\rrbracket ^{T}}.\left\llbracket \text{Tot}\left(R\right)\right\rrbracket _{x_{1}}^{S}\supset\left\langle x_{2}\leftarrow x_{0}\;x_{1}\right\rangle \left\llbracket \forall_{P:\star}.\left(\left(\forall_{S:N\times I\rightarrow\star}\left(.\text{SubFun}\left(S,R\right)\supset\overline{P}\right)\right)\supset\overline{P}\right)\right\rrbracket _{x_{2}}^{S}\right)\\&=\cap_{X_{R}:\left\llbracket N\times I\right\rrbracket ^{K}\rightarrow*}\forall_{y_{R}:\left\llbracket N\times I\rightarrow\star\right\rrbracket _{X_{R}}^{I}}\left\langle x_{0}\leftarrow p\;X_{R}\right\rangle \left(\sqcap_{x_{1}:\left\llbracket \text{Tot}\left(R\right)\right\rrbracket ^{T}}.\left\llbracket \text{Tot}\left(R\right)\right\rrbracket _{x_{1}}^{S}\supset\left\langle x_{2}\leftarrow x_{0}\;x_{1}\right\rangle \left(\cap_{X_{P}:*}\forall_{y_{P}:R_{X}}\left\langle x_{3}\leftarrow x_{2}\;X_{P}\right\rangle \left(\sqcap_{x_{4}:\left\llbracket \left(\forall_{S:N\times I\rightarrow\star}\left(.\text{SubFun}\left(S,R\right)\supset\overline{P}\right)\right)\right\rrbracket ^{T}}\left\llbracket \forall_{S:N\times I\rightarrow\star}\left(\text{SubFun}\left(S,R\right)\supset\overline{P}\right)\right\rrbracket _{x_{4}}^{S}\supset\left\langle x_{5}\leftarrow x_{3}\;x_{4}\right\rangle \left(x_{5}\in y_{p}\right)\right)\right)\right)
\end{align*}

\begin{footnotesize}
\begin{align*}
&\left\llbracket \text{CC}\right\rrbracket _{p}^{S}\\&=\cap_{X_{R}}\forall_{y_{R}}\left\langle x_{0}\leftarrow p\;X_{R}\right\rangle \left(\sqcap_{x_{1}}.\left\llbracket \text{Tot}\left(R\right)\right\rrbracket _{x_{1}}^{S}\supset\left\langle x_{2}\leftarrow x_{0}\;x_{1}\right\rangle \left(\cap_{X_{P}}\forall_{y_{P}}\left\langle x_{3}\leftarrow x_{2}\;X_{P}\right\rangle \left(\sqcap_{x_{4}}\left\llbracket \forall_{S}\left(\text{SubFun}\left(S,R\right)\supset\overline{P}\right)\right\rrbracket _{x_{4}}^{S}\supset\left\langle x_{5}\leftarrow x_{3}\;x_{4}\right\rangle \left(x_{5}\in y_{p}\right)\right)\right)\right)
\end{align*}
\end{footnotesize}


\begin{align*}
&\left\llbracket \forall_{S:N\times I\rightarrow\star}\left(\text{SubFun}\left(S,R\right)\supset\overline{P}\right)\right\rrbracket _{x_{4}}^{S}\\&=\cap_{X_{S}:\left\llbracket N\times I\right\rrbracket ^{K}\rightarrow*}\forall_{y_{S}:\left\llbracket N\times I\rightarrow\star\right\rrbracket _{X_{s}}^{I}\left\langle x_{5}\leftarrow x_{4}\;X_{S}\right\rangle \left\llbracket \text{SubFun}\left(S,R\right)\supset\overline{P}\right\rrbracket _{x_{5}}^{S}}\\&=\cap_{X_{S}:\left\llbracket N\times I\right\rrbracket ^{K}\rightarrow*}\forall_{y_{S}:\left\llbracket N\times I\rightarrow\star\right\rrbracket _{X_{s}}^{I}\left\langle x_{5}\leftarrow x_{4}\;X_{S}\right\rangle \left(\sqcap_{x_{6}:\left\llbracket \text{SubFun}\left(S,R\right)\right\rrbracket ^{T}}\left\llbracket \text{SubFun}\left(S,R\right)\right\rrbracket _{x_{6}}^{S}\supset\left\langle x_{7}\leftarrow x_{5}\;x_{6}\right\rangle \left(x_{6}\in y_{p}\right)\right)}
\end{align*}

\begin{align*}
    &\left\llbracket \text{SubFun}\left(S,R\right)\right\rrbracket _{x_{6}}^{S}\\&=\left\llbracket \text{Tot}\left(S\right)\wedge S\subseteq R\wedge\text{Det}\left(S\right)\right\rrbracket _{\left(x_{t},x_{s},x_{d}\right)}^{S}\\&=\left(\left\langle x_{t}'\leftarrow x_{t}\right\rangle \left\llbracket \text{Tot}\left(S\right)\right\rrbracket _{x_{t}^{'}}^{S}\right)\wedge\left(\left\langle x_{s}'\leftarrow x_{s}\right\rangle \left\llbracket S\subseteq R\right\rrbracket _{x_{s}^{'}}^{S}\right)\wedge\left(\left\langle x_{d}'\leftarrow x_{d}\right\rangle \left\llbracket \text{Det}\left(S\right)\right\rrbracket _{x_{d}^{'}}^{S}\right)
\end{align*}

To axiomatize terms we use Leibniz equality:
\newcommand{\propeq}{\cong}
\[ \term_{1} \propeq_{\type} \term_{2}  \eqdef \tspecindprod{\exprsvar:\refpredN{\type}}{\left(\tmembase{\term_{1}}{\exprsvar}  \supset  \tmembase{\term_{2}}{\exprsvar}\right) \wedge \left(\tmembase{\term_{2}}{\exprsvar}  \supset  \tmembase{\term_{1}}{\exprsvar}\right)}   \]


\begin{definition}[Mem axiomatization]
    Let $MeM$ be the following set of axioms:
\agnote{We really need to allow support for pure functions}
The signature is parameterized by a type of results $I$.
\begin{enumerate}
    
    \item A type $\N$ of natural numbers (with the appropriate axioms)
    
    \item Product types (with the appropriate axioms)
    
    \item Unit type $\boldsymbol{1}$, with value $\left(\right)$
    
    \item A type constructor \agnote{or type operator?} $ \maybe : \typecon{\star}$ of option/maybe type (with the appropriate axioms)
    
    \item A type constructor \agnote{or type operator?} $S : \typecon{\star}$ of states

    \item An infinite type $L$ of locations
    
    \item State interface:
        \[ \interface : \typefun{L \times \N}{ \sum_{X : *} \left( \typecomp{\maybe\left(X\right)} \times \left(\typefun{\maybe\left(X\right)}{\typecomp{\boldsymbol{1}}}\right) \right) } \]        
    
    % \item State update:
    % \[ \update : \prod_{\typevar : \star} \typefun{\left(L \times \N\right) \times \maybe\left(\typevar\right)}{\typecomp{\boldsymbol{1}}} \]

    \item Location allocation:
    \[ \alloc : \typecomp{L} \]

    \item Update and Lookup standard axioms (for variables $i : L \times \N$, $j : L \times \N$, $\typevar : \star$, $x : \typevar$, and $y : \typevar$)
    \begin{align*}
        \termbind{ m_{x} }{ \lookup\left(i\right) }{ \termbind{ m_{y} }{ \lookup\left(i\right) }{ \termret{ \left(m_{x} , m_{y}\right)} } } &= \termbind{ m_{x} }{ \lookup\left(i\right) }{ \termret{\left(m_{x},m_{x}\right)} }\\
        \termbind{ m_{x} }{ \lookup\left(i\right) }{ \recmaybe{m_{x}}{x}{ \update\left(i,x\right) }{ \termret{\left(\right)} } } &= \termret{ \left(\right) }\\
        \termbind{\_}{\update\left(i,x\right)}{\lookup\left(i\right)} &= \termbind{\_}{\update\left(i,x\right)}{\termret{ \some\left(x\right) }}\\
        \termbind{\_}{ \update\left(i,x\right) }{ \update\left(i,y\right) } &= \update\left(i,y\right)\\
        i \neq j \quad \Rightarrow \termbind{m_{x}}{ \lookup\left(i\right) }{ \termbind{m_{y}}{ \lookup\left(j\right) }{ \termret{\left(m_{x} , m_{y}\right)} } }
    \end{align*}

    \item Axioms ensuring $L$ is finitely supported (only a finite amount of locations in $L$ has a defined lookup value:
    \begin{align*}
        \forall n : \N . \termbind{\termvar_{1}}{\alloc}{\termapp{\lookup}{ \pair{\termvar_{1}}{n}}} = \termret{ \nothing }\\
    \end{align*}
    
\end{enumerate}

The evidence for CC takes a realizer of totality and assigns a new location in $L$ (guaranteed to exist because of finite support), then uses it to memoize the results of the totality realizer, yielding a function.


\end{definition}


 \begin{small}
\[\left\llbracket \text{CC}\right\rrbracket ^{T} = \prod_{X_{R}:\left\llbracket \mathbb{N}\times I\right\rrbracket ^{K}\rightarrow*}M\left(\left\llbracket \text{Tot}\left(R\right)\right\rrbracket ^{T}\rightarrow M\left(\prod_{X:*}M\left(\prod_{X_{R}:\left\llbracket \mathbb{N}\times I\right\rrbracket ^{K}\rightarrow*}M\left(M\left\llbracket \text{Tot}\left(S\right)\right\rrbracket ^{T}\times M\left\llbracket S\subseteq R\right\rrbracket ^{T}\times M\left\llbracket \text{Det}\left(S\right)\right\rrbracket ^{T}\right)\rightarrow MX\right)\rightarrow MX\right)\right) \]
\end{small}

\[
\text{CC} = \termret{ \termabs{t}{ \ttrtype{a}{\Total\left(R\right)} }{\termret{ \termabs{k}{ M\left(\prod_{X_{R}} M\left( \cdots \right) \rightarrow MX\right) }{ \termbind{k'}{k}{ \termapp{k'}{ \termret{\left( \mathsf{tot}_{S}\left(t\right) , \mathsf{sub}_{S} , \mathsf{det}_{S} \right)} } } } }} }
\]

\[ \mathsf{tot}_{S}\left(t\right) = \termbind{l_{0}}{\alloc}{ \termret{\termret{ \termabs{ n }{ \N }{ \termret{ \lambda k . \termbind{k'}{k}{ \termapp{k}{ e_{t,l_{0},n} } } } } } }} \]

\[\interp{\Total\left(R\right)}^{T}
 = \ttypprod{\typevar_n :\ttrkind{\N}} {\typecomp{\typefun{\N}{  \typecomp{  \ttypprod{\typevar :\star}{ \typecomp{ \typefun{\left(\ttypprod{\typevar_{i} :\ttrkind{I}}{ \typecomp{ \typefun{ \typevar_{R} \; \ttretype{}{\left(n,i\right)}{}  }{\typecomp{\typevar}}  } }\right)}{\typecomp{\typevar}} }  }}}}}\]

\begin{align*}
    &e_{t,l_{0},n}\\
    &=\termbind{ m_{i} }{ \lookup\left(l_{0},n\right) }{}\\
    &\recmaybe{m_{i}}{i}{ \termret{i} }{ \termbind{t'}{t}{ \termbind{ r }{ \termapp{t'}{n} }{ \termbind{t''}{ \termtypeapp{t'}{\typevar} }{ \termbind{ r' }{ \termapp{r}{\termret{ \lambda p . \termret{p} }} }{  \termbind{\_}{ \update\left(\left(l_{0},n\right),\some\left(r\right)\right) }{ \termret{r} } } } } } }
\end{align*}

\begin{align*}
e_{t,l_{0},n}=&m_{i}\leftarrow\text{lookup}\left(l_{0},n\right);\\&m_{i}\ \left(\text{some}\left(i\right)\mapsto\left[i\right];\text{none}\mapsto\left(t'\leftarrow t;r\leftarrow t'\;n;\text{update}\left(\left(l_{0},n\right),r\right);\left[r\right]\right)\right)
\end{align*}

\begin{definition}[Countable Choice]
Given a type $\type$
\[ \sforall{\spred_{1} : \predcon{\N \times \type}}{\simplies{ \totrel\left(\spred_{1}\right) }{ \sexists{\spred_{2} : \predcon{\N \times \type}}{\sconj{\left(\spred_{2} \subseteq \spred_{1}\right)}{\sconj{\detrel\left(\spred_{2}\right)}{\totrel\left(\spred_{2}\right)}}} }}  \]
\end{definition}



\lcnote{extension/instantiation}

\newcommand{\monadmorph}{\beta}

\begin{definition}[Monad Morphism]
A parametric function:
\[ \monadmorph :  \ttypprod{\typevar:\star}{\typefun{M\left(\typevar\right)}{N\left(\typevar\right)}} \]

\begin{align*}
    \monadmorph\left(\termret{p}_{M}\right) &\propeq_{N\left(\type\right)} \termret{p}_{N}\\
    \monadmorph\left(\left[\termbind{\termvar}{\term_{1}}{\term_{2}}\right]_{M}\right) &\propeq_{N\left(\type\right)} \left[\termbind{\termvar}{\monadmorph\left(\term_{1}\right)}{\monadmorph\left(\term_{2}\right)}\right]_{N}
\end{align*}

\end{definition}

A monad morphism from $M$ to $N$, allows you to transform any $N$-modality $\left(\after{\term}{\termvar}{\tprop}\right)_{N}$ (where $p : N\left(\type\right)$ for some type $\type$) into an $M$-modality:
\[ \left(\after{\monadmorph\left(\term\right)}{\termvar}{\tprop}\right)_{N} \]
(where $p : M\left(\type\right)$)

Given a monad morphism, and evidence $\term : \typefun{\type_{1}}{M\left(\type_{2}\right)}$ for some proposition $\tprop$, the function $\monadmorph \circ \term : \typefun{\type_{1}}{N\left(\type_{2}\right)}$ is an evidence for $\tprop$ when the following holds \agnote{this is an example for one argument, need to generalize to an arbitrary number of arguments}:
\[
\elsequent{\context , \termvar_{1} : \type_{1}}{\left(\after{\termapp{\term}{\termvar_{1}}}{\termvar}{\tprop}\right)_{M} }{ \left(\after{\termapp{\left(\monadmorph \circ \term\right)}{\termvar_{1}}}{\termvar}{\tprop}\right)_{N} }
\]


% \section*{Pairs}
% \input{section/OldpairExm}

==> section/Fw.tex <==

\subsection[Deductive System F-omega]{Deductive System F$\omega$}

==== COPY ====

\agnote{Use more intuition and words, less technical details. Show for a concrete interesting example instead of a general definition}
Deductive System F$\omega$ combines the propositions of higher-order logic with the types of System F$\omega$, using the types as sorts and making all the propositions depend type operator variables in addition to term variables, and the types of the term variables can depend on the type operator variables.

Deductive System F$\omega$ has a set of kinds $\boldsymbol{Kind}$, and type operators. Each type operator has a kind of the form $\left(\kappa_{1} , \ldots , \kappa_{n}\right) \Rightarrow \star$, meaning it takes type operators of kind $\kappa_{1}$ to $\kappa_{n}$ as arguments to produce a type.
Concrete types have the kind $\left(\right) \Rightarrow \star$, meaning they take no arguments, which can also be written as simply $\star$.

A \emph{kind context}, often marked as $\Delta$, is a list of kinded variables $\left[ \sigma_{1} : \kappa_{1} , \ldots , \sigma_{n} : \kappa_{n} \right]$ where the $\sigma_{i}$ are variables, denoting type operators, each with its assigned kind $\kappa_{i}$.

Each kind context $\Delta$ has its corresponding set of types $\typ{\Delta}$, where all the free type operator variables appear in $\Delta$.

Given a kind context $\Delta$, \emph{type context} over $\Delta$, often marked as $\Gamma_{\Delta}$, is a list of typed variables $\left[ x_{1} : \sigma_{1} , \ldots , x_{n} : \sigma_{n} \right]$ where the $x_{i}$ are variables, denoting terms, each with its assigned type $\sigma_{i}$ taken from $\typ{\Delta}$.

To reason about programs, for each kind context $\Delta$ and each type context $\Gamma_{\Delta}$ over $\Delta$, there is a set $\spec{\Delta}{\Gamma_{\Delta}}$ of \emph{refinements}, defined as the set of propositions in higher-order logic.

The realizability translation we present translates propositions of higher-order logic to refinements of Deductive System F$\omega$.

By abuse of notation, we extend the sort translations to translate contexts: The sort to kind translation is extended to translate sort contexts to kind contexts, and the sort to type translation is extended to translate sort contexts to type context:
\begin{align*}
\trkind{x_{1} : \sigma_{1} , \ldots , x_{n} : \sigma_{n} } &:= \alpha_{x_{1}} : \trkind{\sigma_{1}} , \ldots , \alpha_{x_{n}} : \trkind{\sigma_{n}}\\
\trind{\alpha_{1} : \kappa_{1} , \ldots , \alpha_{n} : \kappa_{n} }{x_{1} : \sigma_{1}, \ldots , x_{n} : \sigma_{n} } &:= \widehat{x_{1}} : \trind{\alpha_{1} : \kappa_{1}}{\sigma_{1}} , \ldots , \widehat{x_{n}} : \trind{\alpha_{n} : \kappa_{n}}{\sigma_{n}} 
\end{align*}
From now on, we'll use the notation:
\[ 
\Delta_{\Sigma} := \trkind{\Sigma}
\qquad
\Gamma_{\Sigma} :=
\trind{\Delta_{\Sigma}}{\Sigma}
\]
The translation functions are defined by mutual recursion:
\begin{table}[H]
\begin{tabular}{ll}
$\trkind{-} : \mathcal{U} \rightarrow \boldsymbol{Kind}$ &
  $\trind{-}{-} : \prod_{\sigma \in \mathcal{U}} \prod_{\alpha \in \kvar{\trkind{\sigma}}} \typ{\alpha : \trkind{\sigma} }$
   \\
$\trtype{\Sigma}{-} : \prop{\Sigma} \rightarrow \typ{\Delta_{\Sigma}}$ &
  $\trspec{\Sigma}{-} : \prod_{\varphi \in \prop{\Sigma}} \spec{\Delta_{\Sigma}}{\Gamma_{\Sigma} , c : \trtype{\Sigma}{\varphi}}$
\end{tabular}
\end{table}
For the sorts, we consider only the sort of predicates, recursively assigning each predicate with a type constructor\agnote{\textbf{operator}} for the type of its realizers:
\begin{align*}
    \trkind{\pred{\sigma_{1} , \ldots , \sigma_{n}}} &:= \left(\trkind{\sigma_{1}} , \ldots , \trkind{\sigma_{n}}\right) \Rightarrow \star\\
    \trind{\alpha : \left(\kappa_{1} , \ldots , \kappa_{n} \right) \Rightarrow \star}{\pred{\sigma_{1} , \ldots , \sigma_{n}}} &:= \prod_{\alpha_{1} : \kappa_{1} , \ldots , \alpha_{n} : \kappa_{n}  } \mathsf{Ref}_{\alpha\left( \alpha_{1} , \ldots , \alpha_{n} \right)}\left(\trind{\alpha_{1} : \kappa_{1}}{\sigma_{1}} , \ldots , \trind{\alpha_{n} : \kappa_{n}}{\sigma_{n}} \right)
\end{align*}
% \[ \trkind{\pred{\sigma_{1} , \ldots , \sigma_{n}}} := \left(\trkind{\sigma_{1}} , \ldots , \trkind{\sigma_{n}}\right) \Rightarrow \star \]
% \[ \trind{\alpha : \left(\kappa_{1} , \ldots , \kappa_{n} \right) \Rightarrow \star}{\pred{\sigma_{1} , \ldots , \sigma_{n}}} := \prod_{\alpha_{1} : \kappa_{1} , \ldots , \alpha_{n} : \kappa_{n}  } \pred{\trind{\alpha_{1} : \kappa_{1}}{\sigma_{1}} , \ldots , \trind{\alpha_{n} : \kappa_{n}}{\sigma_{n}} , \alpha\left( \alpha_{1} , \ldots , \alpha_{n} \right) } \]
Each proposition is assigned with the type of its realizers, by recursion over the logical constants:
\begin{align*}
    \trtype{\Sigma}{\varphi_{1} \supset \varphi_{2}} &:= \trtype{\Sigma}{\varphi_{1}} \Rightarrow \trtype{\Sigma}{\varphi_{2}}\\
    \trtype{\Sigma}{\forall_{x : \sigma} . \varphi} &:= \trtype{\Sigma , x : \sigma}{\varphi}\\
    \trtype{\Sigma}{ \tmem{\left(p_{1} , \ldots , p_{n}\right)}{p} {?}} &:= \alpha_{p} \left(\alpha_{p_{1}} , \ldots , \alpha_{p_{n}}\right)
\end{align*}
The realizability conditions are described for each logical constant as refinements over the corresponding realizer:
\begin{align*}
    \trspec{\Sigma}{\varphi_{1} \supset \varphi_{2}}\left[f\right] &:= \forall_{c : \trtype{\Sigma}{\varphi_{1}} } . \trspec{\Sigma}{\varphi_{1}}\left[c\right] \supset \trspec{\Sigma}{\varphi_{2}}\subst{f\left(c\right)}\\
    \trspec{\Sigma}{\forall_{x : \sigma} . \varphi}\left[y\right] &:= \forall_{x : \trind{\alpha_{x} : \trkind{\sigma}}{\sigma}} .
    \trspec{\Sigma , x:\sigma}{\varphi}\subst{x,y}\\
    \trspec{\Sigma}{ \tmem{\left(p_{1} , \ldots , p_{n}\right)}{p} {?}}\subst{c} &:= \tmem{\left(\widehat{p_{1}} , \ldots , \widehat{p_{n}} ; c\right)}{\widehat{p}}{?}
\end{align*}

======

==> section/MCA.tex <==
\subsection{Monadic Combinatory Algebras}
Standard realizability models of Higher-Order logic are standardly constructed from a partial combinatory algebra (PCA).
%
One key feature of PCAs is that they are partial, meaning that the application of a program to an input is a partial operator, \ie not all inputs are guaranteed to produce valid outputs. 
%
This means that PCA offers inherent support for non-termination as a computational effect, but other useful effects, such as nondeterminism, stateful computation or exceptions, are not directly supported by PCA. 
% 
Such effects can be modeled by PCAs, usually by incorporating additional structures or operations into the underlying algebraic framework, such as in PCAs with errors (PCAE),  with choice (PCAC), with partiality and exceptions (PCAX) \cite{cohen2019effects,cohen2021evidenced}.
This section aims to introduce computational effects other than termination directly into combinatory algebra in the same natural manner as termination is embedded in the definition of PCA.
%
For this generalization we employ the standard structure for describing and reasoning about general effects: monads~\cite{moggi1991notions}. 
Using this categorical model has the benefit of preserving many useful properties of functions while allowing a wider variety of models.
%
Roughly speaking, monads are used to relate a computational effect with a specific functor, say $M$, and consider effectful programs that return results of type $A$ as generalized elements of the object $M\left(A\right)$.
A \emph{generalized element} of an object $Y$ in category $\C$ is a morphism $f \in \hom{\C}{X}{Y}$ for some object $X$.
A \emph{monad} $M$ over category $\C$ is a functor $M : \C \rightarrow \C$ s.t generalized elements of the form $\hom{\C}{A}{M\left(B\right)}$ for arbitrary objects $A,B \in \obj{\C}$ are composable.
When $M$ is a monad, morphisms of the form $\hom{\C}{A}{M\left(B\right)}$ (for arbitrary $A , B \in \obj{\C}$) form a category, called the \emph{Kleisli category}\lcnote{CITE}.


Accordingly, we define the notion of Monadic Combinatory Algebras, which generalizes the notion of a PCA, but instead of partial computation, exhibits a computational effect encapsulated behind a monad.
Concretely, just as Partial Applicative Structures describe the application as a \emph{partial} operator, the following definition describes the application as an \emph{effectful} operator, parameterized by some $\mathbf{Set}$ monad.

\begin{definition}[Monadic Applicative Structure]
Given a $\mathbf{Set}$ monad $M$, a \emph{Monadic Applicative Structure}  over $M$ is an set of ``codes''
$\mca$ together with an application Kleisli function:
\[\left(-\right)\app\left(-\right) : \mca\times\mca \rightarrow M\mca\]
\end{definition}

We think of $\left(-\right)\app\left(-\right)$ as a function which takes two codes and returns a ``computation'' of a code.
%
To ensure the model can do general computation, we want it to be at least as computationally powerful as the $\lambda$-calculus.
There are various different but equivalent approaches to do so, we will use the following. 
First, we define terms over $\mca$ with variables and substitution, by natural extension of the grammar of PCAs.
%Given a \emph{MAS} $\mca$, the set $E_{n}\left(\mca\right)$
%of \emph{terms over }$\mca$ is defined by the grammar:
%\[
%\hfill
%e \ ::= \  0 \ | \  \ldots \ | \  n-1 \ | \  c \in \mca \ | \  e \app e
%\hfill
%\]
%
%Given a term $e \in E_{n+1}\left(\mca\right)$ and a code $c\in\mca$, their 
%\emph{substitution} $e\left[c\right] \in E_{n}\left(\mca\right)$ is defined inductively by:
%
%\begin{center}
%	\begin{tabular}[H]{|c|c|} 
%		\hline
%		$e$ & $e\left[c_{a}\right]$ \\ 
%		\hline
%		$0$ & $c_{a}$ \\ 
%		$i+1$ & $i$ \\
%		$c$ & $c$ \\
%		$e_{f} \app e_{a}$ & $e_{f}\left[c_{a}\right] \app e_{a}\left[c_{a}\right]$ \\
%		\hline
%	\end{tabular}
%\end{center}
Then, we define the evaluation of closed terms as follows.
For closed terms in $E_{0}\left(\mca\right)$ we define an \emph{evaluation} Kleisli operator
\[
\nu :E_{0}\left(\mca\right)\rightarrow M\left(\mca\right)
\]
which, when given a term, ``computes'' the ``value'' of the term.
%
Evaluation is defined by induction on $E_{0}\left(\mca\right)$ (using do-notation):
%
\[\nu\left(c\right) :=\eta\left(c\right)
\qquad\qquad
\nu\left(e_{f}\app e_{a}\right) :=\text{do}\ c_{f}\leftarrow\nu\left(e_{f}\right)\ ;\ c_{a}\leftarrow\nu\left(e_{a}\right)\ ;\ c_{f} \app c_{a}
\]

Lastly, we define an \emph{abstraction} operator that turns open terms into codes which ``internalize'' their evaluation after substitution.

\begin{definition}[Monadic Combinatory Algebra]\label{mca}
A Monadic Combinatory Algebra (MCA) is a monadic applicative structure $\mca$ with 
an abstraction operator  for each $n\in\mathbb{N}$ 
\[
\encode{n}{\left(-\right)} :E_{n+1}\left(\mca\right)\rightarrow\mca
\]
such that:
$$\begin{array}{@{}ll}
	\forall n.\forall e \in \Expr{n+2}.\forall c. & \encode{n+1}{e} \app c = \eta \left( \encode{n}{e[c]} \right) \\
	\forall e \in \Expr{1}.\forall c. & \encode{0}{e} \app c = \nu \left( e[c] \right)
\end{array}$$
\end{definition}

%Note the similarity to the definition of a PCA:
%$$\begin{array}{@{}ll}
%\forall n.\forall e \in \Expr{n+2}.\forall c_a. & \encode{n+1}{e} \app c_a \downarrow \encode{n}{e[c_a]} \\
%\forall e \in \Expr{1}.\forall c_a, c_r. & \encode{0}{e} \app c_a \downarrow c_r \iff e[c_a] \downarrow c_r
%\end{array}$$

Principally, the MCA laws state that the abstraction operator ``delays'' the evaluation of an open term it encloses until all the free variables in it are substituted by a code.
Whenever there is more than one free variable in the term, using $\eta$ means the application of the abstracted term to a code only substitutes the outermost parameter with the argument.
However,  when there is precisely one free variable in the term,  substituting it with the argument obtains a closed term, which will then immediately be evaluated. 

To relate the semantics of computational effects (monads) with the semantics of logic (hyperdoctrines\lcnote{cite}), we define a notion we call \emph{oplax post-module}.
Concretely, this notion is used to interpret specifications involving modality.
%
Oplax post-modules, when defined in the context of a hyperdoctrine with inverse image functor $\P$ with a monad $M$, ``lift'' formulas over values in $\P\left(A\right)$ to formulas over computations in $\P\left(M\left(A\right)\right)$.
It can be considered as a way to turn a pure proposition into a post-condition on the result of a computation.
The laws of an oplax post-module ensure that post-conditions are preserved through entailment by introducing the basic operations of the monad.
\begin{definition}[Oplax Post-Module]
Given a monad $\monad$ over category $\indcat$, an oplax post-module for $\monad$ is a pair $\left( \P , \module \right)$ where $\P : \indcat \rightarrow \opcat{\preordcat}$ is a functor, and $\module : \P \circ \monad \Rightarrow \P$ is a natural transformation which satisfies the following conditions, for any $\object \in \obj{\indcat}$ and $\varphi \in \P\left(\object\right)$:
$$
\varphi \leq \P{\eta} \left( \module \left( \varphi \right) \right) 
\qquad ; \qquad 
\module \left( \module \left( \varphi \right) \right) \leq \P{\mu} \left( {\module} \left( \varphi \right) \right)
$$
\end{definition}

\begin{comment}
    
\subsubsection{MCA Examples}
~\\
The notion of MCA subsumes many common combinatory algebras suggested in the literature. Below we review some and show which monad allows us to instantiate the specific case. 

% \agnote{TODO: describe examples}
% \emnote{will do}
% 	\begin{itemize}
% 		\item[ok] PCA
% 		\item Bauer parameterized realizability as a special case (ParCA)
% 		\item RCAs, SCAs, Computational Systems...
% 		\item Ross had a probability example we can look into \agnote{Giry's monad?}
% 		\item continuations?
% 	\end{itemize}

\paragraph{Partial Combinatory Algebra}
The notion of an MCA is a generalization of a PCA, and the laws of a PCA are precisely the MCA laws when the monad is the sub-singleton monad, i.e.  $M A$ is the set of subsets of $A$ in which all elements are equal:
\[M A = \{X\subseteq A \mid \forall x,y\in X. x = y \}
 \qquad
 \eta_A:x\mapsto \{x\}
 \qquad
 \mu_A:\mathbb{X}\mapsto \bigcup_{X\in\mathbb{X}} X
\]


==== COPY ====
 
\paragraph{Relational Combinatory Algebra}

Relational Combinatory Algebras (RCAs) were defined in~\cite{cohen2019effects,cohen2021evidenced}
to account for demonic non-determinism.
RCAs correspond to an MCA with $M$ being the \textbf{powerset} monad:
\[
 M A = \P(A) 
 \qquad\qquad 
 \eta_A: x \mapsto \{x\}
 \qquad\qquad
 \mu_A:\mathbb{X}\mapsto \bigcup_{X\in\mathbb{X}} X
\]


\paragraph{Stateful Combinatory Algebra}
In \cite{cohen2019effects,cohen2021evidenced},
the authors defined Stateful Combinatory Algebras (SCAs) as a stateful extension of RCAs, 
which can in particular be used to memoize non-deterministic
computations and recover a realizer of Countable Choice even in the presence
of nondeterminism.
Again, an SCA is a particular case of MCA, with $M$ being 
the \textbf{transformer} of the \textbf{increasing state} monad (for a 
given set of states $\Sigma$) over the \textbf{powerset} monad:
\[
 \begin{array}{l}
 M A = \left\{ u:\Sigma\rightarrow \P\left(\Sigma\times A\right)\
 \mid\ \forall\sigma_{0}\in\Sigma.\forall\left(\sigma_{1},x\right)\in u\left(\sigma_{0}\right).\sigma_{0}\leq\sigma_{1}\right\}\\[.5em]
 
 \eta_A(x)(\sigma):= \{(\sigma,x)\}
 \qquad\qquad
 \mu_A(u)(\sigma):=\bigcup_{(\sigma',f)\in u(\sigma)}f(\sigma)
\end{array}
\]


\paragraph{Bauer?}

\paragraph{CPS?}

\paragraph{CbV/CbN}


\lcnote{probability example as a new one?}


\subsubsection{modeling MCAs}

Monadic Combinatory Algebras with an Effectful Tripos \agnote{future reference} is the same as a model of $\effhol$ where there is some type $\mca$ equal to its type of endofunctions ($\mca = \mca \rightarrow \mca$).




=======
\end{comment}


==> section/MCAmodel.tex <==
\lcnote{Can we ? Fingers crossed!}
This section provides a semantic account for $\effhol$. 

Here, we aim to generalize than construction to obtain models that support computational effects other than just non-termination. 
We do so by introducing a notion of Monadic Combinatory Algebra (MCA), which extends the notion of a PCA, based on incorporating effects through a monad. 

\input{section/MCA}

\begin{definition}[Interpretation]

\input{section/figures/MCAinter}

Kinds are completely ignored.?\\
\textbf{Kinds:}\\
$\mcatype{\star}=\mathcal{U}$ 
\qquad\qquad
$\mcatype{\kind\to \star}=\mathcal{U}^{\mcatype{\kind}}$
where $\mathcal{U} = \left\{ \monad^{\left(n\right)}\left(\mca\right) \mid n \in \mathbb{N} \right\}$
\\


Valuation $\rho$: variable -> $\mathbb{K}$

\textbf{Types}\\
$\mcatype{\type:\kind} \in \mcatype{\kind}$


$: ? \rightarrow \left\{ \monad^{\left(n\right)}\left(\mca\right) \mid n \in \mathbb{N} \right\}$

Types are interpreted by:
\begin{align*}
    \mcatype{\typevar}_\theta &:=  \theta(\typevar)\\
    % \mcatype{\typevar} &:= \monad\left(\mca\right) \\
    \mcatype{\typeapp{\type_1}{\type_2}}_\theta &:= \mcatype{{\type_1}}_\theta(\mcatype{\type_2}_\theta)\\
    % \mcatype{\typeabs{\typevar}{\kind}{\type}}_\rho &:= \{f:\P(E(\mca))^{\mcatype{\kind}} \mid \forall x\in\mcatype{\kind}, \forall e\in x, f(e)\in \mcatype{\type}_{\rho,X\leftarrow x}
    % \}\\
    % \mcatype{\typeabs{\typevar}{\kind}{\type}}_\theta &:= \lambda U . \mcatype{\typevar}_{\theta , X \leftarrow U}
    \mcatype{\typeabs{\typevar}{\kind}{\type}}_\theta &:= \lambda U . \mcatype{\type}_{\theta , X \leftarrow U} 
    \\
    % \mcatype{\typefun{\type_1}{\typecomp{\type_2}}}_\theta &:= \{ c \in E(\mca) \mid \forall e_1\in\mcatype{\type_1}. c\cdot e_1 \in\mcatype{\typecomp{\type_2}}\} \\
    \mcatype{\typefun{\type_1}{\typecomp{\type_2}}}_\theta &:= \left\{ c \mid \forall c_{1} \in \mcatype{\type_{1}}_{\theta} . c \cdot c_{1} \in \mcatype{\type_{2}}_{\theta}  \right\} \\
    \mcatype{\ttypprod{\typevar:\kind}{\type}}_\theta &:= \bigcap_{U\in \mcatype{\kind}}\mcatype{\type}_{\theta, X\leftarrow U} \\
    % \mcatype{\typecomp{\type}}_\theta &:= \{e\in E(\mca) \mid c\leftarrow \nu(e);c\in\mcatype{\type}_{\theta}\}
    % \mcatype{\typecomp{\type}}_\theta &:= \{e\in E(\mca) \mid c\leftarrow \nu(e);c\in\mcatype{\type}_{\theta}\}
    \mcatype{\typecomp{\type}}_\theta &:= \monad\left(\mcatype{\tau}_{\theta}\right)
\end{align*}




=========Etienne=========

$\mcatype{\star}=\P(\nu(M(\mca)))$ 
\qquad\qquad
$\mcatype{\kind\to \star}=\P(\P(M(\mca))^{\mcatype{\kind}})$
\qquad\qquad
$\mathbb{K} = \bigcup_{\kind}\mcatype{\kind}$\\


Types are interpreted by:
\begin{align*}
    \mcatype{\typevar} &:= \monad\left(\mca\right) \\
        \mcatype{\typeapp{\type_1}{\type_2}}_\theta &:= \mcatype{{\type_1}}_\theta(\mcatype{\type_2}_\theta)\\
    \mcatype{\typeabs{\typevar}{\kind}{\type}}_\rho &:= \{f:\P(E(\mca))^{\mcatype{\kind}} \mid \forall x\in\mcatype{\kind}, \forall e\in x, f(e)\in \mcatype{\type}_{\rho,X\leftarrow x}
    \}\\
        \mcatype{\typefun{\type_1}{\typecomp{\type_2}}}_\theta &:= \{ c \in E(\mca) \mid \forall e_1\in\mcatype{\type_1}. c\cdot e_1 \in\mcatype{\typecomp{\type_2}}\} \\
        \mcatype{\ttypprod{\typevar:\kind}{\type}}_\theta &:= \bigcap_{U\in \mcatype{\kind}}\mcatype{\type}_{\theta, X\leftarrow U} \\
    \mcatype{\typecomp{\type}}_\theta &:= \monad\left(\mcatype{\type}_{\theta}\right)
    % \{\nu\left(e\right)\in E(\mca) \mid
    % \nu\left(e\right) \in \rho\left(\mcatype{\type}_{\theta}\right)\}
\end{align*}
===================

Programs are interpreted by expressions in the corresponding interpretation of the type (in $E(\mca)$)

\newcommand{\rhop}{{\rho_\mathrm{p}}}
Valuation $\rhop$ : $(x:\type)\to \mcatype{\type}_{}$

\begin{align*}
    \mcaterm{\rhop}{\tcontext}{\termvar} &:=\rhop(x) \\
    \mcaterm{\rhop}{\tcontext}{\termtypeabs{\typevar}{\kind}{\term}} &:= \mcaterm{\rhop}{\tcontext}{\term}\\
    \mcaterm{\rhop}{\tcontext}{\termtypeapp{\term}{\type}} &:= \mcaterm{\rhop}{\tcontext}{\term}\\
    \mcaterm{\rhop}{\tcontext}{\termabs{\termvar}{\type}{\term}} &:=\lambda z. \mcaterm{\rhop,\termvar\leftarrow z}{\tcontext}{\termvar} \text{\emnote{should be with De Bruijn}}\\
    \mcaterm{\rhop}{\tcontext}{\termapp{\term_1}{\term_2}} &:= \mcaterm{\rhop}{\tcontext}{\term_1}\cdot \mcaterm{\rhop}{\tcontext}{\term_2}\\
    \mcaterm{\rhop}{\tcontext}{\termret{\term}} &:= \eta(\mcaterm{\rhop}{\tcontext}{\term})\\
    \mcaterm{\rhop}{\tcontext}{\termbind{\termvar}{\term_1}{\term_2}} &:=
    \text{do}\ c\leftarrow\nu(\mcaterm{\rhop}{\tcontext}{\term_1}) ;\ \mcaterm{\rhop,x\leftarrow c}{\tcontext}{\term_2}
\end{align*}




Index
\begin{align*}
       \interptype{\kcontext}{\refpredN{\type}} & :=  
            \\
            \interptype{\kcontext}{\refpred{\type}{\indice}} & :=  
            \\
             \interptype{\kcontext}{\tindprod{\typevar:\kind}{\indice}} & :=  
\end{align*}

Expressions


specification



\end{definition}


% &
% \begin{array}{l@{\hspace{-0.5in}}llll}
% \textbf{Indices} &&&&\\
%             & \indice 
%             & ::=  & \refpredN{\type} & \mbox{(null refinement)}%\lcnote{where is it used?}}
%             \\
%             & &\mid  & 
%             \refpred{\type}{\indice} & \mbox{(refinement)}
%             \\
%             & &\mid  & \tindprod{\typevar:\kind}{\indice}  & \mbox{(universal) }
%             \\[\myskip]
            
% \textbf{Expressions} &&&&\\
%             & \exprs
%             & ::=  & \epred & \mbox{(variable)}
%             \\
%             && \mid  &\ecomp{\termvar}{\type}{\exprsvar}{\indice}{\tprop}
%             & \mbox{(comprehension)}\\
%             &&\mid & \eforall{\typevar:\kind}{\exprs} & \mbox{(type abstraction)}\\
%             &&\mid & \eapp{\exprs}{\type} & \mbox{(type application)}\\
%             \\[\myskip]

% \textbf{Specifications} &&&&\\
%             & \tprop 
%             & ::=  & \tmem{\term}{\exprs}{\langle \exprs\rangle} & \mbox{(membership)}
%             \\
%             & &\mid & \timplies{ \tprop }{ \tprop } & \mbox{(implication)}
%             \\
%             & &\mid &  \after{\term}{\termvar}{\tprop}  & \mbox{(modality)}
%             \\
%             & &\mid & \tspeckinprod{\typevar:\kind}{\tprop} & \mbox{(type uni.)}
%             \\
%             & &\mid & \tspectypprod{\termvar:\type}{\tprop} & \mbox{(program uni.)} 
%             \\
%             & &\mid &  \tspecindprod{\epred:\indice}{\tprop} & \mbox{(expression uni.)} 
%              \\[\sskip]
%             % \\[\sskip]
%             % \\[\sskip]
% \\

==> section/PCA.tex <==
\subsection{Partial Combinatory Algebras}

Next, we show how perhaps the most standard approach to realizability semantics, using partial combinatory algebras (PCAs) to construct realizers, is captured by our framework. 
%A standard approach to realizability semantics is to construct realizers by using partial combinatory algebras. The following realizability translation is the standard construction, presented as an special case of the more general approach of this paper.
%

The definition of partial combinatory algebra is based on  \emph{partial applicative structures}.
%
%\begin{definition}[Partial Applicative Structure]
A partial applicative structure is a set $\mca$ of ``codes'' equipped with a partial binary ``application'' operator on $\mca$.
%\[ \left(-\right) \cdot \left(-\right) : \mca \times \mca \rightharpoonup \mca \]
%
We use~$c_f \app c_a \downarrow c_r$ to denote $c_r$ being the (successful) result of the application~$c_f \app c_a$, and  $c_{f} \cdot c_{a} \in S$ to denote that there is a code $c_{r} \in S$ such that $c_{f} \cdot c_{a} \downarrow c_{r}$.
%For any two codes $c_{f}$ and $c_{a}$, the expression $c_{f} \cdot c_{a} \downarrow$ is used to say the application $c_{f} \cdot c_{a}$ is defined, and $c_{f} \cdot c_{a} \downarrow c_{r}$ is used to say $c_{f} \cdot c_{a}$ is defined and equal to $c_{r}$.
%\end{definition}

%From now on, for any two codes $c_{f} , c_{a} \in \mca$ and any set $S$, the notation $c_{f} \cdot c_{a} \in S$ will be used to denote that there is a code $c_{r} \in \mca$ such that $c_{f} \cdot c_{a} \downarrow c_{r}$ and $c_{r} \in S$.

%Semantically, the application operator takes a code $c_{f}$, denoting some program, and a code $c_{a}$, and then runs the program represented by $c_{f}$ on $c_{a}$ as an input, yielding $c_{f} \cdot c_{a}$ as a result.
%The partiality of the application operator allows this execution to never terminate. If the execution does terminate, and yields the code $c_{r}$ as a result, it is expressed by the judgement $c_{f} \cdot c_{a} \downarrow c_{r}$.

A PCA is then defined as a partial applicative structure that is ``functionally complete'', meaning there is a way to encode application expressions 
%(such as $(c_1 \app (c_2 \app c_3)) \app (c_4 \app c_5)$) 
with $n$~free variables as individual codes accepting $n$~arguments through applications. 
That is, we ensure that every formal expression involving variables, codes, and application, can be ``internalized'' in a similar vein to the abstraction done in $\lambda$-calculus.
%
This ensures the necessary expressiveness for modeling computational systems like the $\lambda$-calculus.
%Given a partial applicative structure, one can consider application ``expressions'' such as $(c_1 \app (c_2 \app c_3)) \app (c_4 \app c_5)$.
%%, meaning $c_1 \app c_2 \app c_3$ is shorthand for $(c_1 \app c_2) \app c_3$).
%A partial combinatory algebra is a partial applicative structure that is ``functionally complete'', meaning there is a way to encode such expressions with $n$~free variables as individual codes accepting $n$~arguments through applications.
%
To present the formal definition, we first formalize expressions~$e$ with numbered free variables~$i \in \mathbb{N}$, substitution~$e[c_a]$, and the extension of evaluation to expressions~$e \downarrow c_r$.
To make the formalism easier to mechanize, we opt for lexical addresses (DeBruijn notation), rather than nominal variables.
Lexical addresses are numbers representing the index of a formal parameter within the body of a bound expression.
For example, given a function $f(x_{0},x_{1},x_{2})$, $2$ is the lexical address of $x_{2}$ because it is the third parameter, so instead of writing $x_{2}$ within the body of $f$, one can use the number $2$.
%
%Here we define partial combinatory algebras in terms of functional completeness rather than combinators, and as such we need to formalize expressions, substitution, and the extension of evaluation to expressions.
\begin{center}$\begin{array}{@{}c@{\qquad}c@{\qquad}c@{}}
\begin{array}{@{}r@{}c@{}l@{}}
e & {}::={} & i \in \left\{ 0 , \ldots , n - 1 \right\} \mid c \in \mca \mid e \bullet e \\
E_n(\mca) & {}::={} & \{ e \mid \text{all $i$s in $e$ are $< n$}\} \\
\end{array}
&
    \begin{tabular}{c|c}
         $e_{a} $ & $e_{a}\left[e_{b}\right]$ \\
         \hline
         $0$ & $e_{b}$ \\
         $i + 1$ & $i$ \\
         $c$ & $c$ \\
         $e_{1} \bullet e_{2}$ & $e_{1}\left[e_{b}\right] \bullet e_{2}\left[e_{b}\right]$
    \end{tabular}
\end{array}$
$$
\inferrule*{ }{c \downarrow c} \qquad  \ \inferrule*{e_f \downarrow c_f \\ e_a \downarrow c_a \\ c_f \bullet c_a \downarrow c_r}{e_f \bullet e_a \downarrow c_r} $$
\end{center}
\label{exp+sub}
Elements of $E_{0}\left(\mca\right)$ are called \emph{closed} , while for every $n>0$, elements of $E_{n}\left(\mca\right)$ are called \emph{open}.

% Next comes substitution, which expresses the idea that variables are ``stand-ins'' for other expressions.
% The expression $e_{a}\left[e_{b}\right]$ represents the substitution of every free occurrence of the index $0$ by $e_{b}$ within $e_{a}$.
% Substitution is defined by recursion on the structure of $e_{a}$:

\begin{definition}[Partial Combinatory Algebra]
A \emph{partial combinatory algebras (PCA)} is a partial applicative structure $\mca$, equipped with a (total) ``abstraction'' operator
\[ \left\langle \lambda^{n} . - \right\rangle : E_{n+1}\left(\mca\right) \rightarrow \mca \]
which takes an open expression and returns a code, abiding by the following laws:
\begin{align*}
\left\langle \lambda^{n+1} . e \right\rangle \cdot c_{a} \downarrow \left\langle \lambda^{n} . e \left[c_{a}\right] \right\rangle \qquad ; \qquad
\left\langle \lambda^{0} . e \right\rangle \cdot c_{a} \downarrow c_{r} \iff e \left[ c_{a} \right] \Downarrow c_{r}
\end{align*}
\end{definition}
%
The abstraction operator essentially takes an open expression, and ``delays'' the evaluation of the result of substituting each free variable in it with a code.

%\subsection{Realizability Tripos}
With PCAs, one can construct an interpretation of $\ihol$ where formulas are satisfied by concrete programs which serve as witness to their truth.
The construction creates a special tripos where the Heyting algebra is derived from an evidence relation between $\mca$-valued predicates.
An $\mca$-valued predicate is a function of the form $X \rightarrow \P\left(\mca\right)$, where $\mca$ is a PCA, $X$ is a set and $\P\left(\mca\right)$ is the power set of $\mca$.
Given an $x \in X$, when $c \in \varphi\left(x\right)$ we call $c$ a \emph{realizer} of $\varphi\left(x\right)$.


To form a Heyting algebra, the \emph{evidence relation} is defined such that for two $\mca$-predicates over $X$,
$\varphi , \psi : X \rightarrow P\left(\mca\right)$, we say there is an \emph{evidence} that $\varphi$ entails $\psi$ (and  write $\varphi \leq \psi$) when:
\[ \exists e \in \mca \forall x \in X \forall c_{a} \in \mca \; . \; c_{a} \in \varphi\left(x\right) \supset e \cdot c_{a} \in \psi\left(x\right) \]
%
That is, there is a code $e$ such that for every $x$, the program $e$ takes an input in $\varphi\left(x\right)$ and outputs a result in $\psi\left(x\right)$.
%
The evidence relation forms a Heyting algebra when $\mca$ is a PCA, by using the expressive power of abstraction to construct realizers for specific predicates and evidence for specific rules.
For example, given two $\mca$-valued predicates $\varphi_{1} , \varphi_{2} : X \rightarrow P\left(\mca\right)$, their meet is defined by:
\[ \left(\varphi_{1} \sqcap \varphi_{2}\right)\left(x\right) := \left\{ c \in \mca \mid c \cdot \left\langle \lambda^{1} . 0 \right\rangle \in \varphi_{1} \wedge c \cdot \left\langle \lambda^{1} . 1 \right\rangle \in \varphi_{2} \right\} \]
%
From this, the construction of a realizability tripos is standard, as in, \eg~\lcnote{CITE:Pitts? Is it standard?}

\lcnote{Need to decide: do we give a direct translation   from HOL to PCA? or just demonstrate that they are an instance of HOPL discussing the consequences for the translation? I lean towards the latter}

======COPY=====


The realizability tripos is constructed as follows:
\begin{itemize}
    \item The underlying category $\C$ is the category $\boldsymbol{Set}$ of sets and functions
    \item The inverse image functor is defined by
    \begin{align*}
        \P\left(X\right) & := P\left(\mca\right)^{X} \\
        f^{-1}\left(\varphi\right)\left(x\right) & := \varphi\left(f\left(x\right)\right)
    \end{align*}
    where the Heyting algebra in $P\left(\mca\right)^{X}$ is defined via the evidence relation
    \item The quantifier functors are defined by:
    \begin{align*}
        \prod_{f}\left(\varphi\right)\left(y\right) & := \bigcap \left\{ \varphi\left(x\right) | f\left(x\right) = y \right\} \\
        \coprod_{f}\left(\varphi\right)\left(y\right) & := \bigcup \left\{ \varphi\left(x\right) | f\left(x\right) = y \right\}
    \end{align*}
    \item Powers are defined by:
        \[ \Omega^{X} := P\left(\mca\right)^{X} \]
    \item Membership is defined by application:
        \begin{align*}
            \boldsymbol{In}_{X} & : X \times P\left(\mca\right)^{X} \rightarrow P\left(\mca\right) \\
            \boldsymbol{In}_{X}\left(x,\varphi\right) & := \varphi\left(x\right)
        \end{align*}
    \item Comprehension is defined by currying:
        \[ \left\{ \varphi \right\}\left(y\right)\left(x\right) := \varphi\left(x,y\right) \]
\end{itemize}


=====

\agnote{Explain, \textbf{in words}, what a PCA is, focus on an example}

To reason about PCAs, the notion of refinements over PCAs is described through PCA-valued predicates.
Given a PCA $\mca$ and a set $X$, we call any function of the form $X \rightarrow \P\left(\mca\right)$, where $\P\left(\mca\right)$ is the power set of $\mca$, a $\mca$-valued predicate.
The refinements of the standard translation are $\mca$-valued predicates.

To describe the refinements we introduce the following notation:
\[ \definedto{c_{f} \cdot c_{a}}{\varphi} \]
meaning $c_{f} \cdot c_{a}$ is defined and the result is in $\varphi$:
\[ \exists c_{r} : \mca \; . \; c_{f} \cdot c_{a} \downarrow c_{r} \; \wedge \; c_{r} \in \varphi \]

Since PCAs have only one type, there is no need for a kind system, so there is no need for a kind translation either.
Instead, we only need the following translation functions:
\agnote{Note: $\boldsymbol{Set}$ is the class of logical types, $\left\{\mca\right\}$ is the class of program types}
\[ \trind{}{-} : \mathcal{U} \rightarrow \boldsymbol{Set} \qquad
    \trtype{\Gamma}{-} : \prop{\Gamma} \rightarrow \left\{ \mca \right\} \qquad
    \trspec{\Gamma}{-} : \prop{\Gamma} \rightarrow \trind{}{\Gamma} \rightarrow \P\mca \]
Where $\trind{}{\Gamma}$ is defined by extending $\trind{}{-}$ to contexts through a cartesian product:
\[ \trind{}{\left[x_{1} : \sigma_{1} , \ldots , x_{n} : \sigma_{n}\right]} := \trind{}{\sigma_{1}} \times \cdots \times \trind{}{\sigma_{n}}  \]
With $\trind{}{-}$ assigning a set to each context $\Gamma$, $\trspec{\Gamma}{-}$ translates each proposition over $\Gamma$ into an $\mca$-valued predicate over $\trind{}{\Gamma}$.
\[ \trind{}{\pred{\sigma_{1} , \ldots , \sigma_{n}}} := \P\left(\trind{}{\sigma_{1}} \times \cdots \times \trind{}{\sigma_{n}} \right) \]
The type translation is trivial, since there is only one possible type to choose from:
\[ \trtype{\Gamma}{\varphi_{1} \supset \varphi_{2}} := \mca
    \qquad
    \trtype{\Gamma}{\forall_{x : \tau} . \varphi} := \mca
    \qquad
    \trtype{\Gamma}{e_{0} \in_{\tau} e_{1}} := \mca \]
The translation is using a set-theoretic foundation to describe the refinements, so they are defined through set comprehension notation, with the refinement of implication now accounting for partiality:
\begin{align*}
    \trspec{\Sigma}{\varphi_{1} \supset \varphi_{2}}\left(\gamma\right) &:= \comp{c_{f} : \mca}{ \forall {c_{a} : \mca } . c_{a} \in \trspec{\Sigma}{\varphi_{1}}\left(\gamma\right) \; \supset \; \definedto{c_{f} \cdot c_{a}}{\trspec{\Sigma}{\varphi_{2}}}\left(\gamma\right) }\\
    \trspec{\Sigma}{\forall {x : \sigma} . \varphi}\left(\gamma\right) &:= \comp{c : \mca}{ \forall{x : \sigma} .
    c \in \trspec{\Sigma , x:\sigma}{\varphi}\left(\left\langle\gamma,x\right\rangle\right)}\\
    \trspec{\Sigma}{ \tmem{\left(p_{1} , \ldots , p_{n}\right)}{p}{?} }\left(\left\langle\gamma , A , a_{1} , \ldots , a_{n}\right\rangle\right) &:= \comp{ c : \mca }{\left\langle a_{1} , \ldots , a_{n} , c \right\rangle \in A }
\end{align*}

==> section/effhol_old.tex <==
\section{Higher-Kinded Polymorphic Evaluation Logic}
\agnote{Rename HKPEL to Higher Evaluation Logic}
As a general, complex example. explain why it is important and the difference from previous examples in the overview.
Formal definition of the  logic.
\agnote{no need to deal with basic types}

As an example of a program logic which supports higher-kinded polymorphism, we introduce \emph{Higher-Kinded Polymorphic Evaluation Logic}.

The language has the following judgements:
\begin{itemize}
    \item $\boxed{\elkind{k}}$, $k$ is a \emph{kind}
    \item $\boxed{\elcon{\Delta}{\sigma}{k}}$, $\sigma$ is a type constructor of kind $k$ in context $\Delta$
    \item $\boxed{\eltrm{\Delta}{\Gamma}{e}{\sigma}}$, $e$ is a term of type $\sigma$ in kind context $\Delta$ and type context $\Gamma$
\end{itemize}

We assume a set $K$ of \emph{kinds}, which has a kind of $n$-ary type operators $\left(k_{1},\ldots,k_{n}\right) \Rightarrow \star$ for any natural number $n$ and any $k_{i} \in K$ (for any $i\in\left\{1,\ldots,n\right\}$).
The kind of nullary type operators $\left(\right)\Rightarrow\star$ will be written simply as $\star$, and it is the kind of types.
Unary type operators $\left(k\right) \Rightarrow \star$ will be written simply as $k \Rightarrow \star$.

% The presence of the unit kind requires the equation, for any kind $k$\emnote{very naive question maybe, but why?}\agnote{I think I haven't explained it properly. The idea is that this way I can easily define the kinds of predicates recursively without having to deal with 1st-order predicates as a special case. It's merely a matter of convenience}:
% \[ \boldsymbol{1} \Rightarrow k \; = \; k \]

% Similarly, on the type level, if $\sigma_{a} : \boldsymbol{1} \Rightarrow k$ and $\sigma_{b} : \boldsymbol{1}$, then:
% \[ \sigma_{a}\left(\sigma_{b}\right) = \sigma_{a} \]
% \emnote{this suggests that types of kind $\boldsymbol{1}$ are irrelevant, can we consider that there is a unique such type?}

A \emph{kind context} $\Delta$ is a list of kinds.

Given a kind context $\Delta$, we can define a \emph{type context} $\Gamma_{\Delta}$ of types over $\Delta$. We'll simply write $\Gamma$ when $\Delta$ is implicitly understood from context.

Type constructors are the same as in System F$\omega$, with the addition of \emph{predicate} types and \emph{computational} types.

\begin{definition}[Type Constructors]\label{def:typCons}
Given a kind context $\Delta$ and a kind $k$ in $\Delta$, the set $\con{\Delta}{k}$ of \emph{type constructors} of kind $k$ over $\Delta$, is inductively generated by:
\newcommand{\myskip}{1.2em}
\begin{table}[H]
    \begin{tabular}{cc}
         Type Variables & $\dfrac{(X : k) \in \Delta}{ \elcon{\Delta}{X}{k}}$\\[\myskip]
         Arrow & $\dfrac{}{\elcon{\Delta}{\mathsf{Arr}}{\left(\star , \star\right) \Rightarrow \star}}$\\[\myskip]
         Universal Quantification & $\dfrac{}{\elcon{\Delta}{\mathsf{Forall}_{k}}{\left(k \Rightarrow \star \right) \Rightarrow \star}}$\\[\myskip]
         Kind Abstraction & $\dfrac{\elcon{\Delta , X : k_{1}}{C}{k_{2}}}{\elcon{\Delta}{\lambda X . C}{k_{1} \Rightarrow k_{2}}}$\\[\myskip]
         Kind Application & $\dfrac{\elcon{\Delta}{C_{1}}{k_{1} \Rightarrow k_{2}} \qquad \elcon{\Delta}{C_{2}}{k_{1}}}{\elcon{\Delta}{C_{1} \left(C_{2}\right)}{k_{2}}}$\\[\myskip]
         Predicates & $\dfrac{}{\elcon{\Delta}{\mathsf{P}}{\star \Rightarrow \star}}$\\[\myskip]
         Computations & $\dfrac{}{\elcon{\Delta}{\mathsf{M}}{\star \Rightarrow \star}}$
    \end{tabular}
\caption{Type Constructors}
\end{table}

Any type constructor of kind $\star$ is a \emph{type}.

We use the following abbreviations:
\begin{itemize}
    \item $\tau_{1} \rightarrow \tau_{2} := \mathsf{Arr} \left( \tau_{1} , \tau_{2} \right)$
    \item $\prod_{X : k} C := \mathsf{Forall}_{k} \; \left( \lambda X . C \right) $
\end{itemize}

\end{definition}

\begin{definition}[Formulas and Terms]\label{def:termsForm}

Given a kind context $\Delta$, a type context $\Gamma$ over $\Delta$, and a type $\tau$ over $\Delta$, the set $\trm{\Delta ; \Gamma}{\tau}$ of \emph{pure terms} of type $\tau$ over $\Delta ; \Gamma$ is inductively generated by:
\newcommand{\myskip}{1.2em}
\begin{table}[H]
    \begin{tabular}{cc}
         Value Variables & $\dfrac{x:\tau \in \Gamma}{x \in \trm{\Delta ; \Gamma}{\tau}}$ \\[\myskip]
         Type Abstraction & $\dfrac{e \in \trm{\Delta , X : k ; \Gamma}{\tau}}{\Lambda X . e \in \trm{\Delta ; \Gamma}{\prod_{X : k} \tau} }$ \\[\myskip]
         Value Abstraction & $\dfrac{e \in \trm{\Delta ; \Gamma , x : \tau_{1}}{\tau_{2}}}{\lambda x . e \in \trm{\Delta ; \Gamma}{\tau_{1} \rightarrow \tau_{2}} }$ \\[\myskip]
         Type Application & $\dfrac{e \in \trm{\Delta ; \Gamma}{\prod_{X : k} \tau} \quad C \in \con{\Delta}{k}}{e\:C \in \trm{\Delta ; \Gamma}{\tau \left[ X := C \right]}}$ \\[\myskip]
         Comprehension & $\dfrac{\varphi \in \prop{\Delta ; \Gamma , x:\tau}}{\left\{ x : \tau \, | \, \varphi \right\}\in \trm{\Delta ; \Gamma}{\pred{\tau}}}$ \\[\myskip]
         Return & $\dfrac{e \in \trm{\Delta ; \Gamma}{\tau}}{\eta\left(e\right) \in \trm{\Delta ; \Gamma}{M \left(\tau\right)}}$\\[\myskip]
         Bind & $\dfrac{m \in \trm{\Delta ; \Gamma}{M \left(\tau_{1}\right)} \quad n \in \trm{\Delta ; \Gamma , x : \tau_{1}}{M \left(\tau_{2}\right)}}{\left[ x \leftarrow m \, | \, n \right] \in \trm{\Delta ; \Gamma}{M \left(\tau_{2}\right)}}$
    \end{tabular}
\caption{Terms}
\end{table}

The set $\prop{\Delta ; \Gamma}$ of \emph{formulas} over $\Delta ; \Gamma$ is inductively generated by:
\renewcommand{\myskip}{1.2em}
\begin{table}[H]
    \centering
    \begin{tabular}{cc}
        Equality & $\dfrac{e_{1} , e_{2} \in \trm{\Delta ; \Gamma}{\tau}}{e_{1} = e_{2} \in \prop{\Delta ; \Gamma}}$ \\[\myskip]
        Top & $\dfrac{}{\top \in \prop{\Delta ; \Gamma}}$ \\[\myskip]
        Bottom & $\dfrac{}{\bot \in \prop{\Delta ; \Gamma}}$ \\[\myskip]
        Conjunction & $\dfrac{\varphi_{1},\varphi_{2} \in \prop{\Delta ; \Gamma}}{\varphi_{1} \wedge \varphi_{2} \in \prop{\Delta ; \Gamma}}$ \\[\myskip]
        Implication & $\dfrac{\varphi_{1},\varphi_{2} \in \prop{\Delta ; \Gamma}}{\varphi_{1} \supset \varphi_{2} \in \prop{\Delta ; \Gamma}}$ \\[\myskip]
        Universal quantification & $\dfrac{\varphi \in \prop{\Delta ; \Gamma , x : \tau}}{\forall_{x:\tau} \varphi \in \prop{\Delta ; \Gamma}}$ \\[\myskip]
        Membership & $\dfrac{e \in \trm{\Delta ; \Gamma}{\tau} \quad \varphi \in \trm{\Delta ; \Gamma}{\pred{\tau}}}{e \inplus \varphi \in \prop{\Delta ; \Gamma}}$ \\[\myskip]
        After & $\dfrac{e \in \trm{\Delta ; \Gamma}{M \left(\tau\right)} \quad \varphi \in \prop{\Delta ; \Gamma , x : \tau}}{\left\{ x \leftarrow m \, | \, \varphi \right\} \in \prop{\Delta ; \Gamma}}$
    \end{tabular}
    \caption{Formulas}
    \label{tab:effhol-prop}
\end{table}

\end{definition}

Sequents in the language are defined with an extra \emph{kind context} $\Delta$ on which everything else depends. So we have:

\[ \sequent{\Delta \mid \Gamma}{\varphi_{1} , \ldots , \varphi_{n}}{\psi} \]
where:
\[ \varphi_{1} , \ldots , \varphi_{n} , \psi \in \prop{\Delta ; \Gamma} \]

\subsubsection{Higher-Order Translation}

In HOL we can derive most logical constants from a few basic ones, so the translation will only focus on them. The formula translations are similar to the ones for FOL, with the addition of the membership predicate.

\begin{align*}
    \trtype{\Gamma}{\top} &:= \mathbb{1}\\
    \trtype{\Gamma}{\varphi_{1} \wedge \varphi_{2}} &:= M \trtype{\Gamma}{\varphi_{1}} \times M \trtype{\Gamma}{\varphi_{2}}\\
    \trtype{\Gamma}{\varphi_{1} \supset \varphi_{2}} &:= \trtype{\Gamma}{\varphi_{1}} \Rightarrow M \trtype{\Gamma}{\varphi_{2}}\\
    \trtype{\Gamma}{\forall_{x : \tau} . \varphi} &:= M \trtype{\Gamma , \tau}{\varphi}\\
    \trtype{\Gamma}{e_{0} \in_{\tau} e_{1}} &:= \tretype{\Gamma}{e_{1}}{\pred{\tau}}\left(\tretype{\Gamma}{e_{0}}{\tau}\right)
\end{align*}

\begin{align*}
    \trprop{\Gamma}{\top}\left[c\right] &:= \top\\
    \trprop{\Gamma}{\varphi_{1} \wedge \varphi_{2}}\left[p\right] &:= 
    \after{\mathsf{fst}\left(p\right)}{x_{1}}{\trprop{\Gamma}{\varphi_{1}}\subst{x_{1}}} \wedge \after{\mathsf{snd}\left(p\right)}{x_{2}}{\trprop{\Gamma}{\varphi_{2}}\subst{x_{2}}}\\
    \trprop{\Gamma}{\varphi_{1} \supset \varphi_{2}}\left[f\right] &:= \forall {c : \trtype{\Gamma}{\varphi_{1}} } . \trprop{\Gamma}{\varphi_{1}}\left[c\right] \supset \after{f\left(c\right)}{y}{\trprop{\Gamma}{\varphi_{2}}\subst{y}}\\
    \trprop{\Gamma}{\forall {x : \tau} . \varphi}\left[m\right] &:= \forall{x : \tau} .
    \after{m}{y}{\trprop{\Gamma , \tau}{\varphi}\subst{x,y}}\\
    \trprop{\Gamma}{e_{0} \in_{\tau} e_{1}}\subst{c} &:= \left\langle \trtrm{\Gamma}{e_{0}}{\tau} , c \right\rangle \in \trtrm{\Gamma}{e_{1}}{\pred{\tau}}
\end{align*}
\emnote{in the last case, isn't it the $\inplus$ membership ?}

Now, in addition to the aforementioned translations, we also need a translation of terms to type constructors:
\begin{align*}
    \tretype{\Gamma , x : \tau}{x}{\tau} &= \sigma_{x} : \trkind{\tau}\\
    \tretype{\Gamma}{ \comprehend{x}{\tau}{\varphi}}{\pred{\tau}} &:= \lambda \sigma_{x} : \trkind{\tau} . \trtype{\Gamma , x:\tau}{\varphi}\subst{\sigma_{x}}
\end{align*}
\emnote{is the $\trtype{\Gamma , x:\tau}{\varphi}\subst{\sigma_{x}}$ ok? $\trtype{-}{-}\subst{t}$ is not defined, is it?}
and a translation of terms to terms:
\begin{align*}
    \trtrm{\Gamma , x : \tau}{x}{\tau} &= \widehat{x} : \truniv{\sigma_{x} : \trkind{\tau}}{\tau}\\
    \trtrm{\Gamma}{ \comprehend{x}{\tau}{\varphi}}{\pred{\tau}} &:= \comprehend{p}{\truniv{\sigma_{x} : \trkind{\tau}}{\tau} \times \trtype{\Gamma , x:\tau}{\varphi}}{\trprop{\Gamma , x:\tau}{\varphi}\emnote{[p] ?}}
\end{align*}
\emnote{$ \widehat{x}$ is $x$ but in the target? Also, the first rules somehow suggest you consider contexts upto permutation right? If at some point we want to add dependencies I guess it should come with the companion rule:
\[ \trtrm{\Gamma , y : \tau'}{x}{\tau} = \trtrm{\Gamma }{x}{\tau} \]}
Which also requires a translation of types to types:
\begin{align*}
    \truniv{\sigma : \boldsymbol{1}}{\beta} &:= \beta\\
    \truniv{\sigma : k \Rightarrow \star}{\pred{\tau}} &:= \prod_{\alpha : k} \pred{\truniv{\alpha : k}{\tau} \times \sigma\left(\alpha\right) }
\end{align*}

and a translation of types to kinds:
\begin{align*}
    \trkind{\beta} &:= \boldsymbol{1}\\
    \trkind{\pred{\tau}} &:= \trkind{\tau} \Rightarrow \star
\end{align*}

We extend the types to kinds translation to a type context to kind context translation by mapping, and we extend the types to types translation to a translation of contexts to context:
\[ \truniv{\sigma : k , \Delta}{x : \tau , \Gamma} := \widehat{x} : \truniv{\sigma : k}{\tau} , \truniv{\Delta}{\Gamma} \]

In summary, we have the following translation functions:
\begin{align*}
    \trtype{\Gamma}{-} &: \prop{\Gamma} \rightarrow \con{\trkind{\Gamma}}{\star} \\
    \trprop{\Gamma}{-} &: \prod_{\varphi : \prop{\Gamma}} \prop{\trkind{\Gamma} ; \truniv{\trkind{\Gamma}}{\Gamma}, e : \trtype{\Gamma}{\varphi}} \\
    \tretype{\Gamma}{-}{\tau} &: \trm{\Gamma}{\tau} \rightarrow \con{\trkind{\Gamma}}{\trkind{\tau}} \\
    \trtrm{\Gamma}{-}{\tau} &: \prod_{\trm{\Gamma}{\tau}} \trm{\trkind{\Gamma} ; \truniv{\trkind{\Gamma}}{\Gamma}}{\truniv{\Gamma}{\tau}} \\
    \truniv{-}{-} &: \prod_{\tau : \mathcal{U}} \prod_{\sigma : \trkind{\tau}} \con{\sigma : \trkind{\tau}}{\star} \\
    \trkind{-} &: \mathcal{U} \rightarrow \boldsymbol{Kind}
\end{align*}
\emnote{some $\Pi$ quantifies over unused variables, is it intended (rather than a simple arrow)?}

Triples now have, in addition, a \emph{kind context} $\Delta$. So the following triple:
\[  \triple{\Delta \mid \Gamma \mid \Sigma}{\Phi}{ x \leftarrow m }{\Psi}  \]
is defined as:
\[ \sequent{\Delta \mid \Gamma , \Sigma}{\Phi}{\after{m}{x}{\psi\subst{x}}} \]
In the case of Polymorphic Evaluation Logic both $\Gamma$ and $\Sigma$ are taken from the same universe.

We show that the translation is sound by proving for each theorem \[\sequent{\Delta \mid \Gamma}{\varphi_{1} , \ldots , \varphi_{n}}{\Psi}\]
in FOL, that there is some program
\[ f \in \trm{\trkind{\Gamma} ; \truniv{\trkind{\Gamma}}{\Gamma}}{\trtype{\Gamma}{\varphi_{1}} \times \hdots \times \trtype{\Gamma}{\varphi_{n}} \rightarrow M\trtype{\Gamma}{\psi} } \]
\emnote{$\trkind{\Delta}$?}
such that:
\[ \triple{\Delta \mid \Gamma \mid c_{1} :\trtype{\Gamma}{\varphi_{1}} , \ldots , c_{n} :\trtype{\Gamma}{\varphi_{n}} }{ \Theta }{c_{r} \leftarrow f\left(c_{1} , \ldots , c_{n}\right)}{\trprop{}{\psi}\left[ c_{r} \right]} \]
where:
\[ \Theta := \trprop{\Gamma}{\varphi_{1}}\left[ c_{1} \right] , \ldots , \trprop{\Gamma}{\varphi_{n}}\left[ c_{n} \right]\]

Let's look at an example. Let $A$ be some type.
Consider the following theorem:
\[ \sequent{\varphi_{1} , \varphi_{2} : \pred{A} , \Phi_{1} , \Phi_{2}  : \pred{\pred{A}}}{\left( \varphi_{1} \in \Phi_{1} \right) \wedge \left( \varphi_{2} \in \Phi_{2}\right)}{\left( \varphi_{2} \in \Phi_{2} \right) \wedge \left( \varphi_{1} \in \Phi_{1}\right)} \]

We have:
\[ \Gamma =  \varphi_{1} : \pred{A}  , \varphi_{2} : \pred{A} , \Phi_{1} : \pred{\pred{A}} , \Phi_{2} : \pred{\pred{A}} \]

So the context to kinds context translation is:
\begin{align*}
&\Delta := \trkind{\Gamma}\\
&= \trkind{\varphi_{1} : \pred{A}}  , \trkind{\varphi_{2} : \pred{A}} , \trkind{\Phi_{1} : \pred{\pred{A}}} , \trkind{\Phi_{2} : \pred{\pred{A}}}\\
&=\sigma_{\varphi_{1}} : \boldsymbol{1} \Rightarrow \star \; , \;\sigma_{\varphi_{2}} : \boldsymbol{1} \Rightarrow \star \; , \;\sigma_{\Phi_{1}} : \left(\boldsymbol{1} \Rightarrow \star\right) \Rightarrow \star \; , \; \sigma_{\Phi_{2}} : \left(\boldsymbol{1} \Rightarrow \star\right) \Rightarrow \star\\
&=\sigma_{\varphi_{1}} : \star \; , \;\sigma_{\varphi_{2}} : \star \; , \;\sigma_{\Phi_{1}} : \star \Rightarrow \star \; , \; \sigma_{\Phi_{2}} : \star \Rightarrow \star
\end{align*}
The context to types context translation is:
\begin{align*}
&\truniv{\trkind{\Gamma}}{\Gamma}\\
&= \truniv{\sigma_{\varphi_{1}} : \boldsymbol{1} \Rightarrow \star }{\varphi_{1} : \pred{A}}  \; , \; \truniv{\sigma_{\varphi_{2}} : \boldsymbol{1} \Rightarrow \star }{\varphi_{2} : \pred{A}} \; \\ &, \; \truniv{\sigma_{\Phi_{1}} : \left(\boldsymbol{1} \Rightarrow \star\right) \Rightarrow \star }{\Phi_{1} : \pred{\pred{A}}} \; , \; \truniv{\sigma_{\Phi_{2}} : \left(\boldsymbol{1} \Rightarrow \star\right) \Rightarrow \star }{\Phi_{2} : \pred{\pred{A}}}\\
&= \widehat{\varphi_{1}} : \prod_{\alpha : \boldsymbol{1}} \pred{\truniv{\alpha : \boldsymbol{1}}{A} \times \sigma_{\varphi_{1}}\left(\alpha\right) }  \; , \; \widehat{\varphi_{2}} :\prod_{\alpha : \boldsymbol{1}} \pred{\truniv{\alpha : \boldsymbol{1}}{A} \times \sigma_{\varphi_{2}}\left(\alpha\right) } \; \\
& , \; \widehat{\Phi_{1}} : \prod_{\alpha : \boldsymbol{1} \Rightarrow \star} \pred{\truniv{\alpha : \boldsymbol{1} \Rightarrow \star}{\pred{A}} \times \sigma_{\Phi_{1}}\left(\alpha\right) } \; , \; \widehat{\Phi_{2}} : \prod_{\alpha : \boldsymbol{1} \Rightarrow \star} \pred{\truniv{\alpha : \boldsymbol{1} \Rightarrow \star}{\pred{A}} \times \sigma_{\Phi_{2}}\left(\alpha\right) }\\
&= \widehat{\varphi_{1}} : \pred{A \times \sigma_{\varphi_{1}} }  \; , \; \widehat{\varphi_{2}} :\pred{A \times \sigma_{\varphi_{2}} } \; \\
& , \; \widehat{\Phi_{1}} : \prod_{\alpha : \star} \pred{ \pred{A \times \alpha } \times \sigma_{\Phi_{1}}\left(\alpha\right) } \; , \; \widehat{\Phi_{2}} : \prod_{\alpha : \star} \pred{ \pred{A \times \alpha } \times \sigma_{\Phi_{2}}\left(\alpha\right) }
\end{align*}

Note that for $i \in \left\{1,2\right\}$ and term $x : \sigma_{\Phi_{i}}\left(\sigma_{\varphi_{i}}\right)$, the formulas $\left\langle \widehat{\varphi_{i}} , x \right\rangle \in \widehat{\Phi_{i}}$ are well typed in context $\truniv{\trkind{\Gamma}}{\Gamma}$ by instantiating $\alpha$ with $\sigma_{\varphi_{i}}$.

We also have:
\begin{align*}
    & \trtype{\Gamma}{\left( \varphi_{1} \in \Phi_{1} \right) \wedge \left( \varphi_{2} \in \Phi_{2}\right)} \\ &= M \trtype{\Gamma}{\varphi_{1} \in \Phi_{1}} \times M \trtype{\Gamma}{\varphi_{2} \in \Phi_{2}}\\
    &= M\left(\tretype{\Gamma}{\Phi_{1}}{\pred{\pred{A}}}\left(\tretype{\Gamma}{\varphi_{1}}{\pred{A}}\right)\right) \times M\left(\tretype{\Gamma}{\Phi_{2}}{\pred{\pred{A}}}\left(\tretype{\Gamma}{\varphi_{2}}{\pred{A}}\right)\right)\\
    &= M \left(\sigma_{\Phi_{1}}\left(\sigma_{\varphi_{1}}\right)\right) \times M \left(\sigma_{\Phi_{2}}\left(\sigma_{\varphi_{2}}\right)\right)
\end{align*}
and similarly:
\begin{align*}
    \trtype{\Gamma}{\left( \varphi_{2} \in \Phi_{2} \right) \wedge \left( \varphi_{1} \in \Phi_{1}\right)} = M \left(\sigma_{\Phi_{2}}\left(\sigma_{\varphi_{2}}\right)\right) \times M \left(\sigma_{\Phi_{1}}\left(\sigma_{\varphi_{1}}\right)\right)
\end{align*}

Also, the formula translation for the assumption is:
\begin{align*}
& \trprop{\Gamma}{\left( \varphi_{1} \in \Phi_{1} \right) \wedge \left( \varphi_{2} \in \Phi_{2}\right)}\subst{c}\\
& = \after{\mathsf{fst}\left(c\right)}{x_{1}}{\trprop{\Gamma}{\varphi_{1} \in \Phi_{1}}\subst{x_{1}}} \wedge \after{\mathsf{snd}\left(c\right)}{x_{2}}{\trprop{\Gamma}{\varphi_{1} \in \Phi_{1}}\subst{x_{2}}}\\
& = \after{\mathsf{fst}\left(c\right)}{x_{1}}{\left\langle \trtrm{\Gamma}{\varphi_{1}}{\pred{A}} , x_{1} \right\rangle \in \trtrm{\Gamma}{\Phi_{1}}{\pred{\pred{A}}}}\\ &\wedge \after{\mathsf{fst}\left(c\right)}{x_{2}}{\left\langle \trtrm{\Gamma}{\varphi_{2}}{\pred{A}} , x_{2} \right\rangle \in \trtrm{\Gamma}{\Phi_{2}}{\pred{\pred{A}}}}\\
& = \after{\mathsf{fst}\left(c\right)}{x_{1}}{\left\langle \widehat{\varphi_{1}} , x_{1} \right\rangle \in \widehat{\Phi_{1}}} \wedge \after{\mathsf{fst}\left(c\right)}{x_{2}}{\left\langle \widehat{\varphi_{2}} , x_{2} \right\rangle \in \widehat{\Phi_{2}} }
\end{align*}
and for the conclusion:
\begin{align*}
& \trprop{\Gamma}{\left( \varphi_{2} \in \Phi_{2} \right) \wedge \left( \varphi_{1} \in \Phi_{1}\right)}\subst{c}\\
& = \after{\mathsf{fst}\left(c\right)}{x_{2}}{\left\langle \widehat{\varphi_{2}} , x_{2} \right\rangle \in \widehat{\Phi_{2}}} \wedge \after{\mathsf{fst}\left(c\right)}{x_{1}}{\left\langle \widehat{\varphi_{1}} , x_{1} \right\rangle \in \widehat{\Phi_{1}} }
\end{align*}

To prove soundness, we require a program:
\[ f \in \trm{\trkind{\Gamma} ; \truniv{\trkind{\Gamma}}{\Gamma}}{M\left(\sigma_{\Phi_{1}}\left(\sigma_{\varphi_{1}}\right)\right) \times M\left(\sigma_{\Phi_{2}}\left(\sigma_{\varphi_{2}}\right)\right) \rightarrow M\left(M \left(\sigma_{\Phi_{2}}\left(\sigma_{\varphi_{2}}\right)\right) \times M\left(\sigma_{\Phi_{1}}\left(\sigma_{\varphi_{1}}\right)\right)\right) } \]
such that given a realizer of the assumption:
\[ c : M\left(\sigma_{\Phi_{1}}\left(\sigma_{\varphi_{1}}\right)\right) \times M\left(\sigma_{\Phi_{2}}\left(\sigma_{\varphi_{2}}\right)\right) \]
will compute a realizer of the output, satisfying the triple:
\[ \triple{\Delta \mid \truniv{\Delta}{\Gamma} \mid c : M\left(\sigma_{\Phi_{1}}\left(\sigma_{\varphi_{1}}\right)\right) \times M\left(\sigma_{\Phi_{2}}\left(\sigma_{\varphi_{2}}\right)\right) }{ \Theta }{c_{r} \leftarrow f\left(c\right)}{\Psi} \]
where:
\begin{align*}
    \Theta & := \after{\mathsf{fst}\left(c\right)}{x_{1}}{\left\langle \widehat{\varphi_{1}} , x_{1} \right\rangle \in \widehat{\Phi_{1}}} \wedge \after{\mathsf{fst}\left(c\right)}{x_{2}}{\left\langle \widehat{\varphi_{2}} , x_{2} \right\rangle \in \widehat{\Phi_{2}} }\\
    \Psi & := \after{\mathsf{fst}\left(c_{r}\right)}{x_{2}}{\left\langle \widehat{\varphi_{2}} , x_{2} \right\rangle \in \widehat{\Phi_{2}}} \wedge \after{\mathsf{fst}\left(c_{r}\right)}{x_{1}}{\left\langle \widehat{\varphi_{1}} , x_{1} \right\rangle \in \widehat{\Phi_{1}} }
\end{align*}

For that end, we use:
\[ f := \lambda c . \eta(\left( \left\langle \mathsf{snd}\left(c\right) , \mathsf{fst}\left(c\right) \right\rangle \right) \]

So we get:
\[ \sequent{\Delta \mid \truniv{\Delta}{\Gamma} , c : M\left(\sigma_{\Phi_{1}}\left(\sigma_{\varphi_{1}}\right)\right) \times M\left(\sigma_{\Phi_{2}}\left(\sigma_{\varphi_{2}}\right)\right)}{\Theta}{\after{\eta(\left( \left\langle \mathsf{snd}\left(c\right) , \mathsf{fst}\left(c\right) \right\rangle \right)}{c_{r}}{\Psi}} \]
which, by the definition of the triples over the language, is exactly what we need.

To prove this theorem, we simply take the introduction law of the modality, transforming the above sequent to:
\[ \sequent{\Delta \mid \truniv{\Delta}{\Gamma} , c : M\left(\sigma_{\Phi_{1}}\left(\sigma_{\varphi_{1}}\right)\right) \times M\left(\sigma_{\Phi_{2}}\left(\sigma_{\varphi_{2}}\right)\right)}{\Theta}{\Psi\subst{\left\langle \mathsf{snd}\left(c\right) , \mathsf{fst}\left(c\right) \right\rangle}} \]

Now, since:
\[ \Psi\subst{\left\langle \mathsf{snd}\left(c\right) , \mathsf{fst}\left(c\right) \right\rangle} \dashv \vdash \Theta \]
we get:
\[ \sequent{\Delta \mid \truniv{\Delta}{\Gamma} , c : M\left(\sigma_{\Phi_{1}}\left(\sigma_{\varphi_{1}}\right)\right) \times M\left(\sigma_{\Phi_{2}}\left(\sigma_{\varphi_{2}}\right)\right)}{\Theta}{\Theta} \]
which is trivial.

==> section/figures/HOPL_beta.tex <==

\begin{minipage}{0.45\textwidth}
\textbf{Reduction rules}\\[-2em]
\begin{mathpar}
\qquad \qquad

\termbind{\termvar}{\termret{\term_1}}{\term_2} \betared \term_2 \subst{\termvar:=\term_1}

\termtypeapp{(\termtypeabs{\typevar}{\kind}{\term})}{\type}\betared \term\subst{\typevar:=\type}

\termapp{(\termabs{\termvar}{\type}{\term})}{\termvalue}\betared \term\subst{\termvar:=\termvalue}
\end{mathpar}

\vspace{0.15cm}
where:
% \[\begin{array}{rcl}
$ \termvalue  ::= \termvar \mid \termtypeabs{\typevar}{\kind}{\term}
\mid \termabs{\termvar}{\type}{\term}$
%  \mid \emnote{remove}\termret{\term}\\
% \progcontext &::=& \hole
% \mid \termtypeapp{\progcontext}{\type}
% \mid \termapp \progcontext  {\term}
% \mid \termapp{\termvalue}{\progcontext}
% \mid \termbind{\termvar}{\progcontext}{\term}\\
% \end{array}\]
\end{minipage}%~~\vrule\quad
\\
\begin{minipage}{0.45\textwidth}
\textbf{Conversion}
\begin{mathpar}
\typeapp{(\typeabs{\typevar}{\kind}{\type_1})}{\type_2}\conv_\type\type_1\subst{\typevar:=\type_2}

\typeapp{(\eforall{\typevar:\kind}{\exprs})}{\type}\conv_\exprs \exprs\subst{\typevar:=\type}

{\conv \text{is the reflexive, symmetric, transitive contextual closure of }\conv_\type\cup\conv_\exprs}
\end{mathpar}
\end{minipage}
\emnote{does it still deserve to be in a "figure" ?}
\lcnote{the appendix contains a figure with the full reduction system. Do we not need anything there anymore? I'll see what we can say now about progress and preservation}










==> section/figures/HOPL_beta_old.tex <==
\begin{minipage}{0.45\textwidth}

\raggedright
\textbf{Types}

\begin{mathpar}

\typeapp{(\typeabs{\typevar}{\kind}{\type_1})}{\type_2}\typered \type_1\subst{\typevar:=\type_2}


\infer{\taucontext[\type_1]\typered \taucontext[\type_2]}{\type_1 \typered \type_2}
\end{mathpar}
~\\
where:
\[\begin{array}{rcl}
 \typevalue & ::= & \typevar \mid \typeabs{\typevar}{\kind}{\type}\mid\\
 &&\typefun{\typevalue}{\typevalue}\mid \typecomp{\typevalue}\mid\ttypprod{\typevar:\kind}{\typevalue}
 \\[\myskip]
\taucontext &::= &\hole \mid \typeapp{\taucontext}{\type} \mid \typeapp{\typevalue}{\taucontext}
\mid
\typefun{\taucontext}{\typecomp{\type}}\mid\\
&&
\typefun{\type}{\typecomp{\taucontext}}
\mid
\ttypprod{\typevar:\kind}{\taucontext}
\mid
\typecomp{\taucontext}\\

\end{array}
\]

%\lcnote{don't we want the C to also include things other than types? say, expression of type application, comprehension, ... type application in programs...}
\end{minipage}
~\vrule\quad
\begin{minipage}{0.47\textwidth}
\raggedright
\textbf{Programs}
\begin{mathpar}
\termtypeapp{(\termtypeabs{\typevar}{\kind}{\term})}{\type}\betared \term\subst{\typevar:=\type}

\termapp{(\termabs{\termvar}{\type}{\term})}{\termvalue}\betared \term\subst{\termvar:=\termvalue}

\termbind{\termvar}{\termret{\term_1}}{\term_2} \betared \term_2 \subst{\termvar:=\term_1}

\infer{\betacontext[\term_1]\betared \betacontext[\term_2]}{\term_1 \betared \term_2}

\infer{\termtypeapp{\term}{\type_1}\betared \termtypeapp{\term}{\type_2}}{
\type_1 \typered \type_2
}
\end{mathpar}
where:
\[\begin{array}{rcl}
 \termvalue & ::= & \termvar \mid \termtypeabs{\typevar}{\kind}{\term}
 \mid \termabs{\termvar}{\type}{\term}
 \mid \termret{\term}\\[\myskip]

\betacontext &::=& \hole
\mid \termtypeapp{\betacontext}{\type}
\mid \termapp \betacontext  {\term}
\mid \termapp{\termvalue}{\betacontext}
\mid \termbind{\termvar}{\betacontext}{\term}
\end{array}\]
\end{minipage}


$\begin{array}{rcl}
\exprcontext
            & ::=  & \hole \mid \ecomp{\termvar}{\type}{\exprsvar}{\indice}{\speccontext}
            \mid  \ecompbase{\termvar}{\type}{\tprop}
            \mid  \eforall{\typevar:\kind}{\exprs} 
            \mid  \eapp{\exprs}{\type} \\

\speccontext & ::= &\tmem{\term}{\hole}{\exprs} 
            \mid \tmembase{\term}{\exprs} 
            \mid \timplies{ \tprop }{ \tprop } 
            \mid \after{\term}{\termvar}{\tprop} 
            \mid \tspeckinprod{\typevar:\kind}{\tprop} 
            \mid \tspectypprod{\termvar:\type}{\tprop} 
            \mid \tspecindprod{\epred:\indice}{\tprop} 
\end{array}$            

==> section/figures/HOPL_semantics.tex <==
% Kinds and Type Constructors
\begin{center}
\begin{tabular}{c|c}
    \infer
    { \eltype{\kcontext}{\typevar : \kind} }
    { \left(\typevar : \kind\right) \in \kcontext }
&
    \infer
    { \pi_{k} \in \hom{\basecat}{\kind_{1} \times \ldots \times \kind_{n}}{\kind_{k}} }
    { \kind_{1} \times \ldots \times \kind_{n} \in \obj{\basecat} }
\\[\myskip]
    \infer
    { \eltype{\kcontext}{ \typeapp{\type_{2}}{\type_{1}} : \star } }
    { \eltype{\kcontext}{\type_{1} : \kind } \qquad \eltype{\kcontext}{\type_{2} : \typecon{\kind} } }
&
    \infer
    { \varepsilon \circ \pair{\type_{2}}{\type_{1}} \in \hom{\basecat}{\kcontext}{\typeobj} }
    { \type_{1} \in \hom{\basecat}{\kcontext}{\kind} \qquad \type_{2} \in \hom{\basecat}{\kcontext}{\expobj{\kind}{\typeobj}} }
\\[\myskip]
    \infer
    { \eltype{\kcontext}{ \typeabs{\typevar}{\kind}{\type} : \typecon{\kind} } }
    { \eltype{\kcontext , \typevar : \kind}{\type : \star} }
&
    \infer
    { \expobj{\type}{\kind} \circ \eta \in \hom{\basecat}{\kcontext}{\expobj{\kind}{\typeobj}} }
    { \type \in \hom{\basecat}{\kcontext \times \kind}{\typeobj} }
\\[\myskip]
    \infer
    { \eltype{\kcontext}{\typefun{\type_{1}}{\type_{2}} : \star} }
    { \eltype{\kcontext}{\type_{1} : \star} \qquad \eltype{\kcontext}{\type_{2} : \star} }
&
    \infer
    { \expobj{\type_{1}}{\type_{2}} \in \obj{\ind{\indcat}{\kcontext}} }
    { \type_{1} \in \obj{\ind{\indcat}{\kcontext}} \qquad \type_{1} \in \obj{\ind{\indcat}{\kcontext}} }
\\[\myskip]
    \infer
    { \eltype{\kcontext}{\prod_{\typevar : \kind} \type : \star} }
    { \eltype{\kcontext, \typevar : \kind}{\type} : \star }
&
    \infer
    { \overleftarrow{\ind{\indcat}{\pi_{1}}} \left(\type\right) \in \obj{ \ind{\indcat}{\kcontext}} }
    { \type \in \obj{ \ind{\indcat}{\kcontext \times \kind} } }
\\[\myskip]
    \infer
    { \eltype{\kcontext}{\typecomp{\type} : \star} }
    { \eltype{\kcontext}{\type : \star} }
&
    \infer
    { \monad\left(\type\right) \in \ind{\indcat}{\kcontext} }
    { \type \in \ind{\indcat}{\kcontext} }
\end{tabular}
\end{center}

% Types and Programs
\begin{center}
\begin{tabular}{c|c}
\infer
    { \eltrm{\kcontext \mid \tcontext}{\termvar}{\type} }
    { (\termvar:\type) \in \tcontext }
& AAA
\\[\myskip]
    \infer
    { \eltrm{\kcontext \mid \tcontext}{\termtypeabs{\typevar}{\kind}{\term}}{\prod_{\typevar : \kind} \type} }
    { \eltrm{\kcontext , \typevar : \kind \mid \tcontext}{\term}{\type} }
&
    \infer
    { \radj{\ind{\indcat}{\pi_{1}}}\term \circ \eta \in \hom{\ind{\indcat}{\kcontext}}{\tcontext}{ \radj{\ind{\indcat}{\pi_{1}}} \left(\type\right)} }
    { \term \in \hom{\ind{\indcat}{\kcontext \times \kind}}{ \ind{\indcat}{\pi_{1}} \left(\tcontext\right)}{\type} }
\\[\myskip]
    \infer
    { \eltrm{\kcontext \mid \tcontext}{\termabs{ \termvar}{\type_1}{\term}}{\typefun{\type_{1}}{\type_{2}}} }
    { \eltrm{\kcontext \mid \tcontext, \termvar : \type_{1}}{\term}{\type_{2}} }
&
    \infer
    { \expobj{\type_{1}}{\term}  \circ \eta \in \hom{\ind{\indcat}{\kcontext}}{\tcontext}{\expobj{\type_{1}}{\type_{2}}}  }
    { \term \in \hom{\ind{\indcat}{\kcontext}}{\tcontext \times \type_{1}}{\type_{2}} }
\\[\myskip]
    \infer
    { \eltrm{\kcontext \mid \tcontext}{\termtypeapp{\term}{\type_{1}}}{\type_{2}\subst{\typevar := \type_{1}}} }
    { \eltrm{ \kcontext \mid \tcontext }{\term}{ \prod_{\typevar : \kind} \type_{2} } & \eltype{\kcontext}{\type_{1} : \kind} }
&
    \infer
    { \ind{\indcat}{\pair{\id}{\type_{1}}} \varepsilon \circ \term \in \hom{\ind{\indcat}{\kcontext}}{\tcontext}{\ind{\indcat}{\pair{\id}{\type_{1}}} \left(\type_{2}\right) } }
    { \term \in \hom{\ind{\indcat}{\kcontext}}{\tcontext}{\overleftarrow{\ind{\indcat}{\pi_{1}}}\left(\type_{2}\right) } &
    \type_{1} \in \hom{\basecat}{\kcontext}{\kind} }
\\[\myskip]
    \infer
    { \eltrm{\kcontext \mid \tcontext}{\termapp{\term_{2}}{\term_{1}}}{\typecomp{\type_{2}}} }
    { \eltrm{ \kcontext \mid \tcontext }{\term_{2}}{\typefun{\type_{1}}{\typecomp{\type_{2}}} } \quad \eltrm{ \kcontext \mid \tcontext }{\term_{1}}{\type_{1}} }
& AAA
\\[\myskip]
    \infer
    { \eltrm{\kcontext \mid \tcontext}{\termret{\term}}{\typecomp{\type}} }
    { \eltrm{\kcontext \mid \tcontext}{\term}{\type} }
& AAA
\\[\myskip]
    \infer
    { \eltrm{\kcontext \mid \tcontext}{\termbind{\termvar}{\term_{1}}{\term_{2}}}{\typecomp{\type_{2}}} }
    { \eltrm{\kcontext \mid \tcontext}{\term_{1}}{\typecomp{\type_{1}}} \qquad \eltrm{\kcontext \mid \tcontext, \termvar : \type_{1}}{\term_{2}}{\typecomp{\type_{2}}} }
& AAA
\end{tabular}
\end{center}

% Sorts and Expressions
\begin{center}
\begin{tabular}{c|c}
    \infer
    { \eltype{\context}{\epred : \indice} }
    { \left(\epred : \indice\right) \in \icontext }
& AAB
\\[\myskip]
    \infer
    { \eltrm{\context}{\ecomp{\termvar}{\type}{\exprsvar}{\indice}{\tprop}}{\refpred{\type}{\indice}} }
    { \elprop{\kcontext \mid \tcontext , \termvar : \type \mid \icontext , \exprsvar : \indice}{\tprop} }
& \infer
    { \triposcomp{\tprop} \in \hom{\ind{\expcat}{\kcontext}}{\cxtpair{\kcontext}{\icontext}}{\pred{\cxtpair{\type}{\indice}}} }
    { \tprop \in Q_{\kcontext}\left(\cxtpair{\tcontext \times \type}{\icontext \times \indice}\right) = \P \left( I_{\kcontext}\left(\left(\cxtpair{\tcontext }{\icontext}\right) \times \left( \cxtpair{\type}{\indice}\right)\right)\right) }
\\[\myskip]
    \infer
    { \eltype{\context}{\eforall{\typevar:\kind}\exprs : \tindprod{\typevar:\kind}{\indice}} }
    { \eltype{\kcontext,\typevar:\kind \mid \tcontext  \mid \icontext}{\exprs : {\indice}} }
&
    \infer
    {\radj{\ind{\expcat}{\pi_{1}}} \exprs \circ \adjunit \in \hom{\ind{\expcat}{\kcontext}}{\cxtpair{\tcontext}{\icontext}}{\overleftarrow{\ind{\expcat}{\pi_{1}}} \left(\indice\right)}}
    {\exprs \in \hom{\ind{\expcat}{\kcontext \times \kind}}{\ind{\expcat}{\pi_{1}}\left( \cxtpair{\tcontext}{\icontext} \right) }{\indice}}
\\[\myskip]
    \infer
    { \eltype{\context}{\eapp{\exprs}{\type} : {\indice\subst{\typevar:=\type}}} }
    { \eltype{\context}{\exprs : \tindprod{\typevar:\kind}{\indice}} & \eltype{\kcontext}{\type:\kind} }
&
    \infer
    {\ind{\expcat}{\pair{\id}{\type}} \varepsilon \circ e \in \hom{\ind{\indcat}{\kcontext}}{\tcontext}{\ind{\expcat}{\pair{\id}{\type_{1}}} \left(\type_{2}\right) }}
    {e \in \hom{\ind{\expcat}{\kcontext}}{\cxtpair{\tcontext}{\icontext}}{\overleftarrow{\ind{\expcat}{\pi_{1}}} \left(\indice\right)} \; \type \in \hom{\basecat}{\kcontext}{\kind}}
\\[\myskip]
    \infer
    { \elprop{\context}{\tmem{\term}{\exprs_{2}}{\langle \exprs_{1}\rangle}} }
    { \eltype{\context}{\term : \type} \quad \eltype{\context}{\exprs_{1} : \indice} \quad \eltype{\context}{\exprs_{2} : \refpred{\type}{\indice}} }
& AAA
\end{tabular}
\end{center}

% Specifications
\begin{center}
\begin{tabular}{c|c}
    \infer
    { \elprop{\context}{\after{\term}{\termvar}{\tprop}} }
    { \eltype{\kcontext \mid \tcontext}{\term : \typecomp{\type}} \quad \elprop{\kcontext \mid \tcontext , \typevar : \type \mid \icontext}{\tprop} }
&
    \infer
    { Q_{\kcontext}\left(\cxtpair{\left(\strength \circ \pair{\id_{\tcontext}}{\term}\right)}{\id_{\icontext}}\right)\left(\rho\left(\tprop\right)\right) \in Q_{\kcontext}\left(\cxtpair{\tcontext}{\icontext}\right) }
    {\term \in \hom{\ind{\indcat}{\kcontext}}{\tcontext}{ \ind{\monad}{\kcontext} \left(\type\right)}
    \quad
    \tprop \in Q_{\kcontext}\left( \cxtpair{\left(\tcontext \times \type\right)}{\icontext} \right)
    }
\\[\myskip]
    \infer
    { \elprop{\context}{\timplies{ \tprop_{1} }{ \tprop_{2} }} }
    { \elprop{\context}{\tprop_{1}} \qquad \elprop{\context}{\tprop_{2}} }
& AAA
\\[\myskip]
    \infer
    { \elprop{\context}{\tspeckinprod{\typevar:\kind}{\tprop}} }
    { \elprop{\kcontext , \typevar : \kind \mid \tcontext \mid \icontext}{\tprop} }
&
    \infer
    % { \radj{\P\left( \pi_{1} \right)}  \left( \P\left(\id , \pi_{1}\right)\left(\tprop\right)\right) \in \P\left(\kcontext ,  \ind{\expfun}{\kcontext}\left(\tcontext , \icontext\right) \right) }
    { \radj{\P\left(\int \pfreyd \left( \indemb{\pi_{1}} \right) \right)} \left(\tprop\right) \in Q_{\kcontext}\left( \cxtpair{\tcontext}{\icontext} \right) }
    { \tprop \in Q_{\kcontext \times \kind}\left( \ind{\left(\indcat \times \statecat\right)}{\pi_{1}}\left(\cxtpair{\tcontext}{\icontext}\right) \right) }
    % { \tprop \in \P\left(\kcontext \times \kind , \ind{\expcat}{\pi_{1}}\left( \ind{\expfun}{\kcontext}\left(\tcontext, \icontext \right)\right)\right) }
\\[\myskip]
    \infer
    { \elprop{\context}{\tspectypprod{\termvar:\type}{\tprop}} }
    { \elprop{\kcontext \mid \tcontext , \termvar : \type \mid \icontext}{\tprop} }
&
    \infer
    {\radj{Q_{\kcontext}\left(\cxtpair{\pi_{1}}{\id}\right)}\left(\tprop\right) \in Q_{\kcontext}\left( \cxtpair{\tcontext}{\icontext} \right) }
    { \tprop \in Q_{\kcontext}\left( \cxtpair{\tcontext \times \type}{\icontext} \right) }
\\[\myskip]
    \infer
    { \elprop{\context}{\tspecindprod{\epred:\indice}{\tprop}} }
    { \elprop{\kcontext \mid \tcontext \mid \icontext , \epred : \indice }{\tprop} }
&
    \infer
    {\radj{Q_{\kcontext}\left(\cxtpair{\id}{\pi_{1}}\right)}\left(\tprop\right) \in Q_{\kcontext}\left( \cxtpair{\tcontext}{\icontext} \right) }
    {\tprop \in Q_{\kcontext}\left( \cxtpair{\tcontext}{\icontext \times \indice } \right) }
\end{tabular}
\end{center}



{\color{magenta}TODO: 
\begin{itemize}
    \item example of the negation of classical logic
    \item classical meta via realizability adjuctions
    \item HOPL -> EF
    \item fix separator 
    \item capturing multiple concrete effectful implementations of DC in (classical) HOPL, e.g.~\cite{Herbelin:lics:2012,Miquey:lics:2018,Berardi+Bezem+Coquand:jsyml:1998} (synthesizing an abstract specification for memoization?)
    \item blurred separation
\end{itemize}
}



==> section/figures/HOPL_syntax.tex <==
    $\begin{array}{l:l:l}
    \begin{array}[t]{l@{\hspace{-0.35in}}llll}
\textbf{Kinds} &&&&\\
            & \kind 
            & ::=  & \star & 
            \mbox{(base type const.)}
            \\
            & & \mid &\typecon{\kind} & \mbox{(type const.)}
\\[\sskip]
\textbf{Types} &&&&\\
            & \type 
            & ::=  & \typevar  & \mbox{(variable)}
            \\
            & &\mid  & \typeapp{\type}{\type}  & \mbox{(application)}
            \\
            & &\mid  & \typeabs{\typevar}{\kind}{\type}  & \mbox{(abstraction)}
            \\
            & &\mid  & \typefun{\type}{\typecomp{\type}} & \mbox{(function)}
            \\
            & &\mid  &\ttypprod{\typevar:\kind}{\type} & \mbox{(universal)}
            \\
            & &\mid  & \typecomp{\type}  & \mbox{(computation)}
            \\[\sskip]

\textbf{Programs} & &&&\\
            &\term 
            & ::=  & \termvar & \mbox{(variable)}
            \\
            && \mid  &\termtypeabs{\typevar}{\kind}{\term} & \mbox{(type abstraction)}
            \\
            & &\mid & \termabs{\termvar}{\type}{\term} & \mbox{(term abstraction)}
            \\
            & &\mid &  \termtypeapp{\term}{\type} & \mbox{(type application)}
            \\
            & &\mid & \termapp{\term}{\term} & \mbox{(term application)}
            \\
            & &\mid &  \termret{\term}  & \mbox{(return)}
            \\
            & &\mid &  \termbind{\termvar}{\term}{\term}  & \mbox{(bind)}
         %   ~\\
\end{array}
&
\begin{array}[t]{l@{\hspace{-0.55in}}llll}
\textbf{Indices} &&&&\\
            & \indice 
            & ::=  & \refpredN{\type} & \mbox{(base refinement)}%\lcnote{where is it used?}}
            \\
            & &\mid  & 
            \refpred{\type}{\indice} & \mbox{(refinement)}
            \\
            & &\mid  & \tindprod{\typevar:\kind}{\indice}  & \mbox{(universal) }
            \\[\sskip]
            
\textbf{Expressions} &&&&\\
            & \exprs
            & ::=  & \epred & \mbox{(variable)}
            \\
            && \mid  &\ecomp{\termvar}{\type}{\exprsvar}{\indice}{\tprop}
            & \mbox{(comprehension)}\\
            && \mid  &\ecompbase{\termvar}{\type}{\tprop}
            & \mbox{(base comprehension)}\\
            &&\mid & \eforall{\typevar:\kind}{\exprs} & \mbox{(type abstraction)}\\
            &&\mid & \eapp{\exprs}{\type} & \mbox{(type application)}
            \\[\sskip]

\textbf{Specifications} &&&&\\
            & \tprop 
            & ::=  & \tmem{\term}{\exprs}{\exprs} & \mbox{(membership)}\\
            & &\mid& \tmembase{\term}{\exprs} & \mbox{(base membership)}\\ 
            & &\mid & \timplies{ \tprop }{ \tprop } & \mbox{(implication)}
            \\
            & &\mid &  \after{\term}{\termvar}{\tprop}  & \mbox{(modality)}
            \\
            & &\mid & \tspeckinprod{\typevar:\kind}{\tprop} & \mbox{(type uni.)}
            \\
            & &\mid & \tspectypprod{\termvar:\type}{\tprop} & \mbox{(program uni.)} 
            \\
            & &\mid &  \tspecindprod{\epred:\indice}{\tprop} & \mbox{(expression uni.)} 
            % \\[\sskip]
            % \\[\sskip]
%\\
\end{array}
% \\
% \hdashline
% \end{array}$
% ~\\[\sskip]
&
    \begin{array}[t]{|l@{\hspace{-0.6in}}l@{\hspace{0.1in}}l@{\hspace{0.1in}}l|}
    \hline
  %\rule{0pt}{3ex}% more  vertical space for 1st line
    \texttt{Kind Context} &&&\\
    & 
\kcontext & ::=  & \emptyset \mid \kcontext,\typevar:\kind
\\[\myskip]
    \texttt{Index Context}  &&&\\
    & 
\icontext & ::=  & \emptyset \mid \icontext,\epred:\indice
\\[\myskip]
    \texttt{Type Context}  &&&\\
    & 
\tcontext & ::=  & \emptyset \mid \tcontext,\termvar:\type\\
\hline
   \end{array}
\end{array}$


==> section/figures/MCAinter.tex <==
\begin{figure}[t]
\begin{small}
    \centering
        $\begin{array}{l@{\hspace{0.01in}}:l}
        \hspace{-0.5in}
        \def\arraystretch{1.3}
    \begin{array}{l@{\hspace{-0.3in}}l@{\hspace{0.01in}}l@{\hspace{0.1in}}l}


\textbf{Types} &&&\\
            & \interptype{\typevar_{1} : \kind_{1} , \ldots , \typevar_{n} : \kind_{n}}{\typevar_{j}} & :=  & \pi_{2} \circ \pi_{1}^{\left(n-j\right)} 
            \\
            & \interptype{\kcontext}{\typeapp{\type_{1}}{\type_{2}}} & := & \adjcounit \circ \pair{\interptype{\kcontext}{\type_{2}}}{\interptype{\kcontext}{\type_{1}}}
            \\
            & \interptype{\kcontext}{\typeabs{\typevar}{\kind}{\type}} & := & \expobj{\interptype{\kcontext}{\type}}{\interpkind{\kind}} \circ \adjunit
            \\
            & \interptype{\kcontext}{\typefun{\type_{1}}{\type_{2}}}  & := & \expobj{\interptype{\kcontext}{\type_{1}}}{\interptype{\kcontext}{\type_{2}}}
            \\
            & \interptype{\kcontext}{\ttypprod{\typevar:\kind}{\type}} & := & \radj{\ind{\indcat}{\pi_{1}}} \left(\interptype{\kcontext , \typevar : \kind}{\type}\right)
            \\
            &  \interptype{\kcontext}{\typecomp{\type}} &:=& \monad \left(\interptype{\kcontext}{\type}\right)
            \\
            [\myskip]

\textbf{Programs} &&&\\
            & \interpterm{\kcontext}{\termvar_{1} : \type_{1} , \ldots , \termvar_{n} : \type_{n}}{\termvar_{j}} & :=  & \pi_{2} \circ \pi_{1}^{\left(n-j\right)}
            \\
            & \interpterm{\kcontext}{\tcontext}{\termtypeabs{\typevar}{\term}} & :=  & \radj{\ind{\indcat}{\pi_{1}}}\left(\interpterm{\kcontext , \typevar : \kind}{\tcontext}{\term}\right) \circ \adjunit
            \\
             & \interpterm{\kcontext}{\tcontext}{\termabs{\termvar}{\term}} & :=  & \expobj{\interptype{\kcontext}{\type_{1}}}{\left(\interpterm{\kcontext}{\tcontext , \termvar : \type}{{\term}}\right)} \circ \adjunit
            \\
            & \interpterm{\kcontext}{\tcontext}{\termtypeapp{\term}{\type}} & :=  & \ind{\indcat}{\pair{\id}{\interptype{\kcontext}{\type}}} \adjcounit \circ \interpterm{\kcontext}{\tcontext}{\term}
            \\
            &\interpterm{\kcontext}{\tcontext}{\termapp{\term_{1}}{\term_{2}}} & :=  & \adjcounit \circ \pair{\interpterm{\kcontext}{\tcontext}{\term_{1}}}{\interpterm{\kcontext}{\tcontext}{\term_{2}}}
            \\
            & \interpterm{\kcontext}{\tcontext}{\termret{\term}} & :=  & \eta \circ \interpterm{\kcontext}{\tcontext}{\term}
            \\
            & \interpterm{\kcontext}{\tcontext}{\termbind{\termvar}{\term_{1}}{\term_{2}}} & :=  & \mu \circ \monad\interpterm{\kcontext}{\tcontext , \termvar : \type}{\term_{2}} \circ \strength \circ \pair{\id}{\interpterm{\kcontext}{\tcontext}{\term_{1}}}
            \\[\myskip]

\end{array}
&
        \def\arraystretch{1.3}
    \begin{array}{l@{\hspace{-0.5in}}l@{\hspace{0.01in}}l@{\hspace{0.1in}}l}
\textbf{Indicies} &&&\\
            & \interptype{\kcontext}{\refpredN{\type}} & :=  & \pred{\ind{\expfun}{ \interpkind{\kcontext} }\left(\interptype{\kcontext}{\type} , \terminalobj \right)}
            \\
            & \interptype{\kcontext}{\refpred{\type}{\indice}} & :=  & \pred{\ind{\expfun}{ \interpkind{\kcontext} }\left(\interptype{\kcontext}{\type} , \interptype{\kcontext}{\indice}\right)}
            \\
            & \interptype{\kcontext}{\tindprod{\typevar:\kind}{\indice}} & :=  & \radj{\ind{\expcat}{\pi_{1}}}\left(\interptype{\kcontext , \typevar : \kind}{\indice}\right)
            \\[\myskip]

\textbf{Expressions} &&&\\
            & \interpexpr{\kcontext}{\tcontext}{\epred_{1} : \indice_{1} , \ldots , \epred_{n} : \indice_{n}}{\epred_{j}} & :=  & \unitor^{-1} \circ \ind{\expfun}{\interpkind{\kcontext}}\left(\terminalmap , \pi_{2} \circ \pi_{1}^{\left(n-j\right)}\right)
            \\
            &     \interpexpr{\kcontext}{\tcontext}{\icontext}{\ecomp{\termvar}{\type}{\exprsvar}{\indice}{\tprop}} &:=& {\color{red} \text{COMPREHENSION}}\\
    &\interpexpr{\kcontext}{\tcontext}{\icontext}{\eforall{\typevar:\kind}{\exprs}} &:=& \radj{\ind{\expcat}{\pi_{1}}} \interpexpr{\kcontext , \typevar : \kind}{\tcontext}{\icontext}{\exprs} \circ \adjunit \\
    &\interpexpr{\kcontext}{\tcontext}{\icontext}{\eapp{\exprs}{\type}} &:=& \ind{\expcat}{\pair{\id}{\interptype{\kcontext}{\type}}} \adjcounit \circ \interpexpr{\kcontext}{\tcontext}{\icontext}{\exprs}\\
    [\myskip]




\textbf{Specifications} &&&\\
               & \interpspec{\kcontext}{\tcontext}{\icontext}{\tmem{\term}{\exprs}{\langle \exprs\rangle}} &:=&
               ?
               \\
    &\interpspec{\kcontext}{\tcontext}{\icontext}{\timplies{ \tprop_{1} }{ \tprop_{2} }} &:=& \interpspec{\kcontext}{\tcontext}{\icontext}{\tprop_{1}} \sqsupset \interpspec{\kcontext}{\tcontext}{\icontext}{\tprop_{2}}\\
    &\interpspec{\kcontext}{\tcontext}{\icontext}{\after{\term}{\termvar}{\tprop}} &:=& \P\left( \id , \ind{\expfun}{\interpkind{\kcontext}}\left( \strength \circ \pair{\id}{\interpterm{\kcontext}{\tcontext}{\term}} , \id \right) \right)\left(\rho\left(\interpspec{\kcontext}{\tcontext , \termvar : \type}{\icontext}{\tprop}\right)\right)\\
    &\interpspec{\kcontext}{\tcontext}{\icontext}{\tspeckinprod{\typevar:\kind}{\tprop}} &:=& \radj{\P\left( \pi_{1} \right)}  \left( \P\left(\id , \pi_{1}\right)\left( \interpspec{\kcontext , \typevar : \kind}{\tcontext}{\icontext}{ \tprop}\right)\right)\\
    &\interpspec{\kcontext}{\tcontext}{\icontext}{\tspectypprod{\termvar:\type}{\tprop}} &:=&
    \radj{\P\int\expfun\left(\id , \pi_{1}\right)} \left( \P\left( \id , \ind{\expfun}{\kcontext}\left(\id,\pi_{1}\right) \right)\left( \interpspec{\kcontext}{\tcontext , \termvar:\type}{\icontext}{\tprop} \right)\right) \\
    &\interpspec{\kcontext}{\tcontext}{\icontext}{\tspecindprod{\epred:\indice}{\tprop}} &:= &\radj{\P\int\expfun\left(\id , \pi_{1}\right)} \left( \P\left( \id , \ind{\expfun}{\kcontext}\left(\pi_{1}, \id\right) \right)\left(\interpspec{\kcontext}{\tcontext}{\icontext , \epred:\indice}{\tprop}\right)\right)\\
            [\myskip]
\end{array}
\end{array}$
\end{small}
    \caption{The Interpretation of $\effhol$\lcnote{TODO: clean context}}
    \label{fig:inter}
\end{figure}

==> section/figures/seminter.tex <==
\begin{figure}[t]
\begin{small}
    \centering
        $\begin{array}{l@{\hspace{0.01in}}:l}
        \hspace{-0.5in}
        \def\arraystretch{1.3}
    \begin{array}{l@{\hspace{-0.3in}}l@{\hspace{0.01in}}l@{\hspace{0.1in}}l}
\textbf{Kinds} &&&\\
         & \interpkind{\star}  & :=  &  ?
            \\
            & \interpkind{\typecon{\kind}}  & :=  &  \expobj{\interpkind{\kind}}{\typeobj}
            \\[\myskip]

\textbf{Types} &&&\\
            & \interptype{\typevar_{1} : \kind_{1} , \ldots , \typevar_{n} : \kind_{n}}{\typevar_{j}} & :=  & \pi_{2} \circ \pi_{1}^{\left(n-j\right)} 
            \\
            & \interptype{\kcontext}{\typeapp{\type_{1}}{\type_{2}}} & := & \adjcounit \circ \pair{\interptype{\kcontext}{\type_{2}}}{\interptype{\kcontext}{\type_{1}}}
            \\
            & \interptype{\kcontext}{\typeabs{\typevar}{\kind}{\type}} & := & \expobj{\interptype{\kcontext}{\type}}{\interpkind{\kind}} \circ \adjunit
            \\
            & \interptype{\kcontext}{\typefun{\type_{1}}{\type_{2}}}  & := & \expobj{\interptype{\kcontext}{\type_{1}}}{\interptype{\kcontext}{\type_{2}}}
            \\
            & \interptype{\kcontext}{\ttypprod{\typevar:\kind}{\type}} & := & \radj{\ind{\indcat}{\pi_{1}}} \left(\interptype{\kcontext , \typevar : \kind}{\type}\right)
            \\
            &  \interptype{\kcontext}{\typecomp{\type}} &:=& \monad \left(\interptype{\kcontext}{\type}\right)
            \\
            [\myskip]

\textbf{Programs} &&&\\
            & \interpterm{\kcontext}{\termvar_{1} : \type_{1} , \ldots , \termvar_{n} : \type_{n}}{\termvar_{j}} & :=  & \pi_{2} \circ \pi_{1}^{\left(n-j\right)}
            \\
            & \interpterm{\kcontext}{\tcontext}{\termtypeabs{\typevar}{\term}} & :=  & \radj{\ind{\indcat}{\pi_{1}}}\left(\interpterm{\kcontext , \typevar : \kind}{\tcontext}{\term}\right) \circ \adjunit
            \\
             & \interpterm{\kcontext}{\tcontext}{\termabs{\termvar}{\term}} & :=  & \expobj{\interptype{\kcontext}{\type_{1}}}{\left(\interpterm{\kcontext}{\tcontext , \termvar : \type}{{\term}}\right)} \circ \adjunit
            \\
            & \interpterm{\kcontext}{\tcontext}{\termtypeapp{\term}{\type}} & :=  & \ind{\indcat}{\pair{\id}{\interptype{\kcontext}{\type}}} \adjcounit \circ \interpterm{\kcontext}{\tcontext}{\term}
            \\
            &\interpterm{\kcontext}{\tcontext}{\termapp{\term_{1}}{\term_{2}}} & :=  & \adjcounit \circ \pair{\interpterm{\kcontext}{\tcontext}{\term_{1}}}{\interpterm{\kcontext}{\tcontext}{\term_{2}}}
            \\
            & \interpterm{\kcontext}{\tcontext}{\termret{\term}} & :=  & \eta \circ \interpterm{\kcontext}{\tcontext}{\term}
            \\
            & \interpterm{\kcontext}{\tcontext}{\termbind{\termvar}{\term_{1}}{\term_{2}}} & :=  & \mu \circ \monad\interpterm{\kcontext}{\tcontext , \termvar : \type}{\term_{2}} \circ \strength \circ \pair{\id}{\interpterm{\kcontext}{\tcontext}{\term_{1}}}
            \\[\myskip]

\end{array}
&
        \def\arraystretch{1.3}
    \begin{array}{l@{\hspace{-0.5in}}l@{\hspace{0.01in}}l@{\hspace{0.1in}}l}
\textbf{Indicies} &&&\\
            & \interptype{\kcontext}{\refpredN{\type}} & :=  & \pred{\ind{\expfun}{ \interpkind{\kcontext} }\left(\interptype{\kcontext}{\type} , \terminalobj \right)}
            \\
            & \interptype{\kcontext}{\refpred{\type}{\indice}} & :=  & \pred{\ind{\expfun}{ \interpkind{\kcontext} }\left(\interptype{\kcontext}{\type} , \interptype{\kcontext}{\indice}\right)}
            \\
            & \interptype{\kcontext}{\tindprod{\typevar:\kind}{\indice}} & :=  & \radj{\ind{\expcat}{\pi_{1}}}\left(\interptype{\kcontext , \typevar : \kind}{\indice}\right)
            \\[\myskip]

\textbf{Expressions} &&&\\
            & \interpexpr{\kcontext}{\tcontext}{\epred_{1} : \indice_{1} , \ldots , \epred_{n} : \indice_{n}}{\epred_{j}} & :=  & \unitor^{-1} \circ \ind{\expfun}{\interpkind{\kcontext}}\left(\terminalmap , \pi_{2} \circ \pi_{1}^{\left(n-j\right)}\right)
            \\
            &     \interpexpr{\kcontext}{\tcontext}{\icontext}{\ecomp{\termvar}{\type}{\exprsvar}{\indice}{\tprop}} &:=& {\color{red} \text{COMPREHENSION}}\\
    &\interpexpr{\kcontext}{\tcontext}{\icontext}{\eforall{\typevar:\kind}{\exprs}} &:=& \radj{\ind{\expcat}{\pi_{1}}} \interpexpr{\kcontext , \typevar : \kind}{\tcontext}{\icontext}{\exprs} \circ \adjunit \\
    &\interpexpr{\kcontext}{\tcontext}{\icontext}{\eapp{\exprs}{\type}} &:=& \ind{\expcat}{\pair{\id}{\interptype{\kcontext}{\type}}} \adjcounit \circ \interpexpr{\kcontext}{\tcontext}{\icontext}{\exprs}\\
    [\myskip]




\textbf{Specifications} &&&\\
               & \interpspec{\kcontext}{\tcontext}{\icontext}{\tmem{\term}{\exprs}{\langle \exprs\rangle}} &:=&
               ?
               \\
    &\interpspec{\kcontext}{\tcontext}{\icontext}{\timplies{ \tprop_{1} }{ \tprop_{2} }} &:=& \interpspec{\kcontext}{\tcontext}{\icontext}{\tprop_{1}} \sqsupset \interpspec{\kcontext}{\tcontext}{\icontext}{\tprop_{2}}\\
    &\interpspec{\kcontext}{\tcontext}{\icontext}{\after{\term}{\termvar}{\tprop}} &:=& \P\left( \id , \ind{\expfun}{\interpkind{\kcontext}}\left( \strength \circ \pair{\id}{\interpterm{\kcontext}{\tcontext}{\term}} , \id \right) \right)\left(\rho\left(\interpspec{\kcontext}{\tcontext , \termvar : \type}{\icontext}{\tprop}\right)\right)\\
    &\interpspec{\kcontext}{\tcontext}{\icontext}{\tspeckinprod{\typevar:\kind}{\tprop}} &:=& \radj{\P\left( \pi_{1} \right)}  \left( \P\left(\id , \pi_{1}\right)\left( \interpspec{\kcontext , \typevar : \kind}{\tcontext}{\icontext}{ \tprop}\right)\right)\\
    &\interpspec{\kcontext}{\tcontext}{\icontext}{\tspectypprod{\termvar:\type}{\tprop}} &:=&
    \radj{\P\int\expfun\left(\id , \pi_{1}\right)} \left( \P\left( \id , \ind{\expfun}{\kcontext}\left(\id,\pi_{1}\right) \right)\left( \interpspec{\kcontext}{\tcontext , \termvar:\type}{\icontext}{\tprop} \right)\right) \\
    &\interpspec{\kcontext}{\tcontext}{\icontext}{\tspecindprod{\epred:\indice}{\tprop}} &:= &\radj{\P\int\expfun\left(\id , \pi_{1}\right)} \left( \P\left( \id , \ind{\expfun}{\kcontext}\left(\pi_{1}, \id\right) \right)\left(\interpspec{\kcontext}{\tcontext}{\icontext , \epred:\indice}{\tprop}\right)\right)\\
            [\myskip]
\end{array}
\end{array}$
\end{small}
    \caption{The Interpretation of $\effhol$\lcnote{TODO: clean context}}
    \label{fig:inter}
\end{figure}

==> section/figures/translation2.tex <==
\begin{figure}[t]
  %  \centering
   $ \begin{array}{l@{\hspace{-2in}}l@{\hspace{0.1in}}l@{\hspace{0.1in}}l}
   %%%%%%%%%%%%%%%%%% SORT -> KIND %%%%%%%%%%%%%%%%%%%%%%
        \ttrkind{-} : \mathtt{sort} \to \mathtt{kind}&&&
        \\[\sskip]
        & \ttrkind{\STAR} &:= & \star
        \\
        &\ttrkind{\predcon{\sort}} &:= & \typecon{\ttrkind{\sort}}
        \\ &&&
        \\
   %%%%%%%%%%%%%%%%%% SORT -> INDEX %%%%%%%%%%%%%%%%%%%%%%
        \ttrind{-}{-} : \mathtt{sort} \to \mathtt{type}\to \mathtt{index}&&& 
        \\[\sskip]
        & \ttrind{\type} {\STAR} &:= & \refpredN{\typevar} 
        \\
        &\ttrind{\type} {\predcon{\sort}} &:= & \tindprod{\typevar_{0} : \ttrkind{\sort}}{
        \refpred{\typeapp{\type}{\typevar_{0}}}{\ttrind{\typevar_{0} }{\sort}}}
        \\ &&&
        \\      
   %%%%%%%%%%%%%%%%%% PROPOSITION -> TYPE %%%%%%%%%%%%%%%%%%%%%%
        \ttrtype{\scontext}{-} : \mathtt{proposition} \to \mathtt{type}&&&
        \\[\sskip]
    %%% implication
        &\ttrtype{\scontext}{\simplies{\sprop_{1}}{\sprop_{2}}} &:= & \typefun{\ttrtype{\scontext}{\sprop_{1}} } {M \ttrtype{\scontext}{\sprop_{2}}}\\
    %%% forall
        &\ttrtype{\scontext}{\forall_{\spred : \sort}  \sprop} &:=&  \ttypprod{\typevar_\spred :\ttrkind{\sort}} {\typecomp{\ttrtype{\scontext , \spred : \sort}{\sprop}}}\\% \lcnote{should be X_u'?}\\
    %%% membership
        &\ttrtype{\scontext}{\smem{ \sterm_{1} }{\sterm_{2}} } &:= & \typeapp{\ttretype{\scontext}{\sterm_{2}}{\predcon{\sort}}}{\ttretype{\scontext}{\sterm_{1}}{\sort}}
        \\
       &\ttrtype{\scontext}{\smembase{\sterm} }{} &:= & {\ttretype{\scontext}{\sterm}{}}
        \\
 &&&
        \\
   %%%%%%%%%%%%%%%%%% PROPOSITION -> SPECIFICATION %%%%%%%%%%%%%%%%%%%%%%
        \ttrspec{\scontext}{-}{-} : \mathtt{proposition} \to \mathtt{program}\to \mathtt{specification}&&&
        \\[\sskip]
    %%% implication
        &\ttrspec{\scontext}{\simplies{\sprop_{1}}{\sprop_{2}}}{\term} &:= & \tspectypprod{\termvar_{1} : \ttrtype{\scontext}{\sprop_{1}} } . \ttrspec{\scontext}{\sprop_{1}}{\termvar_{1}} \supset \after{\termapp{\term}{\termvar_{1}}}{\termvar_{2}}{\ttrspec{\scontext}{\sprop_{2}}{\termvar_{2}}}\\
    %%% forall
        &\ttrspec{\scontext}{\forall_{\spred : \sort} \sprop}{\term} &:= & \tspeckinprod{\typevar_\spred : \ttrkind{\sort}} \forall_{\tpred_\spred : \ttrind{\typevar_\spred}{\sort} } .
        \after{\termtypeapp{\term}{\typevar_\spred}}{\termvar_{0}}{(\ttrspec{\scontext , \spred : \sort}{\sprop}{\termvar_{0}})}\\
     %   {\color{red}\subst{ \tpred_{\spred} := \tpred }}}\lcnote{I think we don't need it}\\
    %%% membership
        &\ttrspec{\scontext}{\smem{ \sterm_{1}}{\sterm_{2}} }{\term} & := & \tmem{ \term }{ \eapp{\ttrtrm{\scontext}{\sterm_{2}}{\predcon{\sort}}}{\ttretype{\scontext}{\sterm_{1}}{\sort}} }{ \ttrtrm{\scontext}{\sterm_{1}}{\sort} }
        \\
        &\ttrspec{\scontext}{\smembase{ \sterm}}{\term} & := & \tmembase{ \term }{ \ttrtrm{\scontext}{\sterm}{\predcon{\sort}}}
        \\
 &&&
        \\
    %%%%%%%%%%%%%%%%%% TERM -> TYPE %%%%%%%%%%%%%%%%%%%%%%
        \ttretype{\scontext}{-}{\sort} : \mathtt{term} \to \mathtt{type}&&&\\[\sskip]
    %%% var
        &\ttretype{\scontext}{\spred}{\sort} &:=& \typevar_{\spred}\\
    %%% comprehension
        &\ttretype{\scontext}{\comprehend{\spred}{\sort}{\sprop}}{\predcon{\sort}} &:=& \typeabs{\typevar_\spred}{\ttrkind{\sort}}{\ttrtype{\scontext , \spred : \sort}{\sprop}}
        \\ 
        &\ttretype{\scontext}{\compbase{\sprop}}{\predcon{\sort}} &:=& {\ttrtype{\scontext , \spred : \sort}{\sprop}}
        \\
        &&&
        \\
   %%%%%%%%%%%%%%%%%% TERM -> EXPRESSION %%%%%%%%%%%%%%%%%%%%%%
        % \ttrtrm{\scontext}{-}{\sort}  : \left(\sterm : \mathtt{term}_{\scontext}\left(\sort\right)\right) \to \mathtt{expression}\left(\ttrind{\trtype{}{\sterm} }{\sort} \right)&&&\\
        \ttrtrm{\scontext}{-}{\sort}  : \mathtt{term} \to \mathtt{expression}&&&\\[\sskip]
    %%% var
        &\ttrtrm{\scontext}{\spred}{\sort} &:=& \tpred_{\spred}\\
    %%% comprehension
        &\ttrtrm{\scontext}{\comprehend{\spred}{\sort}{\sprop}}{\predcon{\sort}} &:=& \eforall{\typevar_{\spred} : \ttrkind{\sort}}{
            \tcomp{\termvar}{\ttrtype{\scontext , \spred : \sort}{\sprop}}
               {\tpred_\spred}{\ttrind{\typevar_\spred}{\sort}}
               {\ttrspec{\scontext , \spred : \sort}{\sprop}{x} }
            }     \\
          &\ttrtrm{\scontext}{\compbase{\sprop}}{\predcon{\sort}} &:=& {
            \tcompbase{\termvar}{\ttrtype{\scontext , \spred : \sort}{\sprop}}
               {\ttrspec{\scontext , \spred : \sort}{\sprop}{x} }
            }
\end{array}
$

\\[1em]
% \emnote{Due to the way we translate $u$, I think we \textbf{have} to be careful with  name variables $X_u$/$y_u$ (and not only $X$/$y$)}
    \caption{The Realizability Translations}
    \label{fig:trans2}
\end{figure}

==> section/figures/translationFig.tex <==
\begin{figure}[t]
%    \centering
   $ \begin{array}{l@{\hspace{-2in}}l@{\hspace{0.1in}}l@{\hspace{0.1in}}l}
        \trkind{-} : \SORT \rightarrow \KIND&&&\mathtt{sort} \to \mathtt{kind}
        \\[\sskip]
        & \trkind{\star} &:= & \star
        \\
        &\trkind{\predcon{\sort}} &:= & \typecon{\trkind{\sort}}
        \\ &&&
        \\
        \trind{-}{-} : \prod_{\sort : \SORT} \prod_{\type : \trkind{\sort}} \IND{\type : \trkind{\sort}} &&& \mathtt{sort} \to \mathtt{variable}\to \mathtt{kind}
        \\[\sskip]
        & \trind{\type : \star}{\STAR} &:= & \refpredN{\type} 
        \\
        &\trind{\type : \typecon{\kind}}{\predcon{\sort}} &:= & \tindprod{\typevar : \kind}{
        \refpred{\typeapp{\type}{\typevar}}{\trind{\typevar : \kind}{\sort}}}
        \\ &&&
        \\      
        \trtype{\scontext}{-} : \PROP{\scontext} \rightarrow \TYPE{\trkind{\scontext}}{\star} &&&\mathtt{proposition} \to \mathtt{type}
        \\[\sskip]
        &\trtype{\scontext}{\simplies{\sprop_{1}}{\sprop_{2}}} &:= & \typefun{\trtype{\scontext}{\sprop_{1}} } {\typecomp{ \trtype{\scontext}{\sprop_{2}}}}\\
        &\trtype{\scontext}{\forall_{\spred : \sort}  \sprop} &:=&  \prod_{\typevar_\spred : \trkind{\sort}} \typecomp{\trtype{\scontext , \spred : \sort}{\sprop}}
        \\
        % \text{\emnote{don't we need $\tau \to M\trtype{\scontext}{\sprop}$ ?}\agnote{No. Universal realizers are agnostic to the quantified term}}\\
        &\trtype{\scontext}{\smem{ \sterm_{1} }{\sterm_{2}} } &:= & \typeapp{\tretype{\scontext}{\sterm_{2}}{\predcon{\sort}}}{\tretype{\scontext}{\sterm_{1}}{\sort}}
        \\ &&&
        \\
        \trspec{\scontext}{-} : \prod_{\sprop : \PROP{\scontext}} \SPEC{\trkind{\scontext}}
    {\termvar : \trtype{\scontext}{\sprop}}{\trind{\trkind{\scontext}}{\scontext}} &&&\quad\mathtt{proposition} \to \mathtt{program (var?)}\to \mathtt{specification}
        \\[\sskip]
        &\trspec{\scontext}{\simplies{\sprop_{1}}{\sprop_{2}}}\subst{\termvar} &:= & \tspectypprod{\termvar_{1} : \trtype{\scontext}{\sprop_{1}} } . \trspec{\scontext}{\sprop_{1}}\subst{\termvar_{1}} \supset \after{\termapp{\termvar}{\termvar_{1}}}{\termvar_{2}}{\trspec{\scontext}{\sprop_{2}}\subst{\termvar_{2}}}\\
        &\trspec{\scontext}{\forall_{\spred : \sort} \sprop}\subst{\termvar} &:= & \tspeckinprod{\typevar_\spred : \trkind{\sort}} \forall_{\tpred_\spred : \trind{\typevar}{\sort} } . \after{\termtypeapp{\termvar}{\typevar_\spred}  }{\termvar_{0}}{(\trspec{\scontext , \spred : \sort}{\sprop}\subst{\termvar_{0}})}\\
        % \text{\emnote{shouldn't it be $y\,\widehat{p}$}\agnote{maybe? not sure}}\\ 
        &\trspec{\scontext}{\smem{ \sterm_{1}}{\sterm_{2}} }\subst{\termvar} & := & \tmem{ \termvar }{ \eapp{\trtrm{\scontext}{\sterm_{2}}{\predcon{\sort}}}{\tretype{\scontext}{\sterm_{1}}{\sort}} }{ \trtrm{\scontext}{\sterm_{1}}{\sort} }
        \\ &&&
        \\
        \tretype{\scontext}{-}{\sort} : \trm{\scontext}{\sort} \rightarrow \TYPE{\trkind{\scontext}}{\trkind{\sort}}
        &&&\qquad\mathtt{term} \to \mathtt{type}\\[\sskip]
        &\tretype{\scontext}{\spred}{\sort} &:=& \typevar_{\spred}\\
        &\tretype{\scontext}{\comprehend{\spred}{\sort}{\sprop}}{\predcon{\sort}} &:=& \typeabs{\typevar}{\trkind{\sort}}{\trtype{\scontext , \spred : \sort}{\sprop}}
        \\ &&&
        \\
        \trtrm{\scontext}{-}{\sort}  : \prod_{\sterm : \trm{\scontext}{\sort}} \rightarrow \EXP{\trkind{\scontext} \mid \emptyset \mid \trind{\trkind{\scontext}}{\scontext}}{\trind{\tretype{\scontext}{\sterm}{\sort}}{\sort}}
        &&&\qquad\qquad\qquad\mathtt{term} \to \mathtt{expression}\\[\sskip]
        &\trtrm{\scontext}{\spred}{\sort} &:=& \tpred_{\spred}\\
        &\trtrm{\scontext}{\comprehend{\spred}{\sort}{\sprop}}{\predcon{\sort}} &:=& \eforall{\typevar_{\spred} : \trkind{\sort}}{\tcomp{\termvar}{\trtype{\scontext , \spred : \sort}{\sprop}}{\tpred}{\trind{\trkind{\sort}}{\sort}}{ \trspec{\scontext , \spred : \sort}{\sprop} }}
\end{array}
$
    \caption{The Realizability Translations}
    \label{fig:trans}
\end{figure}

==> section/firstorder.tex <==
\section{First Order Realizability}

Given any sufficiently rich programming language, along with a program logic, we can interpret logic through a realizability translation where the logic is considered as specifying the behavior of the programs in the given language.

For every formula, by induction on the syntactic structure, we describe how this formula is translated to a condition on a program. We call this translation a \emph{realizability translation}, and we say that the programs which satisfy the derived condition are \emph{realizers} of the formula.

To make the translation well-defined, all realizers of the same formula will share the same type\emnote{this suggests that realizers are typed, which is indeed what you do afterwards, but I think a good question to keep in mind would be to see whether this restriction might be relaxed afterwards}\agnote{I can try, but if the realizers don't share a type it could probably make the translation much more complicated}.
So formulas are given two interpretations: First, formulas are interpreted as the type of their realizers, and then they are interpreted as a specification formula over an extended context, with a new free variable, which stands for their realizer.

More formally, for First-Order Logic (FOL), if $\prop{\Gamma}$ is the set of fist-order formulas over context $\Gamma$, and $\mathcal{B}$ is the universe of types in the target programming language, then we define the following two translation functions:

Assuming a first-order context $\Gamma$ over $\mathcal{B}$, we define two translations:
\begin{itemize}
    \item $\trtype{\Gamma}{-} : \prop{\Gamma} \rightarrow \mathcal{B}$ - Translation of first-order formulas to types
    \item $\trspec{\Gamma}{-} : \prod\left(\varphi : \prop{\Gamma}\right) . \prop{ \Gamma , \trtype{\Gamma}{\varphi} }$ - Translation of first-order \emph{logic} formulas to first-order \emph{specification} formulas with an extra variable, which stands for a realizer of the formula
\end{itemize}

We may wish to keep the source logic separate from the target logic. So the target logic will have, in addition to the \emph{logical} types of the source logic, \emph{program} types which are the types of the programming language.

We may also want to keep to logical types of the target logic separate from the logical types of the source logic, in which case we also need to translate the types of the source logic to types of the target logic. However, for now we'll assume they are the same, or at least we'll use abuse of notation to make the translation of types implicit.

If we wish to keep the source and target separate, we can write $\prop{\Gamma}^{\mathcal{S}}$ for formulas over $\Gamma$ in the source logic, and $\prop{\Gamma ; \Sigma}^{\mathcal{T}}$ for formulas over logical context $\Gamma$ and program context $\Sigma$ in the target logic.

 Now the translation functions will become:
\begin{itemize}
    \item $\trtype{\Gamma}{-} : \prop{\Gamma}^{\mathcal{S}} \rightarrow \mathcal{B}$
    
    \item $\trspec{\Gamma}{-} : \prod\left(\varphi : \prop{\Gamma}^{\mathcal{S}}\right) . \prop{ \Gamma ; \trtype{\Gamma}{\varphi} }^{\mathcal{T}}$
\end{itemize}
\emnote{in the second case, one $\Gamma$ is defined in the source language while the other is in the target, don't you need something like : $\prod\left(\varphi : \prop{\Gamma}^{\mathcal{S}}\right) . \prop{ \trtype{}{\Gamma}; \trtype{\Gamma}{\varphi} }^{\mathcal{T}}$ ? (where $\trtype{}{A_1,...,A_n}=\trtype{}{A_1},\trtype{A_1}{A_2},\trtype{A_1,A_2}{A_3},...$)}\agnote{Good point, I'll change it}
To interpret theories, the program logic has to have some notion of \emph{triples}. That is, a judgement of the form:

\[ \triple{\Gamma \mid \Sigma}{\Phi}{ m }{\Psi} \]

Where $\Gamma$ is a logical context, $\Sigma$ is a program context, $m \in \prog{\Sigma}{\Xi}$ is a program\emnote{I am not sure I understood the notation, does it mean that in the end $m$ is defined in the context $\Sigma,\Xi$ ?}\agnote{The contexts could come from completely different universes, in which case it doesn't make sense to append them. In the Evaluation Logic example I do define it as the concatenation of both but in general it's best to allow them to be separate}, which binds some program variables $\Xi = \left[x_{1} : \tau_{1} , \ldots , x_{n} : \tau_{n}\right]$, $\Phi \in \prop{\Gamma ; \Sigma}^{*}$ is a list of formulas over $\Gamma$ and $\Sigma$, and $\psi \in \prop{\Gamma ; \Sigma , \Xi}$ is a formula over logical context $\Gamma$ and program context $\Sigma , \Xi$.

A theorem
\[\sequent{\Gamma}{\varphi_{1} , \ldots , \varphi_{n}}{\psi}\]
in the source logic, is interpreted as a triple:
\[ \triple{\Gamma \mid c_{1} : \trtype{\Gamma}{\varphi_{1}} , \ldots , c_{n} : \trtype{\Gamma}{\varphi_{n}} }{ \trspec{\Gamma}{\varphi_{1}}\left[c_{1}\right] , \ldots , \trspec{\Gamma}{\varphi_{n}}\left[c_{n}\right] }{ m }{\trspec{\Gamma}{\psi}}\left[c_{r}\right] \]
where:
\[ m \in \prog{\left[c_{1} : \trtype{\Gamma}{\varphi_{1}} , \ldots , c_{n} : \trtype{\Gamma}{\varphi_{n}}\right]}{ \left[c_{r} :\trtype{\Gamma}{\psi}\right] } \]

\subsection{Examples}

\subsubsection{Simply Typed Lambda Calculus}

\begin{align*}
    \trtype{\Gamma}{e_{1} = e_{2}} &:= \mathbb{1}\\
    \trtype{\Gamma}{\top} &:= \mathbb{1}\\
    \trtype{\Gamma}{\bot} &:= \mathbb{0}\\
    \trtype{\Gamma}{\varphi_{1} \wedge \varphi_{2}} &:= \trtype{\Gamma}{\varphi_{1}} \times \trtype{\Gamma}{\varphi_{2}}\\
    \trtype{\Gamma}{\varphi_{1} \vee \varphi_{2}} &:= \trtype{\Gamma}{\varphi_{1}} + \trtype{\Gamma}{\varphi_{2}}\\
    \trtype{\Gamma}{\varphi_{1} \supset \varphi_{2}} &:= \trtype{\Gamma}{\varphi_{1}} \Rightarrow \trtype{\Gamma}{\varphi_{2}}\\
    \trtype{\Gamma}{\forall_{x : \tau} . \varphi} &:= \trtype{\Gamma , \tau}{\varphi}\\
    \trtype{\Gamma}{\exists_{x : \tau} . \varphi} &:= \trtype{\Gamma , \tau}{\varphi}
\end{align*}

\begin{align*}
    \trspec{\Gamma}{e_{1} = e_{2}}\left[c\right] &:= e_{1} = e_{2}\\
    \trspec{\Gamma}{\top}\left[c\right] &:= \top\\
    \trspec{\Gamma}{\bot}\left[c\right] &:= \bot\\
    \trspec{\Gamma}{\varphi_{1} \wedge \varphi_{2}}\left[p\right] &:= 
    \trspec{\Gamma}{\varphi_{1}}\subst{\mathsf{fst}\left(p\right)} \wedge \trspec{\Gamma}{\varphi_{2}}\subst{\mathsf{snd}\left(p\right)}\\
    \trspec{\Gamma}{\varphi_{1} \vee \varphi_{2}}\left[p\right] &:=
    \exists x_{1} . \left( p = \mathsf{inl}\left(x_{1}\right) \wedge  \trspec{\Gamma}{\varphi_{1}}\left[x_{1}\right] \right) \vee \exists x_{2} . \left( p = \mathsf{inr}\left(x_{2}\right) \wedge  \trspec{\Gamma}{\varphi_{2}}\left[x_{2}\right] \right)\\
    \trspec{\Gamma}{\varphi_{1} \supset \varphi_{2}}\left[f\right] &:= \forall {c : \trtype{\Gamma}{\varphi_{1}} } . \trspec{\Gamma}{\varphi_{1}}\left[c\right] \supset {\trspec{\Gamma}{\varphi_{2}}\subst{f\left(c\right)}}\\
    \trspec{\Gamma}{\forall {x : \tau} . \varphi}\left[y\right] &:= \forall{x : \tau} .
    \trspec{\Gamma , \tau}{\varphi}\subst{x,y}\\
    \trspec{\Gamma}{\exists {x : \tau} . \varphi}\left[y\right] &:= \exists{x : \tau} .
    \trspec{\Gamma , \tau}{\varphi}\subst{{x,y}}
\end{align*}
\emnote{There is a mismatch between your rules for $\land$ and $\lor$, since the first is defined through the eliminators, while the second via the constructors. Also, in the second case, you don't have the closure wrt. anti-reduction, i.e, if $t \to \inl{t_1}$ and $\trspec{\Gamma}{\varphi_1}[t_1]$, you don't have $\trspec{\Gamma}{\varphi_1\lor \varphi_2}[t]$ (and so, you couldn't define a realizer of $A\land B \supset A \lor B$ such as $\lambda x.\inl(\pi_1 x)$). Nonetheless, if I remember correctly, for the disjunction you need to stick to the elimination rule of the logic, since
taking
\[\trspec{\Gamma}{\varphi_{1} \vee \varphi_{2}}\left[p\right] :=\exists i\in\{1,2\}.
   \trspec{\Gamma}{\varphi_{i}}\left[\mathsf{match}\ p\ \mathsf{with} [x.x|y.y]\right]\]
   leads to troubles I believe, and you need something stronger like (where the type of $\Phi$ should be refined to only convey potential "truth values", i.e. the space of interpretation of formulas $\trspec{\varphi}{\Gamma}$)
\[\trspec{\Gamma}{\varphi_{1} \vee \varphi_{2}}\left[p\right] :=\forall \Phi\in \boldsymbol{Prop}^{\mathcal{B}}.(\forall i\in{1,2}. \forall u. \trspec{\Gamma}{\varphi_{i}}[u] \Rightarrow \Phi (t_i[u/x_i])) \Rightarrow
   \Phi(\mathsf{match}\ p\ \mathsf{with} [x_1.t_1|x_2.t_2])\]
The rules for the quantifications puzzles me, especially the pair $x,y$ that serves as realizers in both cases. I would have expected something more like :
\begin{align*}
    \trspec{\Gamma}{\forall {x : \tau} . \varphi}\left[t\right] &:= \forall{x : \tau} .
    \trspec{\Gamma , \tau}{\varphi}[t]\\
    \trspec{\Gamma}{\exists {x : \tau} . \varphi}\left[t\right] &:= \exists{x : \tau} .
    \trspec{\Gamma , \tau}{\varphi}[t]
\end{align*}
or, if quantifications are given computational content, 
\begin{align*}
    \trspec{\Gamma}{\forall {x : \tau} . \varphi}\left[t\right] &:= \forall{x : \tau} .
    \trspec{\Gamma , \tau}{\varphi}[t\, x]\\
    \trspec{\Gamma}{\exists {x : \tau} . \varphi}\left[t\right] &:= \exists {u:\tau}, t=(u,v) \land
    \trspec{\Gamma , \tau}{\varphi[u/x]}[v]
\end{align*}
}

The triple:
\[  \triple{\Gamma \mid \Sigma}{\Phi}{ c }{\Psi}  \]
is defined as:
\[ \sequent{\Gamma , \Sigma}{\Phi}{\psi\subst{c}} \]
In the case of STLC both $\Gamma$ and $\Sigma$ are taken from the same universe.


\subsubsection{Simplified Evaluation Logic}

\begin{align*}
    \trtype{\Gamma}{e_{1} = e_{2}} &:= \mathbb{1}\\
    \trtype{\Gamma}{\top} &:= \mathbb{1}\\
    \trtype{\Gamma}{\bot} &:= M \mathbb{0}\\
    \trtype{\Gamma}{\varphi_{1} \wedge \varphi_{2}} &:= M \trtype{\Gamma}{\varphi_{1}} \times M \trtype{\Gamma}{\varphi_{2}}\\
    \trtype{\Gamma}{\varphi_{1} \vee \varphi_{2}} &:= M \left( \trtype{\Gamma}{\varphi_{1}} + \trtype{\Gamma}{\varphi_{2}}\right)\\
    \trtype{\Gamma}{\varphi_{1} \supset \varphi_{2}} &:= \trtype{\Gamma}{\varphi_{1}} \Rightarrow M \trtype{\Gamma}{\varphi_{2}}\\
    \trtype{\Gamma}{\forall_{x : \tau} . \varphi} &:= M \trtype{\Gamma , \tau}{\varphi}\\
    \trtype{\Gamma}{\exists_{x : \tau} . \varphi} &:= M \trtype{\Gamma , \tau}{\varphi}
\end{align*}

\begin{align*}
    \trspec{\Gamma}{e_{1} = e_{2}}\left[c\right] &:= e_{1} = e_{2}\\
    \trspec{\Gamma}{\top}\left[c\right] &:= \top\\
    \trspec{\Gamma}{\bot}\left[m\right] &:= \after{m}{c}{\bot}\\
    \trspec{\Gamma}{\varphi_{1} \wedge \varphi_{2}}\left[p\right] &:= 
    \after{\mathsf{fst}\left(p\right)}{x_{1}}{\trspec{\Gamma}{\varphi_{1}}\subst{x_{1}}} \wedge \after{\mathsf{snd}\left(p\right)}{x_{2}}{\trspec{\Gamma}{\varphi_{2}}\subst{x_{2}}}\\
    \trspec{\Gamma}{\varphi_{1} \vee \varphi_{2}}\left[p\right] &:=
    \after{p}{x}{\exists x_{1} . \left( x = \mathsf{inl}\left(x_{1}\right) \wedge  \trspec{\Gamma}{\varphi_{1}}\left[x_{1}\right] \right) \vee \exists x_{2} . \left( x = \mathsf{inr}\left(x_{2}\right) \wedge  \trspec{\Gamma}{\varphi_{2}}\left[x_{2}\right] \right) }\\
    \trspec{\Gamma}{\varphi_{1} \supset \varphi_{2}}\left[f\right] &:= \forall {c : \trtype{\Gamma}{\varphi_{1}} } . \trspec{\Gamma}{\varphi_{1}}\left[c\right] \supset \after{f\left(c\right)}{y}{\trspec{\Gamma}{\varphi_{2}}\subst{y}}\\
    \trspec{\Gamma}{\forall {x : \tau} . \varphi}\left[m\right] &:= \forall{x : \tau} .
    \after{m}{y}{\trspec{\Gamma , \tau}{\varphi}\subst{x,y}}\\
    \trspec{\Gamma}{\exists {x : \tau} . \varphi}\left[m\right] &:= \exists{x : \tau} .
    \after{m}{y}{\trspec{\Gamma , \tau}{\varphi}\subst{{x,y}}}
\end{align*}
\emnote{same observations on $\land/\lor$ and quantifications}
The triple:
\[  \triple{\Gamma \mid \Sigma}{\Phi}{ x \leftarrow m }{\Psi}  \]
is defined as:
\[ \sequent{\Gamma , \Sigma}{\Phi}{\after{m}{x}{\psi\subst{x}}} \]
In the case of Simplified Evaluation Logic both $\Gamma$ and $\Sigma$ are taken from the same universe.

We show that the translation is sound by proving for each theorem \[\sequent{\Gamma}{\varphi_{1} , \ldots , \varphi_{n}}{\Psi}\]
in FOL, that there is some program
\[ f \in \trm{\Gamma}{\trtype{\Gamma}{\varphi_{1}} \times \hdots \times \trtype{\Gamma}{\varphi_{n}} \rightarrow M\trtype{\Gamma}{\psi} } \]
such that:
\[ \triple{\Gamma \mid c_{1} :\trtype{\Gamma}{\varphi_{1}} , \ldots , c_{n} :\trtype{\Gamma}{\varphi_{n}} }{ \Theta }{c_{r} \leftarrow f\left(c_{1} , \ldots , c_{n}\right)}{\trspec{\Gamma}{\psi}\left[ c_{r} \right]} \]
where:
\[ \Theta := \trspec{\Gamma}{\varphi_{1}}\left[ c_{1} \right] , \ldots , \trspec{\Gamma}{\varphi_{n}}\left[ c_{n} \right]\]

For example, say $\varphi_{1} , \varphi_{2}, \varphi_{3} \in \prop{\Gamma}$, the proof of soundness will translate the following theory:

\[ \sequent{\Gamma}{\left(\varphi_{1} \wedge \varphi_{2} \right)\supset \varphi_{3}}{\varphi_{1} \supset \left( \varphi_{2} \supset \varphi_{3} \right)} \]

into the triple:

\[ \triple{\Gamma \mid f : M\trtype{\Gamma}{\varphi_{1}}\times M\trtype{\Gamma}{\varphi_{2}} \rightarrow M\trtype{\Gamma}{\varphi_{3}} }{\Theta_{A}}{g \leftarrow \eta\left(\lambda c_{1} . \eta \left( \lambda c_{2} . f\left(\eta\left(c_{1}\right),\left(\eta\left(c_{2}\right)\right)\right)\right)\right) }{\Theta_{B}} \]
where:
\begin{align*}
    \Theta_{A} & := \forall p . \after{\mathsf{fst}\left(p\right)}{c_{1}}{\trspec{\Gamma}{\varphi_{1}}\subst{c_{1}}} \wedge \after{\mathsf{snd}\left(p\right)}{c_{2}}{\trspec{\Gamma}{\varphi_{2}}\subst{c_{2}}}\\
    & \supset \after{f\left(p\right)}{c_{3}}{\trspec{\Gamma}{\varphi_{3}}\subst{c_{3}}}\\
    \Theta_{B} & := \forall c_{1} . \trspec{\Gamma}{\varphi_{1}}\left[c_{1}\right]\\
    & \supset
    \left\{ h \leftarrow g\left(c_{1}\right) \, \mid \, \forall c_{2} . \trspec{\Gamma}{\varphi_{2}}\left[c_{2}\right] \supset \after{h\left(c_{2}\right)}{c_{3}}{\trspec{\Gamma}{\varphi_{3}}\subst{c_{3}}} \right\}
\end{align*}

While the evidence $\eta\left(\lambda c_{1} . \eta \left( \lambda c_{2} . f\left(\eta\left(c_{1}\right),\left(\eta\left(c_{2}\right)\right)\right)\right)\right)$ may seem weird, it actually aligns perfectly with the type translations, since a realizer of $\varphi_{1} \supset \left( \varphi_{2} \supset \varphi_{3} \right)$ must have the type:
\[ \trtype{\Gamma}{\varphi_{1}}\rightarrow M\left(\trtype{\Gamma}{\varphi_{2}} \rightarrow M\trtype{\Gamma}{\varphi_{3}}\right) \]
\emnote{The first $\eta$ (before $\lambda c_{1}$) is there because of the $c_r \leftarrow...$, right?}
So the evidence program takes the realizer $f$ of $\left(\varphi_{1} \wedge \varphi_{2} \right)\supset \varphi_{3}$ and produces are realizer of $\varphi_{1} \supset \left( \varphi_{2} \supset \varphi_{3} \right)$.

\subsubsection{Monadic Combinatory Algebras}



==> section/higherorder.tex <==
\subsection{Higher-Order Logic}

Consider the last example.
In Higher-Order Logic (HOL), $\varphi_{1} , \varphi_{2} , \varphi_{3}$ can be predicate variables rather than some arbitrary formulas.
However, when trying to translate predicate variables we run into a problem: Since predicate variables represent formulas, and since formulas can have realizers, then predicate variables should have realizers, and these realizers should have a type.

What would be the type realizers of a formula represented by a predicate variable?
The natural choice is to use type variables.
However, for type variables, the target language has to have parametric polymorphism, and by a similar argument, to interpret higher-order predicate variables, it has to have higher-kinded polymorphism.
Furthermore, since predicates are terms, we need to also be able to translate terms. That means we need to extend the translation in several ways.

The idea is as follows: Consider again the last example. In HOL, we could take instead the theorem:

\[ \sequent{\varphi_{1} , \varphi_{2} , \varphi_{3} : \prop{} }{\left(\varphi_{1} \wedge \varphi_{2} \right)\supset \varphi_{3}}{\varphi_{1} \supset \left( \varphi_{2} \supset \varphi_{3} \right)} \]

Here $\Gamma = \varphi_{1} , \varphi_{2} , \varphi_{3} : \prop{}$.

Now in the target language, we'll also have, in addition to the logic and program context, a \emph{kind context} $\Delta$ on which all the other components will depend.
So, in particular, triples now have a kind context $\Delta$:

\[  \triple{\Delta \mid \Gamma \mid \Sigma}{\Phi}{ x \leftarrow m }{\Psi}  \]

Now, since $\varphi_{1} , \varphi_{2} , \varphi_{3}$ are all variables, the type of their realizers will be (resp.) $\tau_{1} , \tau_{2} , \tau_{3}$, all are variables of kind $\star$ (the kind of types), given in $\Delta$. That is: $\Delta = \tau_{1} : \star , \tau_{2} : \star , \tau_{3} : \star$.
Furthermore, just like formulas are translated into formulas over realizers, predicates (including predicate variables) are translated into predicates over realizers. So $\varphi_{1} , \varphi_{2} , \varphi_{3}$ will become predicates on their respective realizers ($\rho_{1} : \pred{\tau_{1}} , \rho_{2} : \pred{\tau_{2}} , \rho_{3} : \pred{\tau_{3}}$).

So now the proof obligation becomes:

\begin{align*}
\tau_{1} : \star , \tau_{2} : \star , \tau_{3} : \star \mid \rho_{1} : \pred{\tau_{1}} , \rho_{2} : \pred{\tau_{2}} , \rho_{3} : \pred{\tau_{3}} \mid & \\
\triple{ f : M\tau_{1}\times M\tau_{2} \rightarrow M\tau_{3} }{\Theta_{A}}{g \leftarrow \eta\left(\lambda c_{1} . \eta \left( \lambda c_{2} . f\left(\eta\left(c_{1}\right),\left(\eta\left(c_{2}\right)\right)\right)\right)\right) }{\Theta_{B}} &
\end{align*}

where:
\begin{align*}
    \Theta_{A} & := \forall p . \after{\mathsf{fst}\left(p\right)}{c_{1}}{\rho_{1}}{c_{1}} \wedge \after{\mathsf{snd}\left(p\right)}{c_{2}}{\rho_{2}}{c_{2}} \supset \after{f\left(p\right)}{c_{3}}{\rho_{3}}{c_{3}}\\
    \Theta_{B} & := \forall c_{1} . \rho_{1}\left[c_{1}\right] \supset
    \left\{ h \leftarrow g\left(c_{1}\right) \, \mid \, \forall c_{2} . \rho_{2}\left[c_{2}\right] \supset \after{h\left(c_{2}\right)}{c_{3}}{\rho_{3}}{c_{3}} \right\}
\end{align*}

\subsubsection{Predicates and Higher-Kinded Polymorphism}

While formulas describe the type of their realizers, predicates describe type constructors, which construct the types of the realizers of the corresponding formulas.
Thus, we need a type system with higher kinds, where $\star$ is the kind of types, and $k \Rightarrow \star$ is the kind of type constructors which take constructors of kind $k$ and return a type.
Since predicates are terms, we might as well assign kinds to terms, and since there are also terms of basic types which are not predicates, we assign them the unit kind $\boldsymbol{1}$, which has a single ``trivial'' constructor $\left\langle\right\rangle$ and for which $\boldsymbol{1} \Rightarrow k \; = ; k$ for every kind $k$.
Now, a predicate of $\pred{\tau}$ is assigned with the kind $k \Rightarrow \star$ where $k$ is the kind assigned to $\tau$.
Thus, terms of basic types, deemed as zero order predicates, are assigned with $\boldsymbol{1}$; first order predicates are assigned with $\boldsymbol{1} \Rightarrow \star$, which is equivalent to $\star$; second order predicates are assigned with $\star \Rightarrow \star$; third order predicates are assigned with $\left( \star \Rightarrow \star \right) \Rightarrow \star$; and so on.

With this framework in mind, predicate variables are interpreted as specifying higher-kinded variables of the appropriate kind.
This framework also dictates how to treat the membership relation which relates a term to a predicate, and comprehension which converts an open formula to a predicate: Whenever $e_{0}$ is a term of type $\tau$, and $e_{1}$ is a predicate of type $\pred{\tau}$, $e_{0}$ specifies a type constructor $\sigma_{0} : k$, and $e_{1}$ specifies a type constructor $\sigma_{1} : k \Rightarrow \star$, so the membership formula $e_{0} \in e_{1}$ is specifying the type $e_{1}\left(e_{0}\right)$.
A formula $\varphi$ with a free variable $x : \tau$ is specifying a type $A$ with a free kind variable $\sigma_{x} : k$ (where $k$ is the kind specified by $\tau$), so the comprehension of it $\comprehend{x}{\tau}{\varphi}$ is specifying the type level abstraction $\lambda \sigma_{x} . A$.

==> section/instantiation.tex <==
\section{Syntactic Instantiations}

As one particularly direct family of instantiations of $\effhol$, we consider syntactic translations into deductive $\fomega$, i.e.~the system obtained from exactly dropping all mention of computations in $\effhol$.
Due to its expressiveness, deductive $\fomega$ is expressive allows to define many instantiations for computations, formally described in the following definition.

\begin{definition} \label{def:instance}
\lcnote{conflicts with  the paragraph "Instances of EffHOL. " on page 8}
An instance of $\effhol$ consists of concrete choices of computation types, return, bind, modal specifications, and evaluation strategy such that:
\begin{itemize}
    \item
    Substitution is respected,
    \item
    Reduction and conversion are preserved,
    \item
    Computation types are well-kinded,
    \item
    Return and bind are well-typed,
    \item
    Modal specifications are well-formed,
    \item
    The rules \modintrorule, \modelimrule, and \monrule~ hold with respect to the induced deduction system of $\fomega$.
\end{itemize}
\end{definition}

Every instance gives rise to a recursive translation $\overline \phi$ of $\effhol$ into deductive $\fomega$ preserving all typing judgements and derivations. So by composition, in particular the soundness theorem extends to every instantiation:

\begin{proposition}
For each $\effhol$ instance and $\ihol$ theorem 
$$\scontext \vdash \sprop_{1} , \ldots , \sprop_{n} \Rrightarrow \sprop $$
and ambient $\fomega$ context $\context$ there is a program $\term$ with
% $$ \term \in \trm{\trkind{\scontext} ; \trind{\trkind{\scontext}}
% {\Gamma}}{\trtype{\Gamma}{\varphi_{1}} \times \hdots \times \trtype{\Gamma}{\varphi_{n}} \rightarrow M\trtype{\Gamma}{\psi} } 
% $$
$$ \eltrm{\overline{\trkind{\scontext}},\kcontext\mid \overline{\ttrtype{}{\sprops}},\tcontext}{\term}{ \overline{M\trtype{}{\sprop} }}$$
% \lcnote{$\trtype{\trkind{\scontext}}{\scontext} $ does not type check. The type context does not come from the sort. 
% Also related, I changed $\trtype{\trkind{\scontext}}{\scontext}$ to $\trtype{\scontext}{\scontext}$, to coincide with the definition, but we should make sure the def works}
such that for every ambient collection $\Phi$ of $\fomega$ specifications:
\[ \htriple{\overline{\ttrkind{\scontext}},\kcontext
\mid \overline{\ttrind{}{\scontext}}, \icontext
\mid \overline{\ttrtype{}{\sprops}} ,\tcontext}
{ \overline{\ttrspec{}{\sprops}{}},\Phi }
{\termvar_{r}} {\term  }
{\overline{\ttrspec{\scontext}{\sprop}{\termvar_{r}}}} \]
where $\ttrtype{}{\sprops} := \termvar_{1} :\ttrtype{\scontext}{\sprop_{1}} , \ldots , \termvar_{n} :\ttrtype{\scontext}{\sprop_{n}}$ and where $\ttrspec{}{\sprops}{} := \trspec{\termvar_{1}}{\sprop_{1}} , \ldots , \trspec{\termvar_{n}}{\sprop_{n}}$.
\end{proposition}

\begin{proof}
Take the translation $\overline p$ for the realizer $p$ obtained from \Cref{thm:soundness}.
\end{proof}

\lcnote{again, I am confused. This is not a result, maybe smt to point out. When you have a system over a language with some uninterpreted symbols, obviously every theorem about the system applies to every concrete instantiation of the system with an interpretation for said symbols. What am I missing?}

==> section/modelHOPL.tex <==
\newcommand{\trform}[1]{\left\llbracket #1 \right\rrbracket}




==> section/overview_old.tex <==
\section{Overview}
\lcnote{first, HOL to program logic + example}

The realizability approach to semantics relates logic with computation by interpreting propositions as denoting specifications of computer programs, or equivalently, using computer programs to demonstrate the validity of propositions.
While the approach is very general, with many variations, at its core it usually relates a specific logic with a specific programming language by translating each proposition in the logic to a specification for programs in the programming language.
To describe the specifications, it requires a meta-language rich enough to specify properties of programming languages, that is, a program logic.
Given a program logic, a realizability interpretation translates each proposition, which is a statement about mathematical structures, to a refinement, which is a statement about computer programs.
\[\begin{tikzcd}
	{\text{Proposition}} &&&&& {\text{Refinement}}
	\arrow["{\text{Realizability Translation}}", from=1-1, to=1-6]
\end{tikzcd}\]

To demonstrate realizability through program logics, consider the following proposition of higher-order logic:
\[ \forall \Phi_{1} . \forall \Phi_{2}  .\left(\Phi_{1} \wedge \Phi_{2}\right) \supset \left(\Phi_{2} \wedge \Phi_{1}\right) \]
A realizability interpretation interprets this proposition as a specification of some set of programs, called the \emph{realizers} of the proposition.
The usual approach interprets an implication $\Phi \supset \Psi$ as specifying a program which takes a realizer of $\Phi$ as an input, and computes a realizer of $\Psi$ as an output.
Conjunction $\Phi_{1} \wedge \Phi_{2}$ is realized by ordered pairs, where the first component is a realizer of $\Phi_{1}$ and the second component is a realizer of $\Phi_{2}$.
A realizer of universal quantification $\forall x . \Phi$ (where $x$ may appear free in $\Phi$) is a program that computes a realizer of $\Phi$ for any $x$.
Bringing it all together, a realizer of $\forall \Phi_{1} . \forall \Phi_{2}  .\left(\Phi_{1} \wedge \Phi_{2}\right) \supset \left(\Phi_{2} \wedge \Phi_{1}\right)$ is a program that for any two propositions $\Phi_{1}$ and $\Phi_{2}$ takes an ordered pair of realizers, of $\Phi_{1}$ and $\Phi_{2}$, and computes an ordered pair of realizers, with the first component being a realizer of $\Phi_{2}$ and the second component a realizer of $\Phi_{1}$.

The program need not be purely functional, and there are no overarching rules as to how that ordered pair has to be computed, what representation it should have, or even whether an actual value of an ordered pair will ever be given.

% Realizability can be considered as a translation of \emph{propositions}, which are mathematical statements about mathematical structures, to \emph{refinements}, which are statements about computer programs.
% \[\begin{tikzcd}
% 	{\text{Proposition}} &&&&& {\text{Refinement}}
% 	\arrow["{\text{Realizability Translation}}", from=1-1, to=1-6]
% \end{tikzcd}\]
% That is, we interpret each proposition as a specification of some set of computer programs, subsequently called the \emph{realizers} of the proposition, constrained by refinements derived from the proposition.
% For example, we may interpret an implication formula $\varphi \supset \psi$ as denoting a set of programs that when given a realizer of $\varphi$ as input they compute a realizer of $\psi$ as output.
% Such a program need not be purely functional, and may exhibit various computational effects.

\agnote{"but what happens when this program exhibits computational effects". GIVE CONCRETE EXAMPLE}

\subsection{First Challenge: Types}
Usually, realizability is based on an untyped notion of computer programs, where all realizers of all propositions have the same type. However, given that many programming languages are typed, we may wish to extend realizability to a typed setting. This presents our first challenge: To support typed realizers in a typed programming language. \agnote{\st{REWRITE: given that most programming languages are typed, the most common realizability method is insufficient [TODO: check typed realizability and compare to this work]. For example.... this presents our first challenge: To support typed realizers}} However, to do so, we have to make sure the realizability translation respects the type structure.
\agnote{GIVE CONCRETE EXAMPLE}

If a realizer of $\varphi \supset \psi$ is a program that converts realizers of $\varphi$ to realizers of $\psi$, then in a typed language it will have an input type $S$, and an output type $T$. Since the program can only take inputs of type $S$ and return outputs of type $T$, all realizers of $\varphi$ will have to have the type $S$ and all realizers of $\psi$ will have to have the type $T$.

\agnote{\st{REWRITE: To address this challenge, we enhance the translation to further include an assignment of a type for each proposition}}
To address this challenge, we enhance the translation to further include an assignment of a type for each proposition. So our translation will now look like this:
\[\begin{tikzcd}
	{\text{Proposition}} &&&&& {\text{Type} \times \text{Refinement}}
	\arrow["{\text{Realizability Translation}}", from=1-1, to=1-6]
\end{tikzcd}\]
\agnote{Now, go back to the examples and show what changes when you add types}
That is, we now need two translation functions: One for the types, and one for the refinements.

\subsection{Second-Order Logic}
\agnote{Why do we suddenly discuss SOL?}
\agnote{"In order to obtain the full expressivity of SOL, we must support propositional variables"... + GIVE EXAMPLE! ... However, this presents us with a further complication... ---> DEMONSTRATE EVERYTHING ON THE EXAMPLE}
Second-order logic leads to a further complication: In second-order logic, we have propositional variables, which are variables standing for propositions.
Suppose the translation assigns for each proposition the type of its realizers, and we consider a propositional variable which stands for a proposition. In that case, this variable should also be assigned with a type for its realizers.
Note that a propositional variable stands for an arbitrary proposition, which can be substituted with a more specific proposition.
A sound translation should be able to respect this idea by allowing a realizer of a propositional variable to be substituted with a more specific realizer whenever we substitute the variable with a more specific proposition.
Hence, a realizer of a propositional variable should itself be a variable.
By a similar argument, the type of realizers of a propositional variable cannot be specific and has to be able to get substituted with a more specific type when the propositional variable is substituted, meaning the type of realizers of a propositional variable will be a type variable.
So to interpret second-order logic, we need our programming language to support parametric polymorphism.
\agnote{explain what is parametric polymorphism and what it gives us. cite a source}

\subsection{Higher-Order Logic}

\agnote{TODO: Remove references to comprehension and terms. Explain the higher-kinded stuff using only predicate variables}

\agnote{Same notes for SOL apply here}

\agnote{Motivate HOL, explain how it creates a new challange. GIVE EXAMPLE!}
Higher-order logic takes the complication above even further. In many-sorted logic, we have some collection of \emph{sorts}, and terms are always defined as having a specific sort from that collection. To keep track of the free variables in a proposition, that is, variables not bound by a quantifier, we define a \emph{context}, which is a list of variables, where each variable is marked with its sort. As in $\left[ x_{1} : \sigma_{1} ,  \ldots , x_{n} : \sigma_{n} \right]$ where $x_{1} ,  \ldots , x_{n}$ are variables and $\sigma_{1} ,  \ldots , \sigma_{n}$ are sorts.

Given a context $\Gamma$, we define the judgements
\[ \jprop{\Gamma}{\varphi} \qquad \qquad \jtrm{\Gamma}{e}{\sigma} \]
meaning, respectively, that $\varphi$ is a proposition and $e$ is a term of sort $\sigma$ in which all free variables are in $\Gamma$.

Higher-order logic is a many-sorted logic, in which for every list of sorts $\Sigma = \left[ \sigma_{1} , \ldots , \sigma_{n} \right]$, there is a sort $\pred{\Sigma}$ of \emph{predicates} over $\Sigma$.
Predicates internalize propositions in the following way: Whenever we have a predicate term $p : \pred{\Sigma}$, where $\Sigma = \left[ \sigma_{1} , \ldots , \sigma_{n} \right]$, and we have terms $e_{1} : \sigma_{1} , \ldots , e_{n} : \sigma_{n}$, then we can apply $p$ on the terms with $\member{\left(e_{1} , \ldots , e_{n}\right)}{p}$.
Furthermore, every proposition $\varphi$ can be abstracted as a predicate by binding some of its free variables, with $\comp{x_{1} : \sigma_{1} , \ldots , x_{n} : \sigma_{n}}{\varphi}$. \agnote{which intuitively stands for...}
In judgement form:
\[ \dfrac{ \jtrm{\Gamma}{p}{\pred{\sigma_{1} , \ldots , \sigma_{n}}} \quad \jtrm{\Gamma}{e_{i}}{\sigma_{i}} \; {\scriptscriptstyle\left(i \in \left\{ 1 , \ldots , n \right\} \right)} }{ \jprop{\Gamma}{\member{\left(e_{1} , \ldots e_{n}\right)}{p}} } \qquad \qquad \dfrac{ \jprop{\Gamma , x_{1} : \sigma_{1} , \ldots , x_{n} : \sigma_{n} }{\varphi} }{\jtrm{\Gamma}{ \comp{x_{1} : \sigma_{1} , \ldots , x_{n} : \sigma_{n}}{\varphi} }{ \pred{\sigma_{1} , \ldots , \sigma_{n}} }} \]

The comprehension axiom relates abstraction with application:
\agnote{REWRITE: What of the key features of HOL comes from the comprehension axiom, which relates predicates with propositions}
\[ \dfrac{\jprop{\Gamma , x_{1} : \sigma_{1} , \ldots , x_{n} : \sigma_{n} }{\varphi} \qquad \jtrm{\Gamma}{e_{i}}{\sigma_{i}} \; {\scriptscriptstyle\left(i \in \left\{ 1 , \ldots , n \right\} \right)} }{ \bisequent{\Gamma}{\member{\left(e_{1} , \ldots e_{n}\right)}{\comp{x_{1} : \sigma_{1} , \ldots , x_{n} : \sigma_{n}}{\varphi}}}{ \varphi\subst{x_{i} := e_{i}}_{i \in \left\{ 1 , \ldots , n \right\}  } }} \]

\agnote{Maybe remove judgements? make it a bit less technical}

This way, we get a hierarchy of propositions, where at the bottom we have first-order propositions defined over contexts which have no predicate sorts, above it second-order propositions defined over contexts with only first-order predicate sorts, then third-order propositions defined over second-order predicate sorts, and so on.

The complication of higher-order logic follows from the following example: Consider the second-order formula $\varphi$ with a free predicate variable $x : \pred{\tau}$.
By comprehension, we get:
\[ \member{ \left(x\right) }{ \comp{x : \pred{\sigma}}{\varphi}} \dashv \vdash \varphi \]
Since $\varphi$ and $\member{ \left(x\right) }{ \comp{x : \pred{\sigma}}{\varphi}}$ are propositions, and $\comp{x : \pred{\sigma}}{\varphi}$ and $x$ are predicates, each is assigned its type of realizers.
The equivalence between $\member{ \left(x\right) }{ \comp{x : \pred{\sigma}}{\varphi}}$ and $\varphi$ means the types of their realizers should also be equivalent.
Since we apply $\comp{x : \pred{\sigma}}{\varphi}$ on $x$ and get something equivalent to $\varphi$, we should also be able to combine the type of realizers of $\comp{x : \pred{\sigma}}{\varphi}$ with the type of realizers of $x$ to get a new type, equivalent to the type of realizers of $\varphi$.
That implies the following things: First, the type of realizers of $\comp{x : \pred{\sigma}}{\varphi}$ should somehow keep information about the type of realizers of $\varphi$. Second, it should be able to allow plugging in the type of realizers of $p$ to get something equivalent to the type of realizers of $\varphi$.
These requirements can be achieved by making the type of realizers of $\comp{x : \pred{\sigma}}{\varphi}$ be parametric in the type of realizers of $x$, that is, a \emph{type operator} rather than a specific type.
Thus, for higher-order logic we need, in addition to polymorphism, a \emph{kind system} that supports \emph{higher kinds}, for type operators.

Finally, we also need to translate each sort in the source language to a type in the target language.
\agnote{Explain PROPERLY the motivation}

That is, the translation would require the following functions:
\[\begin{tikzcd}
	&&&&&& {\text{\Large Kind}} \\
	& {\text{\Large Sort}} \\
	|[rotate=-90]|{\text{\huge Source Logic}} &&&&&& {\text{\Large Index}} & |[rotate=90]|{\text{\huge Target Logic}} \\
	&&&&&& {\text{\Large Type}} \\
	& {\text{\Large Proposition}} \\
	&&&&&& {\text{\Large Refinement}}
	\arrow["\trkind{-}", from=2-2, to=1-7]
	\arrow["\truniv{}{-}", from=2-2, to=3-7]
	\arrow["\trtype{}{-}", from=5-2, to=4-7]
	\arrow["\trprop{}{-}", from=5-2, to=6-7]
\end{tikzcd}\]

\subsection{Examples Intro}

To make things more concrete, we consider two examples of realizability translations, for two different systems. \agnote{emphasize: of two polar edges of the spectrum}
The first example we consider is Deductive System F$\omega$, which is a combination of System F$\omega$ with higher-order logic, allowing us to describe refinements over System F$\omega$ programs.
Since System F$\omega$ is a total purely functional language, it has a non-trivial type system, but the refinements of the translation are trivial direct translations of the propositions.
The second example we consider is Partial Combinatory Algebra, which is a partial algebraic abstraction of models of $\lambda$-calculus.
Partial Combinatory Algebras are untyped, but their partiality means the translation will exhibit non-trivial refinements.

\subsection[Deductive System F-omega]{Deductive System F$\omega$}
\agnote{Use more intuition and words, less technical details. Show for a concrete interesting example instead of a general definition}
Deductive System F$\omega$ combines the propositions of higher-order logic with the types of System F$\omega$, using the types as sorts and making all the propositions depend type operator variables in addition to term variables, and the types of the term variables can depend on the type operator variables.

Deductive System F$\omega$ has a set of kinds $\boldsymbol{Kind}$, and type operators. Each type operator has a kind of the form $\left(k_{1} , \ldots , l_{n}\right) \Rightarrow \star$, meaning it takes type operators of kind $k_{1}$ to $k_{n}$ as arguments to produce a type.
Concrete types have the kind $\left(\right) \Rightarrow \star$, meaning they take no arguments, which can also be written as simply $\star$.

A \emph{kind context}, often marked as $\Delta$, is a list of kinded variables $\left[ \sigma_{1} : k_{1} , \ldots , \sigma_{n} : k_{n} \right]$ where the $\sigma_{i}$ are variables, denoting type operators, each with its assigned kind $k_{i}$.

Each kind context $\Delta$ has its corresponding set of types $\typ{\Delta}$, where all the free type operator variables appear in $\Delta$.

Given a kind context $\Delta$, \emph{type context} over $\Delta$, often marked as $\Gamma_{\Delta}$, is a list of typed variables $\left[ x_{1} : \sigma_{1} , \ldots , x_{n} : \sigma_{n} \right]$ where the $x_{i}$ are variables, denoting terms, each with its assigned type $\sigma_{i}$ taken from $\typ{\Delta}$.

To reason about programs, for each kind context $\Delta$ and each type context $\Gamma_{\Delta}$ over $\Delta$, there is a set $\refin{\Delta}{\Gamma_{\Delta}}$ of \emph{refinements}, defined as the set of propositions in higher-order logic.

The realizability translation we present translates propositions of higher-order logic to refinements of Deductive System F$\omega$.

By abuse of notation, we extend the sort translations to translate contexts: The sort to kind translation is extended to translate sort contexts to kind contexts, and the sort to type translation is extended to translate sort contexts to type context:
\begin{align*}
\trkind{x_{1} : \sigma_{1} , \ldots , x_{n} : \sigma_{n} } &:= \alpha_{x_{1}} : \trkind{\sigma_{1}} , \ldots , \alpha_{x_{n}} : \trkind{\sigma_{n}}\\
\truniv{\alpha_{1} : k_{1} , \ldots , \alpha_{n} : k_{n} }{x_{1} : \sigma_{1}, \ldots , x_{n} : \sigma_{n} } &:= \widehat{x_{1}} : \truniv{\alpha_{1} : k_{1}}{\sigma_{1}} , \ldots , \widehat{x_{n}} : \truniv{\alpha_{n} : k_{n}}{\sigma_{n}} 
\end{align*}
From now on, we'll use the notation:
\[ 
\Delta_{\Sigma} := \trkind{\Sigma}
\qquad
\Gamma_{\Sigma} :=
\truniv{\Delta_{\Sigma}}{\Sigma}
\]
The translation functions are defined by mutual recursion:
\begin{table}[H]
\begin{tabular}{ll}
$\trkind{-} : \mathcal{U} \rightarrow \boldsymbol{Kind}$ &
  $\truniv{-}{-} : \prod_{\sigma \in \mathcal{U}} \prod_{\alpha \in \kvar{\trkind{\sigma}}} \typ{\alpha : \trkind{\sigma} }$
   \\
$\trtype{\Sigma}{-} : \prop{\Sigma} \rightarrow \typ{\Delta_{\Sigma}}$ &
  $\trprop{\Sigma}{-} : \prod_{\varphi \in \prop{\Sigma}} \refin{\Delta_{\Sigma}}{\Gamma_{\Sigma} , c : \trtype{\Sigma}{\varphi}}$
\end{tabular}
\end{table}
For the sorts, we consider only the sort of predicates, recursively assigning each predicate with a type constructor\agnote{\textbf{operator}} for the type of its realizers:
\begin{align*}
    \trkind{\pred{\sigma_{1} , \ldots , \sigma_{n}}} &:= \left(\trkind{\sigma_{1}} , \ldots , \trkind{\sigma_{n}}\right) \Rightarrow \star\\
    \truniv{\alpha : \left(k_{1} , \ldots , k_{n} \right) \Rightarrow \star}{\pred{\sigma_{1} , \ldots , \sigma_{n}}} &:= \prod_{\alpha_{1} : k_{1} , \ldots , \alpha_{n} : k_{n}  } \mathsf{Ref}_{\alpha\left( \alpha_{1} , \ldots , \alpha_{n} \right)}\left(\truniv{\alpha_{1} : k_{1}}{\sigma_{1}} , \ldots , \truniv{\alpha_{n} : k_{n}}{\sigma_{n}} \right)
\end{align*}
% \[ \trkind{\pred{\sigma_{1} , \ldots , \sigma_{n}}} := \left(\trkind{\sigma_{1}} , \ldots , \trkind{\sigma_{n}}\right) \Rightarrow \star \]
% \[ \truniv{\alpha : \left(k_{1} , \ldots , k_{n} \right) \Rightarrow \star}{\pred{\sigma_{1} , \ldots , \sigma_{n}}} := \prod_{\alpha_{1} : k_{1} , \ldots , \alpha_{n} : k_{n}  } \pred{\truniv{\alpha_{1} : k_{1}}{\sigma_{1}} , \ldots , \truniv{\alpha_{n} : k_{n}}{\sigma_{n}} , \alpha\left( \alpha_{1} , \ldots , \alpha_{n} \right) } \]
Each proposition is assigned with the type of its realizers, by recursion over the logical constants:
\begin{align*}
    \trtype{\Sigma}{\varphi_{1} \supset \varphi_{2}} &:= \trtype{\Sigma}{\varphi_{1}} \Rightarrow \trtype{\Sigma}{\varphi_{2}}\\
    \trtype{\Sigma}{\forall_{x : \sigma} . \varphi} &:= \trtype{\Sigma , x : \sigma}{\varphi}\\
    \trtype{\Sigma}{ \member{\left(p_{1} , \ldots , p_{n}\right)}{p} } &:= \alpha_{p} \left(\alpha_{p_{1}} , \ldots , \alpha_{p_{n}}\right)
\end{align*}
The realizability conditions are described for each logical constant as refinements over the corresponding realizer:
\begin{align*}
    \trprop{\Sigma}{\varphi_{1} \supset \varphi_{2}}\left[f\right] &:= \forall_{c : \trtype{\Sigma}{\varphi_{1}} } . \trprop{\Sigma}{\varphi_{1}}\left[c\right] \supset \trprop{\Sigma}{\varphi_{2}}\subst{f\left(c\right)}\\
    \trprop{\Sigma}{\forall_{x : \sigma} . \varphi}\left[y\right] &:= \forall_{x : \truniv{\alpha_{x} : \trkind{\sigma}}{\sigma}} .
    \trprop{\Sigma , x:\sigma}{\varphi}\subst{x,y}\\
    \trprop{\Sigma}{ \member{\left(p_{1} , \ldots , p_{n}\right)}{p} }\subst{c} &:= \member{\left(\widehat{p_{1}} , \ldots , \widehat{p_{n}} ; c\right)}{\widehat{p}}
\end{align*}

\subsection{Partial Combinatory Algebras}
\agnote{more intuition, less tech details. focus on an example}

A standard approach to realizability semantics is to construct realizers by using partial combinatory algebras.
The following realizability translation is the standard construction, presented as an special case of the more general approach of this paper.

\agnote{Explain, \textbf{in words}, what a PCA is, focus on an example}

To reason about PCAs, the notion of refinements over PCAs is described through PCA-valued predicates.
Given a PCA $\mca$ and a set $X$, we call any function of the form $X \rightarrow \P\left(\mca\right)$, where $\P\left(\mca\right)$ is the power set of $\mca$, a $\mca$-valued predicate.
The refinements of the standard translation are $\mca$-valued predicates.

To describe the refinements we introduce the following notation:
\[ \definedto{c_{f} \cdot c_{a}}{\varphi} \]
meaning $c_{f} \cdot c_{a}$ is defined and the result is in $\varphi$:
\[ \exists c_{r} : \mca \; . \; c_{f} \cdot c_{a} \downarrow c_{r} \; \wedge \; c_{r} \in \varphi \]

Since PCAs have only one type, there is no need for a kind system, so there is no need for a kind translation either.
Instead, we only need the following translation functions:
\agnote{Note: $\boldsymbol{Set}$ is the class of logical types, $\left\{\mca\right\}$ is the class of program types}
\[ \truniv{}{-} : \mathcal{U} \rightarrow \boldsymbol{Set} \qquad
    \trtype{\Gamma}{-} : \prop{\Gamma} \rightarrow \left\{ \mca \right\} \qquad
    \trprop{\Gamma}{-} : \prop{\Gamma} \rightarrow \truniv{}{\Gamma} \rightarrow \P\mca \]
Where $\truniv{}{\Gamma}$ is defined by extending $\truniv{}{-}$ to contexts through a cartesian product:
\[ \truniv{}{\left[x_{1} : \sigma_{1} , \ldots , x_{n} : \sigma_{n}\right]} := \truniv{}{\sigma_{1}} \times \cdots \times \truniv{}{\sigma_{n}}  \]
With $\truniv{}{-}$ assigning a set to each context $\Gamma$, $\trprop{\Gamma}{-}$ translates each proposition over $\Gamma$ into an $\mca$-valued predicate over $\truniv{}{\Gamma}$.
\[ \truniv{}{\pred{\sigma_{1} , \ldots , \sigma_{n}}} := \P\left(\truniv{}{\sigma_{1}} \times \cdots \times \truniv{}{\sigma_{n}} \right) \]
The type translation is trivial, since there is only one possible type to choose from:
\[ \trtype{\Gamma}{\varphi_{1} \supset \varphi_{2}} := \mca
    \qquad
    \trtype{\Gamma}{\forall_{x : \tau} . \varphi} := \mca
    \qquad
    \trtype{\Gamma}{e_{0} \in_{\tau} e_{1}} := \mca \]
The translation is using a set-theoretic foundation to describe the refinements, so they are defined through set comprehension notation, with the refinement of implication now accounting for partiality:
\begin{align*}
    \trprop{\Sigma}{\varphi_{1} \supset \varphi_{2}}\left(\gamma\right) &:= \comp{c_{f} : \mca}{ \forall {c_{a} : \mca } . c_{a} \in \trprop{\Sigma}{\varphi_{1}}\left(\gamma\right) \; \supset \; \definedto{c_{f} \cdot c_{a}}{\trprop{\Sigma}{\varphi_{2}}}\left(\gamma\right) }\\
    \trprop{\Sigma}{\forall {x : \sigma} . \varphi}\left(\gamma\right) &:= \comp{c : \mca}{ \forall{x : \sigma} .
    c \in \trprop{\Sigma , x:\sigma}{\varphi}\left(\left\langle\gamma,x\right\rangle\right)}\\
    \trprop{\Sigma}{ \member{\left(p_{1} , \ldots , p_{n}\right)}{p} }\left(\left\langle\gamma , A , a_{1} , \ldots , a_{n}\right\rangle\right) &:= \comp{ c : \mca }{\left\langle a_{1} , \ldots , a_{n} , c \right\rangle \in A }
\end{align*}

\agnote{Summarize... + "Now I'm going to give a general framework of using program logic to model HOL, which is substainally more flexibe than previous works. The examples we've seen are special cases but we will also present more subtle and complex cases such as higher-kinded simplified evaluation logic, [EXPLAIN IN WORDS WHAT IS HKSEvalLogic]. For the logics we consider in this paper we provide the following soundness result: [The Soundness Theorem] }


\lcnote{suggested structure for the rest of the paper below:}

\section{Higher-Kinded Polymorphic Evaluation Logic}
\agnote{Rename HKPEL to Higher Evaluation Logic}
As a general, complex example. explain why it is important and the difference from previous examples in the overview.
Formal definition of the  logic.
\agnote{no need to deal with basic types}

\section{From HOL to HKPEL}
\subsection{First-Order Fragment}
base types translation
\subsection{Higher-Order Fragment}
extending with sorts (predicates), membership (propositions) and comprehansion.
\subsection{Soundness}
soundness result and corollaries

\section{Examples}
\subsection{$F_\omega$}
\subsection{PCA}
\subsection{MCAs}
definition, examples.
probability example as a new one

\section{Related Work}

\section{Conclusion}


\lcnote{=======END OF STRUCTURE==========}

==> section/semModel.tex <==
\section{Modeling $\effhol$ via Monadic Combinatory Algebra}
\label{sec:MCAmodel}
\input{section/MCAmodel}




\subsection{Categorical Model for $\effhol$}
\label{sec:semantics}
%\input{section/semantics}
\input{section/semanticDiscussion}


==> section/semanticDiscussion.tex <==
%
Since $\effhol$ combines components of three languages, namely, Higher-Order Logic, System $F_\omega$, and Evaluation Logic, a categorical semantics for it requires a careful combination of the semantics of these languages.
%
More concretely, constructing such a semantics must include the  necessary components for modeling higher-order structure, higher-kinded polymorphism, and computational types and modalities.
%
In a nutshell, we use indexed categories to interpret polymorphism, in a similar manner to Seely’s categorical semantics for higher-order polymorphic lambda calculus~\cite{seely1987categorical}, an indexed strong monad for computational types, along with a tripos~\cite{hyland1980tripos} and a T-modality (as in Evaluation Logic~\cite{pitts1991evaluation}), for the logical components. 
% we build on Seely's approach~\cite{seely1987categorical} for modeling polymorphism which uses a cartesian closed category $\basecat$ in which the objects model the kind contexts and the morphisms model type constructors.
% Higher-order logic is captured via triposes~\cite{hyland1980tripos}, while the interpretation of computational types and modality is obtained through an adaptation of the semantics of Evaluation Logic~\cite{pitts1991evaluation}.
%
However, interleaving these structures in a way that preserves the consistency of the structure while producing a sound semantics for $\effhol$ is non-trivial and therefore we leave its full construction to a future paper.  %and cannot to be introduced in this paper. 
%
%Since this paper focuses on the syntactic account of $\effhol$, and the full, detailed description of such a structure is quite complex, we here opt to provide only a high-level description of how such a model is obtained, leaving the full construction to a future paper. 
%We  next provide some high-level description of how such a model is obtained, leaving the full construction to a future paper. 



% Seely~\cite{seely1987categorical} describes a standard approach for modeling polymorphism, that uses some cartesian closed category $\basecat$ in which the objects model the kind contexts and the morphisms model type constructors. A specific object $\typeobj$ in $\basecat$ is designated as the kind of types. A type $\type$ in kind context $\kcontext$ is interpreted as a morphism in $\basecat$ from the interpretation of $\kcontext$ to $\typeobj$.
% To interpret programs, a $\basecat$-indexed category $\indcat$, which is a contravariant functor
% $\indcat: \opcat{\basecat} 
% \rightarrow \catcat$ 
% into the category $\catcat$ of small categories, is used.
% Objects in $\indcat\left(\baseobject\right)$, where $\baseobject \in \obj{\basecat}$, are morphisms in $\basecat$ from $\baseobject$ to $\typeobj$, so types and type contexts in kind context $\kcontext$ are interpreted as both morphisms in $\basecat$ and as objects in $\indcat\left(\baseobject\right)$, where $\baseobject$ is the interpretation of $\kcontext$, and similarly, 
% programs in kind context $\kcontext$ are interpreted as morphisms in $\indcat\left(\baseobject\right)$.

% The interpretation of higher-order logic is based on triposes~\cite{hyland1980tripos}.
% It requires a contravariant functor $\P_{\baseobject} :  \opcat{\indcat\left(\baseobject\right)} \rightarrow \preordcat$ for each $\basecat$ object $\baseobject$ into the category $\preordcat$ of preordered sets.
% Specifications are interpreted as elements in a preordered set in the image of the functor.

% The interpretation of computational types and modality, requires an adaptation of the semantics of Evaluation Logic~\cite{pitts1991evaluation}.
% It is based on monads $\monad_{\baseobject}$ over $\indcat\left(\baseobject\right)$ for each object $\baseobject$ in $\basecat$. 
% Effectful programs of a computation type $\typecomp{\type}$ are interpreted as morphisms in the corresponding Kleisli category of $\monad_{\baseobject}$.
% To relate the specifications with effectful programs, the tripos functor $\P_{\baseobject}$ has to be an oplax post-module of $\monad_{\baseobject}$, meaning there is a natural transformation $\rho : \P_{\baseobject} \circ \monad_{\baseobject} \Rightarrow \P_{\baseobject}$ that weakly commutes with monad operations of $\monad_{\baseobject}$.




==> section/semantics.tex <==
The semantics of $\effhol$ combines several structures.
For the interpretation of higher-kinded polymorphism, we adopt a variation of PL categories, introduced in \cite{seely1987categorical}.
The interpretation of higher-order logic is based on triposes, introduced in \cite{hyland1980tripos}.
The interpretation of computational types and modality is based on the semantics of Evaluation Logic, introduced in \cite{pitts1991evaluation}.

%\begin{definition}[Indexed Category]\label{def:indexed-category}
Given a base category $\basecat$, a \emph{$\basecat$-indexed category} $\indcat$ is a functor $\indcat : \opcat{\basecat} \rightarrow \catcat$.
We write $\ind{\indcat}{\baseobject}$ for the category that is the image of $\indcat$ on the $\basecat$ object $\baseobject$ and $\ind{\indcat}{\basemap}$ for the functor that is the image of $\indcat$ on the $\basecat$ morphism $\basemap$. 
%\end{definition}
%
%\begin{definition}[Indexed Functor]\label{def:indexed-functor}
For $\basecat$-indexed categories $\mathbb{C} , \mathbb{D}$, a
\emph{$\basecat$-functor} $\functor : \mathbb{C} \Rightarrow \mathbb{D}$ is a natural transformation between them as functors.
We write $\ind{\functor}{\baseobject}$ for the component of $\functor$ on $\baseobject$, $\ind{\functor}{\baseobject}\left(a\right)$ for its image on $\ind{\indcat}{\baseobject}$ object $a$, and $\ind{\functor}{\baseobject}f$ for its image on morphism $f$.
%\end{definition}
%
%\begin{definition}[Indexed Natural Transformation]\label{def:indexed-nattrans}
Finally, given $\basecat$-indexed categories $\mathbb{C} , \mathbb{D}$, and $\basecat$-indexed functors $\functor , \functor' : \mathbb{C} \Rightarrow \mathbb{D}$, a \emph{$\basecat$-indexed natural transformation} $\nattrans : \functor \Rrightarrow \functor'$ is a family of natural transformations $\ind{\nattrans}{\baseobject}: \ind{\functor}{\baseobject} \Rightarrow \ind{\functor'}{\baseobject}$ for every $\baseobject$ in $\basecat$, such that, for any $\basemap \in \hom{\basecat}{\baseobject}{\baseobject'}$:
\[ \ind{\nattrans}{\baseobject} \circ \ind{\mathbb{C}}{\basemap} = \ind{\mathbb{D}}{\basemap} \circ \ind{\nattrans}{\baseobject'} \]
We write $\ind{\nattrans}{\baseobject}_{a}$ for $\ind{\nattrans}{\baseobject}$ component on $\ind{\indcat}{\baseobject}$ object $a$.
For readability, we will omit the component subscript whenever it can be inferred from the context.
%\end{definition}

Indexed categories are useful for interpreting polymorphism, but to combine them with other categorical notions, a useful trick is to convert them into categories through the Grothendieck construction. Given a $\basecat$-indexed category $\indcat$, the Grothendieck construction of $\indcat$, marked $\int\indcat$, is the category which has as objects pairs $\left(\baseobject , \object\right)$ where $\baseobject \in \obj{\basecat}$ and $\object \in \obj{\ind{\indcat}{\baseobject}}$, and a morphism from $\left(\baseobject_{1} , \object_{1}\right)$ to $\left(\baseobject_{2} , \object_{2}\right)$ is a pair $\left(\basemap , u\right)$ such that $\basemap \in \hom{\basecat}{\baseobject_{1}}{\baseobject_{2}}$ and $u \in \hom{\ind{\indcat}{\baseobject_{1}}}{\object_{1}}{ \ind{\indcat}{\basemap}\left(\object_{2}\right) }$.\agnote{CITATION}
Given two $\basecat$-indexed categories $\indcat_{1}$ and $\indcat_{2}$, a $\basecat$-indexed functor $\functor : \indcat_{1} \Rightarrow \indcat_{2}$ induces a functor $\int\functor : \int\indcat_{1} \rightarrow \int\indcat_{2}$, hereby referred to as the \emph{induced functor} of $\functor$, between the corresponding Grothendieck constructions of the corresponding categories.
$\int\functor$ is defined on objects by $\int\functor\left(\baseobject , \object\right) = \left(\baseobject , \ind{\functor}{\baseobject}\left(\object\right)\right)$, and on morphisms by $\int\functor\left(\basemap , u\right) = \left(\basemap , \ind{\functor}{\baseobject_{1}}u \right)$.
\agnote{TODO: Explain induced natural transformation}
For every $\basecat$-indexed category $\indcat$ and every $\baseobject \in \obj{\basecat}$ there is a functor
$ J_{\baseobject} : \ind{\indcat}{\baseobject} \rightarrow \int\indcat $
defined on objects and morphisms (resp.) with:
\[ J_{\baseobject}\left(\object\right) = \left(\baseobject ,  \object\right) \qquad J_{\baseobject}\left(u\right) = \left(\id_{\baseobject} , u\right)\]
Note that this functor has the property that for every $\basecat$-indexed functor $\functor : \indcat_{1} \rightarrow \indcat_{2}$ the following equation holds:
\[ J^{2}_{\baseobject} \circ \ind{\functor}{\baseobject} = \int\functor \circ J^{1}_{\baseobject} \]
Given a base morphism $\basemap \in \hom{\basecat}{\baseobject_{1}}{\baseobject_{2}}$, we have natural transformation $J_{\basemap} : J_{\baseobject_{1}} \circ \ind{\indcat}{\basemap} \Rightarrow J_{\baseobject_{2}}$ defined by:
\[ J_{f} = \left(f , \id\right) \]

% To interpret expressions in $\effhol$ we need a category with some specific features to support \lcnote{TODO}

\begin{definition}[\lcnote{pick a name}E-category]
    An E-category, $\expcat$, is a $\basecat$-indexed category, where:
    \begin{itemize}
        \item 
    each object component $\ind{\expcat}{\baseobject}$ is a cartesian category, 
    \item 
    each morphism component $\ind{\expcat}{\basemap}$ preserves cartesian products and terminal objects, and
    \item 
             for every $\kcontext , \kind \in \obj{\basecat}$, the functor $\ind{\expcat}{\pi_{1}} : \ind{\expcat}{\kcontext} \rightarrow \ind{\expcat}{\kcontext\times\kind}$ has a right adjoint, $\radj{\ind{\expcat}{\pi_{1}}}$.
    % following functors have right adjoints:
        % \begin{align*}
        % \ind{\indcat}{\pi_{1}} &: \ind{\indcat}{\kcontext} \rightarrow \ind{\indcat}{\kcontext\times\kind} \\
        %     \ind{\expcat}{\pi_{1}} &: \ind{\expcat}{\kcontext} \rightarrow \ind{\expcat}{\kcontext\times\kind}
        % \end{align*}
    \end{itemize}
\end{definition}



\begin{definition}[PL-category]
A PL-category, denoted by $\plcat$, is a tuple
$\left(\basecat , \indcat, \typeobj \right)$, 
where:
\begin{itemize}
    \item $\basecat$ is a CCC (Cartesian Closed Category)

    \item $\indcat$ is a $\basecat$-indexed category

    \item $\typeobj \in \obj{\basecat}$   (some designated object in $\basecat$ used to denote the kind of types)
\end{itemize}
satisfying the following properties:\lcnote{can/should we name them?}
\begin{enumerate}

    \item For each $\baseobject \in \obj{\basecat}$, $\ind{\indcat}{\baseobject}$ is a CCC and $\obj{\ind{\indcat}{\baseobject}} = \hom{\basecat}{\baseobject}{\typeobj}$

    %\item For each $\baseobject \in \obj{\basecat}$, $\ind{\indcat}{\baseobject}$ is a CCC 

    \item For each $\baseobject_{1} , \baseobject_{2} \in \obj{\basecat}$, and each $\basemap \in \hom{\basecat}{\baseobject_{1}}{\baseobject_{2}}$, the functor $\ind{\indcat}{\basemap} : \ind{\indcat}{\baseobject_{2}} \rightarrow \ind{\indcat}{\baseobject_{1}}$ strictly preserves the CCC structure (products, terminal object, and exponentials)

    \item For each $\baseobject \in \basecat$, the canonical indexed functor $\ind{\indcat}{\pi_{1}} : \indcat \rightarrow \ind{\indcat}{- \times \baseobject}$ has a right adjoint
    
\end{enumerate}
\end{definition}

To interpret modality we lift the notion of a strong monad 
and we adopt and generalize the notion of a monad modality described in \cite{pitts1991evaluation}. 
\begin{definition}[Indexed Strong Monad]
    A $\basecat$-indexed strong monad over $\indcat$ is a tuple $\left(\monad, \eta, \mu , t \right)$ where $\monad : \indcat \Rightarrow \indcat$ is a $\basecat$-indexed endofunctor over $\indcat$, with $\eta : \mathbb{1} \Rrightarrow \monad$ and $\mu : \monad\monad \Rrightarrow \monad$ being $\basecat$-indexed natural transformations, satisfying the monad laws for any index $\baseobject$, and $t$ a $\basecat$-indexed natural transformation satisfying the strength laws.
    We sometimes standardly only write $\monad$ for the monad.\lcnote{is it ok to say?that's what you do}
\end{definition}

\begin{theorem}
    Given a $\basecat$-indexed category $\indcat$, and a $\basecat$-indexed monad $\monad$ over $\indcat$, the induced functor $\int\monad$ is a monad on the Grothendieck construction $\int\indcat$
\end{theorem}

\lcnote{TODO: adjust this paragraph to the new draft. Provide an intuitive explaination.}
To relate the semantics of computational effects (monads) with the semantics of logic (hyperdoctrines\lcnote{cite}), we define a notion we call \emph{oplax post-module}.
Concretely, this notion is used to interpret specifications involving modality.
%
Oplax post-modules, when defined in the context of a hyperdoctrine with inverse image functor $\P$ with a monad $M$, ``lift'' formulas over values in $\P\left(A\right)$ to formulas over computations in $\P\left(M\left(A\right)\right)$.
It can be considered as a way to turn a pure proposition into a post-condition on the result of a computation.
The laws of an oplax post-module ensure that post-conditions are preserved through entailment by introducing the basic operations of the monad.
\begin{definition}[Oplax Post-Module]
Given a monad $\monad$ over category $\indcat$, an oplax post-module for $\monad$ is a pair $\left( \P , \module \right)$ where $\P : \indcat \rightarrow \opcat{\preordcat}$ is a functor, and $\module : \P \circ \monad \Rightarrow \P$ is a natural transformation which satisfies the following conditions, for any $\object \in \obj{\indcat}$ and $\varphi \in \P\left(\object\right)$:
$$
\varphi \leq \P{\eta} \left( \module \left( \varphi \right) \right) 
\qquad ; \qquad 
\module \left( \module \left( \varphi \right) \right) \leq \P{\mu} \left( {\module} \left( \varphi \right) \right)
$$
\end{definition}

\begin{definition}[$\effhol$ structure]
An $\effhol$-structure is a tuple
%$\left(\basecat , \indcat, \typeobj , \monad , \mu, \eta, t, \P , \module \right)$, 
$\left(\plcat , \monad ,  \expcat, \expfun, \P \right)$, 
where:
\begin{itemize}
    \item $\plcat=\left(\basecat , \indcat, \typeobj\right)$ is a PL category over $\indcat$

        \item $\monad : \indcat \Rightarrow \indcat$ is a $\basecat$-indexed strong monad
    
    \item $\expcat$ is an E-category

    \item $\expfun : \indcat \times \expcat \Rightarrow \expcat$ is a $\basecat$-indexed functor \agnote{TODO: explain product of indexed categories}, equipped with the following $\basecat$-indexed natural isomorphisms \agnote{Should I mention that this is an \emph{actegory}?}:
    \begin{align*}
        \ind{\unitor}{\baseobject}_{\icontext} &: \icontext \rightarrow \ind{\expfun}{\baseobject}\left(\terminalobj , \icontext\right)\\
        \ind{\associator}{\baseobject}_{\tcontext_{1},\tcontext_{2},\icontext} &: \ind{\expfun}{\baseobject}\left(\tcontext_{1} , \ind{\expfun}{\baseobject}\left(\tcontext_{2} , \icontext\right)\right) \rightarrow \ind{\expfun}{\baseobject}\left(\tcontext_{1} \times \tcontext_{2} , \icontext\right)
    \end{align*}

    \item $\P : \int\expcat \rightarrow \opcat{\preordcat} $ is a functor 
    % , without the Galois connections of weakening
    \end{itemize}

satisfying the following properties:

    \begin{itemize}

    \item Each of the compositions $\P \circ \expcat_{\baseobject} : \ind{\expcat}{\baseobject}  \rightarrow \opcat{\preordcat}$ is a tripos
    
    % \item Each of the compositions $\P \circ \expcat_{\baseobject} \circ \ind{\expfun}{\baseobject} : \ind{\indcat}{\baseobject} \times \ind{\expcat}{\baseobject} \rightarrow \opcat{\preordcat}$  is an oplax post-module \lcnote{definition? assumption? lemma?}

    \item $\P$ is an oplax post-module of $\int \monad$

    \item For every $\kcontext \in \obj{\basecat}$, and every $\icontext, \indice \in \ind{\expcat}{\kcontext}$, the monotonic map $\P\left(\id , \pi_{1}\right) : \P\left( \kcontext , \icontext \right) \rightarrow \P\left( \kcontext ,  \icontext \times \indice \right)$ has a right adjoint $\radj{\P\left(\id , \pi_{1}\right)}$\lcnote{isn't this a property of $\P$?}
    % \item For every $\kcontext , \kind \in \obj{\basecat}$, every $\tcontext, \type \in \ind{\indcat}{\kcontext}$, and every $\icontext, \indice \in \ind{\expcat}{\kcontext}$, the following monotonic maps have right Galois connections:
    % \begin{align*}
    %     % \P\left(\id, \ind{\expfun}{\pi_{1}}\times \id \right) &: \P\left(\kcontext , \ind{\expfun}{\kcontext}\left(\tcontext\right) \times \icontext \right) \rightarrow \P\left(\kcontext , \ind{\expfun}{\kcontext}\left(\tcontext \times \type\right) \times \icontext \right)\\
    %     \P\left(\id , \pi_{1}\right) &: \P\left( \kcontext , \icontext \right) \rightarrow \P\left( \kcontext ,  \icontext \times \sort \right)\\
    %     \P\left(\pi_{1} , \id\right) &: \P\left(\kcontext ,  \icontext \right) \rightarrow \P\left(\kcontext \times \kind , \ind{\expcat}{\pi_{1}}\left(\icontext \right)\right)
    % \end{align*}



    % \item The proposition kind weakening indexed functor $\P\left(\pi_{1} , \id\right) : \P\left(-,\Gamma \right) \Rightarrow \P\left(- \times \kind , \fstadj{\kind}\left(\Gamma\right) \right)$ has a right adjoint
    % \[ \foralladj{\kind} : \P\left(- \times \kind , \fstadj{\kind}\left(\Gamma\right) \right) \Rightarrow \P\left(-,\Gamma \right) \]

    % \item $\ind{\expcat}{\pi_{1}} : \ind{\expcat}{\baseobject_{1}} \rightarrow \ind{\expcat}{\baseobject_{1} \times \baseobject_{2}}$ has a right adjoint \agnote{I'm out of universal quantifier symbols}\lcnote{just put a macro with a bar/hat/whatever.}
\end{itemize}

Note that the first projection in $\int\expcat$ is a pair of projections $\left(\pi_{1} , \pi_{1}\right)$, and since $\P$ is a tripos, the inverse image of the first projection $\P\left(\pi_{1} , \pi_{1}\right)$ has a right adjoint, which we mark as $\radj{\P\left(\pi_{1} , \pi_{1}\right)}$.
For all of the mentioned adjunctions, we use $\adjunit$ and $\adjcounit$ to mark the unit and counit of the adjunction, including the unit of the monad $\monad$.

\end{definition}

% We recall the definition of a PL category from~\cite{}, which is essentially an indexed category which is at the basis for interpreting higher-kinded frameworks. 
% \begin{definition}[PL category]
% A PL category, $\plcat$, is...    
% \end{definition}

% For modeling higher-order logic we take the standard notion of a tripos, $\tripos$, as in, e.g.~\cite{}. 

% \begin{definition}    
% \end{definition}

% \begin{definition}[$\effhol$-structure]
   
% \end{definition}

% By construction, we have the following, ensuring a proper model. 
% \lcnote{ Is this semantics "standard"? does it give us a tripos? denotational sem? extensional?}
% \lcnote{What's the relation to the one for EL?}


% \begin{proposition}
%     An $\effhol$-structure is a tripos.
% \end{proposition}

\input{section/figures/seminter}

\begin{definition}[Interpretation of $\effhol$]
Given a $\effhol$-structure, we interpret $\effhol$ by first interpreting kinds as objects in $\basecat$:
\[ \interpkind{\typecon{\kind_{1} , \ldots , \kind_{n}}} := \expobj{\interpkind{\kind_{1}} \times \cdots \times \interpkind{\kind_{n}}}{\typeobj} \]

Kind contexts are interpreted recursively with binary products:
\begin{align*}
    \interpkind{\emptyset} &:= \terminalobj\\
    \interpkind{\kcontext , \typevar : \kind} &:= \interpkind{\kcontext} \times \interpkind{\kind}
\end{align*}
Type variables are interpreted as the composition of projections accordingly.

A type $\type$ in kind context $\kcontext$ is interpreted as a base morphism, or equivalently as an object in the category $\ind{\indcat}{\interpkind{\kcontext}}$:
\[ \interptype{\kcontext}{\type} \in \hom{\basecat}{\interpkind{\kcontext}}{\typeobj} = \obj{\ind{\indcat}{\interpkind{\kcontext}}}  \]
The interpretation of types in a kind context is defined recursively. We take advantage of the fact that objects in $\obj{\ind{\indcat}{\interpkind{\kcontext}}}$ are morphisms in $\hom{\basecat}{\interpkind{\kcontext}}{\typeobj}$ to interpret the first three forms as morphisms in $\hom{\basecat}{\baseobject}{\typeobj}$ and the last three as objects in $\obj{\ind{\indcat}{\baseobject}}$:
\begin{align*}
    \interptype{\typevar_{1} : \kind_{1} , \ldots , \typevar_{n} : \kind_{n}}{\typevar_{j}} &:= \pi_{2} \circ \pi_{1}^{\left(n-j\right)} \\
    \interptype{\kcontext}{\typeapp{\type_{1}}{\type_{2}}} &:= \adjcounit \circ \pair{\interptype{\kcontext}{\type_{2}}}{\interptype{\kcontext}{\type_{1}}}\\
    \interptype{\kcontext}{\typeabs{\typevar}{\kind}{\type}} &:= \expobj{\interptype{\kcontext}{\type}}{\interpkind{\kind}} \circ \adjunit\\
    \interptype{\kcontext}{\typefun{\type_{1}}{\type_{2}}} &:= \expobj{\interptype{\kcontext}{\type_{1}}}{\interptype{\kcontext}{\type_{2}}}\\
    \interptype{\kcontext}{\ttypprod{\typevar:\kind}{\type}} &:= \radj{\ind{\indcat}{\pi_{1}}} \left(\interptype{\kcontext , \typevar : \kind}{\type}\right)\\
    \interptype{\kcontext}{\typecomp{\type}} &:= \monad \left(\interptype{\kcontext}{\type}\right)
\end{align*}

Indices in context $\kcontext$ are interpreted as objects in $\obj{\ind{\expcat}{\interpkind{\kcontext}}}$, using the tripos structure over it to interpret predicates, and the right adjoint $\radj{\ind{\expcat}{\pi_{1}}}$ to interpret kind universal quantification. Types are embedded in $\ind{\expcat}{\interpkind{\kcontext}}$ through the $\expfun$ functor:
\begin{align*}
    \interptype{\kcontext}{\refpredN{\type}} :=  \pred{\ind{\expfun}{ \interpkind{\kcontext} }\left(\interptype{\kcontext}{\type} , \terminalobj \right)}\\
    \interptype{\kcontext}{\refpred{\type}{\indice}} := \pred{\ind{\expfun}{ \interpkind{\kcontext} }\left(\interptype{\kcontext}{\type} , \interptype{\kcontext}{\indice}\right)}\\
    \interptype{\kcontext}{\tindprod{\typevar:\kind}{\indice}} := \radj{\ind{\expcat}{\pi_{1}}}\left(\interptype{\kcontext , \typevar : \kind}{\indice}\right)
\end{align*}

% Kind contexts are interpreted recursively with binary products:
% \begin{align*}
%     \interptype{\kcontext}{\emptyset} &:= \terminalobj\\
%     \interptype{\kcontext}{\tcontext , \termvar : \type} &:= \interptype{\kcontext}{\tcontext} \times \interptype{\kcontext}{\type}
% \end{align*}

Programs of type $\type$ in kind context $\kcontext$ and type context $\tcontext$ are interpreted as morphisms in $\hom{\ind{\indcat}{\interpkind{\kcontext}}}{\interptype{\kcontext}{\tcontext}}{\interptype{\kcontext}{\type}}$
\begin{align*}
    \interpterm{\kcontext}{\termvar_{1} : \type_{1} , \ldots , \termvar_{n} : \type_{n}}{\termvar_{j}} &:= \pi_{2} \circ \pi_{1}^{\left(n-j\right)}\\
    \interpterm{\kcontext}{\tcontext}{\termtypeabs{\typevar}{\term}} &:= \radj{\ind{\indcat}{\pi_{1}}}\left(\interpterm{\kcontext , \typevar : \kind}{\tcontext}{\term}\right) \circ \adjunit\\
    \interpterm{\kcontext}{\tcontext}{\termabs{\termvar}{\term}} &:= \expobj{\interptype{\kcontext}{\type_{1}}}{\left(\interpterm{\kcontext}{\tcontext , \termvar : \type}{{\term}}\right)} \circ \adjunit \\
    \interpterm{\kcontext}{\tcontext}{\termtypeapp{\term}{\type}} &:= \ind{\indcat}{\pair{\id}{\interptype{\kcontext}{\type}}} \adjcounit \circ \interpterm{\kcontext}{\tcontext}{\term}  \\
    \interpterm{\kcontext}{\tcontext}{\termapp{\term_{1}}{\term_{2}}} &:= \adjcounit \circ \pair{\interpterm{\kcontext}{\tcontext}{\term_{1}}}{\interpterm{\kcontext}{\tcontext}{\term_{2}}} \\
    \interpterm{\kcontext}{\tcontext}{\termret{\term}} &:= \eta \circ \interpterm{\kcontext}{\tcontext}{\term}\\
    \interpterm{\kcontext}{\tcontext}{\termbind{\termvar}{\term_{1}}{\term_{2}}} &:= \mu \circ \monad\interpterm{\kcontext}{\tcontext , \termvar : \type}{\term_{2}} \circ \strength \circ \pair{\id}{\interpterm{\kcontext}{\tcontext}{\term_{1}}}
\end{align*}

Expressions of index $\indice$ in kind context $\kcontext$, term context $\tcontext$, and index context $\icontext$ are interpreted as morphisms in $\hom{\ind{\expcat}{\interpkind{\kcontext}}}{ \ind{\expfun}{\interpkind{\kcontext}}\left(\interptype{\kcontext}{\tcontext} , \interptype{\kcontext}{\icontext}\right)}{\interptype{\kcontext}{\indice}}$
\begin{align*}
    \interpexpr{\kcontext}{\tcontext}{\epred_{1} : \indice_{1} , \ldots , \epred_{n} : \indice_{n}}{\epred_{j}} &:= \unitor^{-1} \circ \ind{\expfun}{\interpkind{\kcontext}}\left(\terminalmap , \pi_{2} \circ \pi_{1}^{\left(n-j\right)}\right)\\
    \interpexpr{\kcontext}{\tcontext}{\icontext}{\ecomp{\termvar}{\type}{\exprsvar}{\indice}{\tprop}} &:= {\color{red} \text{COMPREHENSION}}\\
    \interpexpr{\kcontext}{\tcontext}{\icontext}{\eforall{\typevar:\kind}{\exprs}} &:= \radj{\ind{\expcat}{\pi_{1}}} \interpexpr{\kcontext , \typevar : \kind}{\tcontext}{\icontext}{\exprs} \circ \adjunit \\
    \interpexpr{\kcontext}{\tcontext}{\icontext}{\eapp{\exprs}{\type}} &:= \ind{\expcat}{\pair{\id}{\interptype{\kcontext}{\type}}} \adjcounit \circ \interpexpr{\kcontext}{\tcontext}{\icontext}{\exprs}
\end{align*}

Specifications in kind context $\kcontext$, term context $\tcontext$, and index context $\icontext$ are interpreted as elements of $\P\left(\interpkind{\kcontext} , \ind{\expfun}{\interpkind{\kcontext}}\left(\interptype{\kcontext}{\tcontext}, \interptype{\kcontext}{\icontext}\right)\right)$
\begin{align*}
    \interpspec{\kcontext}{\tcontext}{\icontext}{\tmem{\term}{\exprs}{\langle \exprs\rangle}} &:= \\
    \interpspec{\kcontext}{\tcontext}{\icontext}{\timplies{ \tprop_{1} }{ \tprop_{2} }} &:= \interpspec{\kcontext}{\tcontext}{\icontext}{\tprop_{1}} \sqsupset \interpspec{\kcontext}{\tcontext}{\icontext}{\tprop_{2}}\\
    \interpspec{\kcontext}{\tcontext}{\icontext}{\after{\term}{\termvar}{\tprop}} &:= \P\left( \id , \ind{\expfun}{\interpkind{\kcontext}}\left( \strength \circ \pair{\id}{\interpterm{\kcontext}{\tcontext}{\term}} , \id \right) \right)\left(\rho\left(\interpspec{\kcontext}{\tcontext , \termvar : \type}{\icontext}{\tprop}\right)\right)\\
    \interpspec{\kcontext}{\tcontext}{\icontext}{\tspeckinprod{\typevar:\kind}{\tprop}} &:= \radj{\P\left( \pi_{1} \right)}  \left( \P\left(\id , \pi_{1}\right)\left( \interpspec{\kcontext , \typevar : \kind}{\tcontext}{\icontext}{ \tprop}\right)\right)\\
    \interpspec{\kcontext}{\tcontext}{\icontext}{\tspectypprod{\termvar:\type}{\tprop}} &:=
    \radj{\P\int\expfun\left(\id , \pi_{1}\right)} \left( \P\left( \id , \ind{\expfun}{\kcontext}\left(\id,\pi_{1}\right) \right)\left( \interpspec{\kcontext}{\tcontext , \termvar:\type}{\icontext}{\tprop} \right)\right) \\
    \interpspec{\kcontext}{\tcontext}{\icontext}{\tspecindprod{\epred:\indice}{\tprop}} &:= \radj{\P\int\expfun\left(\id , \pi_{1}\right)} \left( \P\left( \id , \ind{\expfun}{\kcontext}\left(\pi_{1}, \id\right) \right)\left(\interpspec{\kcontext}{\tcontext}{\icontext , \epred:\indice}{\tprop}\right)\right)
\end{align*}

\end{definition}

\begin{lemma}[WF]\label{semwf}
The following hold:
        \begin{enumerate}
        \item 
    If $\eltype{\kcontext}{\type:\kind}$, then $\pi_{k} \in \hom{\basecat}{\kind_{1} \times \ldots \times \kind_{n}}{\kind_{k}}$
    \item 
    If $\eltrm{\kcontext \mid \tcontext}{\term}{\type}$ then: 
    \item If $\eltrm{\context}{\exprs}{\indice}$ then
    \item If $\eltype{\context}{\tprop}$ then
     \end{enumerate}
\end{lemma}

\begin{theorem}[Soundness]\label{thm:semsound}
    If $\elsequent{\context}{\tprops }{\tprop} $, then 
\end{theorem}

aFrom the soundness of $\effhol$ with respect to $\effhol$-structures we naturally obtain its consistency.

\begin{corollary}[Consistency]
    $\effhol$ is consistent.
\end{corollary}


\subsubsection{Interpreting the Signature of the Realizability Translation}

The signature needed for the realizability translation, as described in \Cref{chap:translation}, requires several components.
Given a $\boldsymbol{Set}$ based model as described above, along with an MCA $\mca$ for the given monad $M$, the signature is interpreted by using interpreting the type of codes $\mca$ as the MCA $\mca$; for each two types, the type of pairs is interpreted as the cartesian product of their interpretation, and application procedure symbol is interpreted as the application operator of $\mca$.
Furthermore, the required function symbols are interpreted by using the abstraction operator to construct the appropriate realizers.
For example: $\seminterp{\Cid} := \encode{0}{0}$, and $\seminterp{\Ccompose{e_{1}}{e_{2}}} := \encode{0}{e_{2} \bullet \left( e_{1} \bullet 0 \right)}$.




==> section/semantics2.tex <==
The semantics of $\effhol$ combines several structures.
For the interpretation of higher-kinded polymorphism, we adopt a variation of PL categories, introduced in \cite{seely1987categorical}.
The interpretation of higher-order logic is based on triposes, introduced in \cite{hyland1980tripos}.
The interpretation of computational types and modality is based on the semantics of Evaluation Logic, introduced in \cite{pitts1991evaluation}.

%\begin{definition}[Indexed Category]\label{def:indexed-category}
Given a base category $\basecat$, a \emph{$\basecat$-indexed category} $\indcat$ is a functor $\indcat : \opcat{\basecat} \rightarrow \catcat$.
We write $\ind{\indcat}{\baseobject}$ for the category that is the image of $\indcat$ on the $\basecat$ object $\baseobject$ and $\ind{\indcat}{\basemap}$ for the functor that is the image of $\indcat$ on the $\basecat$ morphism $\basemap$. 
%\end{definition}
%
%\begin{definition}[Indexed Functor]\label{def:indexed-functor}
For $\basecat$-indexed categories $\mathbb{C} , \mathbb{D}$, a
\emph{$\basecat$-functor} $\functor : \mathbb{C} \Rightarrow \mathbb{D}$ is a natural transformation between them as functors.
We write $\ind{\functor}{\baseobject}$ for the component of $\functor$ on $\baseobject$, $\ind{\functor}{\baseobject}\left(a\right)$ for its image on $\ind{\indcat}{\baseobject}$ object $a$, and $\ind{\functor}{\baseobject}f$ for its image on morphism $f$.
%\end{definition}
%
%\begin{definition}[Indexed Natural Transformation]\label{def:indexed-nattrans}
Finally, given $\basecat$-indexed categories $\mathbb{C} , \mathbb{D}$, and $\basecat$-indexed functors $\functor , \functor' : \mathbb{C} \Rightarrow \mathbb{D}$, a \emph{$\basecat$-indexed natural transformation} $\nattrans : \functor \Rrightarrow \functor'$ is a family of natural transformations $\ind{\nattrans}{\baseobject}: \ind{\functor}{\baseobject} \Rightarrow \ind{\functor'}{\baseobject}$ for every $\baseobject$ in $\basecat$, such that, for any $\basemap \in \hom{\basecat}{\baseobject}{\baseobject'}$:
\[ \ind{\nattrans}{\baseobject} \circ \ind{\mathbb{C}}{\basemap} = \ind{\mathbb{D}}{\basemap} \circ \ind{\nattrans}{\baseobject'} \]
We write $\ind{\nattrans}{\baseobject}_{a}$ for $\ind{\nattrans}{\baseobject}$ component on $\ind{\indcat}{\baseobject}$ object $a$.
For readability, we will omit the component subscript whenever it can be inferred from the context.
%\end{definition}

Indexed categories are useful for interpreting polymorphism, but to combine them with other categorical notions, a useful trick is to convert them into categories through the Grothendieck construction. Given a $\basecat$-indexed category $\indcat$, the Grothendieck construction of $\indcat$, marked $\int\indcat$, is the category which has as objects pairs $\left(\baseobject , \object\right)$ where $\baseobject \in \obj{\basecat}$ and $\object \in \obj{\ind{\indcat}{\baseobject}}$, and a morphism from $\left(\baseobject_{1} , \object_{1}\right)$ to $\left(\baseobject_{2} , \object_{2}\right)$ is a pair $\left(\basemap , u\right)$ such that $\basemap \in \hom{\basecat}{\baseobject_{1}}{\baseobject_{2}}$ and $u \in \hom{\ind{\indcat}{\baseobject_{1}}}{\object_{1}}{ \ind{\indcat}{\basemap}\left(\object_{2}\right) }$.\agnote{CITATION}
Given two $\basecat$-indexed categories $\indcat_{1}$ and $\indcat_{2}$, a $\basecat$-indexed functor $\functor : \indcat_{1} \Rightarrow \indcat_{2}$ induces a functor $\int\functor : \int\indcat_{1} \rightarrow \int\indcat_{2}$, hereby referred to as the \emph{induced functor} of $\functor$, between the corresponding Grothendieck constructions of the corresponding categories.
$\int\functor$ is defined on objects by $\int\functor\left(\baseobject , \object\right) = \left(\baseobject , \ind{\functor}{\baseobject}\left(\object\right)\right)$, and on morphisms by $\int\functor\left(\basemap , u\right) = \left(\basemap , \ind{\functor}{\baseobject_{1}}u \right)$.
\agnote{TODO: Explain induced natural transformation}
For every $\basecat$-indexed category $\indcat$ and every $\baseobject \in \obj{\basecat}$ there is a functor
$ J_{\baseobject} : \ind{\indcat}{\baseobject} \rightarrow \int\indcat $
defined on objects and morphisms (resp.) with:
\[ J_{\baseobject}\left(\object\right) = \left(\baseobject ,  \object\right) \qquad J_{\baseobject}\left(u\right) = \left(\id_{\baseobject} , u\right)\]
Note that this functor has the property that for every $\basecat$-indexed functor $\functor : \indcat_{1} \rightarrow \indcat_{2}$ the following equation holds:
\[ J^{2}_{\baseobject} \circ \ind{\functor}{\baseobject} = \int\functor \circ J^{1}_{\baseobject} \]
Given a base morphism $\basemap \in \hom{\basecat}{\baseobject_{1}}{\baseobject_{2}}$, we have natural transformation $J_{\basemap} : J_{\baseobject_{1}} \circ \ind{\indcat}{\basemap} \Rightarrow J_{\baseobject_{2}}$ defined by:
\[ J_{f} = \left(f , \id\right) \]

% \begin{definition}[\lcnote{pick a name}E-category]
%     An E-category, $\expcat$, is a $\basecat$-indexed category, where:
%     \begin{itemize}
%         \item 
%     each object component $\ind{\expcat}{\baseobject}$ is a cartesian category, 
%     \item 
%     each morphism component $\ind{\expcat}{\basemap}$ preserves cartesian products and terminal objects, and
%     \item 
%              for every $\kcontext , \kind \in \obj{\basecat}$, the functor $\ind{\expcat}{\pi_{1}} : \ind{\expcat}{\kcontext} \rightarrow \ind{\expcat}{\kcontext\times\kind}$ has a right adjoint, $\radj{\ind{\expcat}{\pi_{1}}}$.
%     % following functors have right adjoints:
%         % \begin{align*}
%         % \ind{\indcat}{\pi_{1}} &: \ind{\indcat}{\kcontext} \rightarrow \ind{\indcat}{\kcontext\times\kind} \\
%         %     \ind{\expcat}{\pi_{1}} &: \ind{\expcat}{\kcontext} \rightarrow \ind{\expcat}{\kcontext\times\kind}
%         % \end{align*}
%     \end{itemize}
% \end{definition}

\begin{definition}[PL-category]
A PL-category, denoted by $\plcat$, is a tuple
$\left(\basecat , \indcat, \typeobj \right)$, 
where:
\begin{itemize}
    \item $\basecat$ is a CCC (Cartesian Closed Category)

    \item $\indcat$ is a $\basecat$-indexed category

    \item $\typeobj \in \obj{\basecat}$   (some designated object in $\basecat$ used to denote the kind of types)
\end{itemize}
satisfying the following properties:\lcnote{can/should we name them?}
\begin{enumerate}

    \item For each $\baseobject \in \obj{\basecat}$, $\ind{\indcat}{\baseobject}$ is a CCC and $\obj{\ind{\indcat}{\baseobject}} = \hom{\basecat}{\baseobject}{\typeobj}$

    %\item For each $\baseobject \in \obj{\basecat}$, $\ind{\indcat}{\baseobject}$ is a CCC 

    \item For each $\baseobject_{1} , \baseobject_{2} \in \obj{\basecat}$, and each $\basemap \in \hom{\basecat}{\baseobject_{1}}{\baseobject_{2}}$, the functor $\ind{\indcat}{\basemap} : \ind{\indcat}{\baseobject_{2}} \rightarrow \ind{\indcat}{\baseobject_{1}}$ strictly preserves the cartesian structure (products and terminal object)
    % CCC structure (products, terminal object, and exponentials)

    \item For each $\baseobject \in \basecat$, the canonical indexed functor $\ind{\indcat}{\pi_{1}} : \indcat \rightarrow \ind{\indcat}{- \times \baseobject}$ has a right adjoint
    
\end{enumerate}
\end{definition}

To interpret modality we lift the notion of a strong monad 
and we adopt and generalize the notion of a monad modality described in \cite{pitts1991evaluation}. 
\begin{definition}[Indexed Strong Monad]
    A $\basecat$-indexed strong monad over $\indcat$ is a tuple $\left(\monad, \eta, \mu , t \right)$ where $\monad : \indcat \Rightarrow \indcat$ is a $\basecat$-indexed endofunctor over $\indcat$, with $\eta : \mathbb{1} \Rrightarrow \monad$ and $\mu : \monad\monad \Rrightarrow \monad$ being $\basecat$-indexed natural transformations, satisfying the monad laws for any index $\baseobject$, and $t$ a $\basecat$-indexed natural transformation satisfying the strength laws.
    We sometimes standardly only write $\monad$ for the monad.\lcnote{is it ok to say?that's what you do}
\end{definition}

\begin{theorem}
    Given a $\basecat$-indexed category $\indcat$, and a $\basecat$-indexed monad $\monad$ over $\indcat$, the induced functor $\int\monad$ is a monad on the Grothendieck construction $\int\indcat$
\end{theorem}

\begin{proof}
    TBD
\end{proof}

Note that due to the aformentioned property of $J_{\baseobject}$, we get:
\[ \int\monad \circ J_{\baseobject} = J_{\baseobject} \circ \ind{\monad}{\baseobject}  \]

\lcnote{TODO: adjust this paragraph to the new draft. Provide an intuitive explaination.}
To relate the semantics of computational effects (monads) with the semantics of logic (hyperdoctrines\lcnote{cite}), we define a notion we call \emph{oplax post-module}.
Concretely, this notion is used to interpret specifications involving modality.
%
Oplax post-modules, when defined in the context of a hyperdoctrine with inverse image functor $\P$ with a monad $M$, ``lift'' formulas over values in $\P\left(A\right)$ to formulas over computations in $\P\left(M\left(A\right)\right)$.
It can be considered as a way to turn a pure proposition into a post-condition on the result of a computation.
The laws of an oplax post-module ensure that post-conditions are preserved through entailment by introducing the basic operations of the monad.
\begin{definition}[Oplax Post-Module]
Given a monad $\monad$ over category $\indcat$, an oplax post-module for $\monad$ is a pair $\left( \P , \module \right)$ where $\P : \indcat \rightarrow \opcat{\preordcat}$ is a functor, and $\module : \P \circ \monad \Rightarrow \P$ is a natural transformation which satisfies the following conditions, for any $\object \in \obj{\indcat}$ and $\varphi \in \P\left(\object\right)$:
$$
\varphi \leq \P{\eta} \left( \module \left( \varphi \right) \right) 
\qquad ; \qquad 
\module \left( \module \left( \varphi \right) \right) \leq \P{\mu} \left( {\module} \left( \varphi \right) \right)
$$
\end{definition}

Note that if you define an oplax post-module have a $\baseobject$-indexed monad $\monad$, and an oplax post-module over a Grothendieck construction $\P : \int \indcat \rightarrow \opcat{\preordcat}$ for the induced monad $\int\monad$, that is:
\[ \rho : \P \circ \int \monad \Rightarrow \P\]
you get an oplax post-module for each of the instances of $\monad$, because:
\[ \int \monad \circ J_{\baseobject} = J_{\baseobject} \circ \ind{\monad}{\baseobject}\]
so by horizontal compostion you get the oplax post-module:
\[ \rho_{J_{\baseobject}} : \P \circ J_{\baseobject} \circ \ind{\monad}{\baseobject} \Rightarrow \P \circ J_{\baseobject} \]

\begin{definition}[$\effhol$ structure]
An $\effhol$-structure is a tuple
$\left(\basecat , \indcat, \statecat , \expcat , \typeobj , \monad, \pfreyd, \P \right)$, 
% $\left(\plcat , \monad , \P \right)$, 
where:
\begin{itemize}
    \item $\basecat$ is a CCC (Cartesian Closed Category)

    \item $\indcat$, $\statecat$, and $\expcat$ are cartesian $\basecat$-indexed categories

    \item $\typeobj \in \obj{\basecat}$   (some designated object in $\basecat$ used to denote the kind of types)

    \item $\monad : \indcat \Rightarrow \indcat$ is a $\basecat$-indexed strong monad, with strength $\strength$

    \item $\pfreyd : \indcat \times \statecat \Rightarrow \expcat$ is a $\basecat$-indexed functor 

    \item $\P : \int\expcat \rightarrow \opcat{\preordcat} $ is a functor 

    
    \end{itemize}

satisfying the following properties:

    \begin{itemize}

        \item For every $\baseobject \in \obj{\basecat}$, $\ind{\expcat}{\baseobject}$ has all the objects of $\ind{\left( \indcat \times \statecat \right)}{\baseobject}$, that is, all pairs of objects of $\ind{\indcat}{\baseobject}$ and $\ind{\statecat}{\baseobject}$ (with possibly other objects as well)

        \item For each $\baseobject \in \obj{\basecat}$, $\ind{\pfreyd}{\baseobject}$ is the identity on objects ($\ind{\pfreyd}{\baseobject}\left(\cxtpair{\tcontext}{\icontext}\right) = \cxtpair{\tcontext}{\icontext}$)

    \item For each $\baseobject \in \obj{\basecat}$, $\ind{\indcat}{\baseobject}$ is a cartesian category with $\monad$-Kleisli exponentials
    
    \item For each $\baseobject \in \obj{\basecat}$, objects of $\ind{\indcat}{\baseobject}$ are reflected in $\basecat$ through $\obj{\ind{\indcat}{\baseobject}} = \hom{\basecat}{\baseobject}{\typeobj}$

    %\item For each $\baseobject \in \obj{\basecat}$, $\ind{\indcat}{\baseobject}$ is a CCC 

    \item For each $\baseobject_{1} , \baseobject_{2} \in \obj{\basecat}$, and each $\basemap \in \hom{\basecat}{\baseobject_{1}}{\baseobject_{2}}$, the functor $\ind{\indcat}{\basemap} : \ind{\indcat}{\baseobject_{2}} \rightarrow \ind{\indcat}{\baseobject_{1}}$ strictly preserves the cartesian structure (products and terminal object), and $\monad$-Kleisli exponentials
    % CCC structure (products, terminal object, and exponentials)

    \item For each $\baseobject \in \basecat$, the canonical indexed functors $\ind{\indcat}{\pi_{1}} : \indcat \rightarrow \ind{\indcat}{- \times \baseobject}$ and $\ind{\expcat}{\pi_{1}} : \expcat \rightarrow \ind{\expcat}{- \times \baseobject}$ have right adjoints $\radj{\ind{\indcat}{\pi_{1}}}$ and $\radj{\ind{\expcat}{\pi_{1}}}$ (resp.)

    \item Each of the compositions $\P \circ \indemb{\baseobject}^{\expcat} : \ind{\expcat}{\baseobject}  \rightarrow \opcat{\preordcat}$ is a tripos
    
    % \item Each of the compositions $\P \circ \expcat_{\baseobject} \circ \ind{\expfun}{\baseobject} : \ind{\indcat}{\baseobject} \times \ind{\expcat}{\baseobject} \rightarrow \opcat{\preordcat}$  is an oplax post-module \lcnote{definition? assumption? lemma?}

    \item $\P \circ \int\pfreyd$ is an oplax post-module of $\int \widehat{\monad}$

    \item Specification right adjoints $\radj{Q_{\kcontext}\left(\cxtpair{\pi_{1}}{\id}\right)}$, $\radj{Q_{\kcontext}\left(\cxtpair{\id}{\pi_{1}}\right)}$, and.... where $Q_{\kcontext} \eqdef \P \circ \int \pfreyd \circ \indemb{\kcontext} =  \P \circ \indemb{\kcontext} \circ \ind{\pfreyd}{\kcontext}$

    % \item $\ind{\expcat}{\pi_{1}} \circ \ind{\pfreyd}{\kcontext} = \ind{\pfreyd}{\kcontext \times \kind} \circ \ind{\left(\indcat \times \statecat\right)}{\pi_{1}}$

\end{itemize}

\end{definition}

\subsection{Interpretation}

Given an $\effhol$-structure as described above, we define interpretation functions by mutual recursion on the structure of the syntax.
To that end, we define:
\[ Q_{\kcontext} \eqdef \P \circ \int \pfreyd \circ \indemb{\kcontext} =  \P \circ \indemb{\kcontext} \circ \ind{\pfreyd}{\kcontext} \]

\begin{align*}
    \interp{\star} & \eqdef \typeobj \\
    \interp{\typecon{\kind}} & \eqdef \typeobj^{\interp{\kind}} 
\end{align*}

\begin{align*}
    \interp{\typevar} & \eqdef \\
    \interp{\typeapp{\type}{\type}} & \eqdef \\
    \interp{\typeabs{\typevar}{\kind}{\type}} & \eqdef \\
    \interp{\typefun{\type}{\typecomp{\type}}} & \eqdef \\
    \interp{\ttypprod{\typevar:\kind}{\type}} & \eqdef \\
    \interp{\typecomp{\type}} & \eqdef 
\end{align*}

\begin{align*}
    \interp{\termvar_{k}}_{\kcontext \mid \termvar_{1} : \type_{1} , \ldots , \termvar_{n} : \type_{n} } & \eqdef \pi_{k} \\
    \interp{\termtypeabs{\typevar}{\kind}{\term}} & \eqdef \radj{\ind{\indcat}{\pi_{1}}}\interp{\term} \circ \eta\\
    \interp{\termabs{\termvar}{\type}{\term}} & \eqdef  \expobj{\type_{1}}{\interp{\term}}  \circ \eta \\
    \interp{\termtypeapp{\term}{\type}} & \eqdef \\
    \interp{\termapp{\term_{1}}{\term_{2}}} & \eqdef \\
    \interp{\termret{\term}} & \eqdef \eta \circ \interp{\term} \\
    \interp{\termbind{\termvar}{\term_{1}}{\term_{2}}} & \eqdef \mu \circ \monad\interp{\term_{2}} \circ \strength \circ \pair{\id}{\interp{\term_{1}}}
\end{align*}

\begin{align*}
    \interp{\refpred{\type}{\indice}} & \eqdef \\
    \interp{\tindprod{\typevar:\kind}{\indice}} & \eqdef 
\end{align*}

\begin{align*}
    \interp{\ecomp{\termvar}{\type}{\exprsvar}{\indice}{\tprop}} & \eqdef \left\{ \interp{\tprop} \right\} \\
    \interp{\ecompbase{\termvar}{\type}{\tprop}} & \eqdef \\
    \interp{\eforall{\typevar:\kind}{\exprs}} & \eqdef \radj{\ind{\expcat}{\pi_{1}}}\left(\interp{\exprs}\right) \\
    \interp{\eapp{\exprs}{\type}} & \eqdef 
\end{align*}

\begin{align*}
    \interp{\tmembase{\term}{\exprs}}_{\kcontext \mid \tcontext \mid \icontext} & \eqdef  \\
    \interp{\timplies{ \tprop }{ \tprop }}_{\kcontext \mid \tcontext \mid \icontext} & \eqdef \\
    \interp{\after{\term}{\termvar}{\tprop}}_{\kcontext \mid \tcontext \mid \icontext} & \eqdef \afterinterp{\interp{\termvar}}  \\
    \interp{\tspeckinprod{\typevar:\kind}{\tprop}} & \eqdef \kuinterp{\interp{\tprop}}\\
    \interp{\tspectypprod{\termvar:\type}{\tprop}}_{\kcontext \mid \tcontext \mid \icontext} & \eqdef \tuinterp{\interp{\tprop}} \\
    \interp{\tspecindprod{\epred:\indice}{\tprop}}_{\kcontext \mid \tcontext \mid \icontext} & \eqdef \iuinterp{\interp{\tprop}}
\end{align*}

% $\left(\plcat , \monad , \P \right)$ where $\plcat=\left(\basecat , \indcat, \typeobj\right)$, kinds are interpreted as objects of $\basecat$, types and indices in kind context $\kcontext$ as objects in $\ind{\indcat}{\kcontext}$, programs and expressions as morphisms in $\ind{\indcat}{\kcontext}$, and specifications over $\kcontext \mid \tcontext \mid \icontext$ as elements of $\P \left( J_{\kcontext}\left( \tcontext \times \icontext\right)\right)$.

% \subsection{The Syntactic Category of $\effhol$}

% To get completeness, we need to define the syntactic category of $\effhol$, derived from the syntax, and show that it is a model.
% However, the separation of programs and expressions complicates things.

% Given kind context $\kcontext$ and program contexts $\tcontext_{1}, \tcontext_{2}$ over $\kcontext$, a program substitution from $\tcontext_{1}$ to $\tcontext_{2}$ is a substitution where all the variables in $\tcontext_{2}$ are assigned with a program over $\tcontext_{1}$ (that is, a program where all the free variables are in $\tcontext_{1}$).
% Thus, we can define an indexed category $\mathsf{Prog}$, indexed over the category of kind substitutions, where the objects are program contexts morphisms are program  substitutions between them.
% That is, $\hom{\ind{\mathsf{Prog}}{\kcontext}}{\tcontext_{1}}{\tcontext_{2}}$ is the hom-set of substitutions from $\tcontext_{1}$ to $\tcontext_{2}$.
% This is possible because all the variables inside programs denote arbitrary programs, so program substitutions are self-contained.

% Expressions, on the other hand, may include both program variables and expression variables, and a simultaneous substitution should be able to replace both, so to make expression substitutions self-contained enough to define hom-sets, they need to consider both program contexts and expression contexts.
% Thus, to define a syntactic category of expression substitutions, you need the objects to be pairs of the form $\left( \tcontext , \icontext \right)$ where $\tcontext$ is a program context and $\icontext$ is an expression context.
% Then, a substitution from $\left( \tcontext_{1} , \icontext_{1} \right)$ to $\left( \tcontext_{2} , \icontext_{2} \right)$ is a pair where the first component is a program substitution from $\tcontext_{1}$ to $\tcontext_{2}$ and the second component is a substitution which assigns to each variable in $\icontext_{2}$ an expression over $\tcontext_{1} \mid \icontext_{1}$.
% This way, we get an indexed-category of expression substitutions, called $\mathsf{Exp}$, where $\hom{\ind{\mathsf{Exp}}{\kcontext}}{\tcontext_{1} \mid \icontext_{1}}{\tcontext_{2} \mid \icontext_{2}}$ is the hom-set of expression substitutions from $\left( \tcontext_{1} , \icontext_{1} \right)$ to $\left( \tcontext_{2} , \icontext_{2} \right)$ as described above.
% This indexed category almost has the structure of a $\effhol$-structure, however, while $\mathsf{Prog}$ has a strong monad, $\mathsf{Exp}$ inherits the monad from $\mathsf{Prog}$ but it does not inherit its strength, since the cartesian structure of $\mathsf{Exp}$ does not reflect the cartesian structure of $\mathsf{Prog}$.
% Thus it can't form a model until we include in the semantics some form of separation between the interpretation of programs and the interpretation of expressions.

\subsection{Soundness}

\input{section/figures/HOPL_semantics}
